Less is more: Embracing sparsity and interpolation with Esiformer for time series forecasting

Time series forecasting has played a significant role in many practical fields. But time series data generated from real-world applications always exhibits high variance and lots of noise, which makes it difficult to capture the inherent periodic patterns of the data, hurting the prediction accuracy significantly. To address this issue, we propose the Esiformer, which apply interpolation on the original data, decreasing the overall variance of the data and alleviating the influence of noise. What's more, we enhanced the vanilla transformer with a robust Sparse FFN. It can enhance the representation ability of the model effectively, and maintain the excellent robustness, avoiding the risk of overfitting compared with the vanilla implementation. Through evaluations on challenging real-world datasets, our method outperforms leading model PatchTST, reducing MSE by 6.5% and MAE by 5.8% in multivariate time series forecasting. Code is available at: https://github.com/yyg1282142265/Esiformer/tree/main.

==> sections/2_related_work.tex <==
\section{Related Work}\label{sec_related_works}

%{\color{blue}

\subsection{Time-series Forecasting}

Temporal variation modeling is a prominent issue in time series analysis and has been extensively investigated with numerous methods been proposed to achieve accurate long-term time series forecasting.

Early studies typically employed traditional statistical methods or machine learning techniques, such as ARIMA (Anderson \& Kendall, 1976) \cite{box_arima2}, Holt-Winter (Hyndman \& Athanasopoulos, 2018) \cite{Holt-Winter18}, DeepAR (Salinas et al., 2020)\cite{DBLP:journals/corr/FlunkertSG17-deepAR} and Prophet (Taylor \& Letham, 2018) \cite{Taylor2018ForecastingAS}. With the rise of deep learning, researchers have turned their attention to more robust and complex neural networks for time series modeling, including TCN (Bai et al., 2018) \cite{TCN}, LSTM (Hochreiter et al., 1997)\cite{hochreiter_long_1997_lstm}. Specifically, N-BEATS (Oreshkin et al., 2019) \cite{nbeats} designed an interpretable layer by encouraging the model to learn trend, seasonality explicitly, and residual components, which shows superior performance on the M4 competition dataset; Dlinear (Zeng et al., 2022)\cite{Dlinear} employs a simple linear layer, while TimesNet (Wu et al. 2023) \cite{TIMESNET} extends the analysis of temporal variations into the 2D space enabling to discover the multi-periodicity adaptively and extract the complex temporal variations. 

Among these, the Transformer (Vaswani et al., 2017) ~\cite{attention_is_all_you_need} and its subsequent adaptations have demonstrated significant success in long sequence modelling tasks, including time series forecasting.  Informer (Zhou et al., 2021) \cite{haoyietal-informer-2021} proposes a ProbSparse self-attention mechanism and distilling operation to address the quadratic complexity of the Transformer, while Reformer (Kitaev et al., 2020)\cite{KitaevKL20-reformer} replaces dot-product attention by using locality-sensitive hashing and improves its complexity, resulting in significant performance improvements. Subsequently, Autoformer (Wu et al. 2021) \cite{Autoformer} designs an efficient auto-correlation mechanism to discover and aggregate information at the series level; FiLM (Zhou
et al., 2022) \cite{zhou2022film} design a Frequency improved Legendre Memory model applying Legendre polynomial projections to approximate historical information, while FEDformer 
et al., 2022) \cite{FedFormer} proposes an attention mechanism with low-rank approximation in frequency and a mixture of experts decomposition to control the distribution shifting. Additionally, Pyraformer (Liu et al., 2022) \cite{liu2022pyraformer} designs pyramidal attention to effectively describe short and long temporal dependencies with low time and space complexity and patchTST (Nie et al., 2023) \cite{patchTST} embeds the whole time series of each variate independently into tokens to enlarge local receptive field. Recently, FPT (Zhou
et al., 2022) \cite{zhou2023onefitsall} leverages pretrained language or CV models for time series analysis firstly and achieves excellent performance in all main time series analysis tasks. Overall, the Transformer architecture is widely regarded as one of the most effective and promising approaches for MTS forecasting (wen et al., 2022\cite{Wen2022transformers}; shao et al., 2023 \cite{Shao2023exploring}).


\subsection{Distribution shift} 

Although various models above make breakthroughs in time-series forecasting, they often encounter challenges when dealing with non-stationary time-series data, where the distribution of the data changes over time. To address this issue, domain adaptation (Tzeng et al., 2017 \cite{Tzeng17Domain_Adaptation}; Ganin et al., 2016 \cite{Ganin16domain_adaptation}; Wang et al., 2018 \cite{Wang18Domain_Adaptation}) and domain generalization (Wang et al., 2021 \cite{Wang2021GeneralizingTU}; Li et al., 2018\cite{Li18DomainGeneralization}; Muandet et al., 2013 \cite{pmlr-v28-muandet13}; Lu et al., 2022 \cite{Lu2022DomaininvariantFE}) approaches are commonly employed to mitigate the distribution shift. Domain adaptation algorithms aim to reduce the distribution gap between the source and target domains, while domain generalization algorithms solely rely on the source domain and aim to generalize to the target domain. 
However, defining a domain becomes challenging in the context of non-stationary time series, as the data distribution shifts over time. Recently, Du et al. (Du et al., 2021) proposed the use of Adaptive RNNs to address the distribution shift issues in non-stationary time-series data,  characterizing the distribution information by dividing the training data into periods and then matches the distributions of these identified periods to generalize the model. RevIN (Kim et al. 2022) \cite{reversible} utilizes a generally applicable normalization-and-denormalization method with learnable affine transformation to address the distribution shift problem. DIVERSIFY (Lu et al. 2023) \cite{lu2023outofdistribution} trys to learn the out of-distribution (OOD) representation on dynamic distributions of times series and then bridges the gap between these latent distributions.



\subsection{Vector Quantization}

Vector quantization (VQ) is a widely used compression technique in signal and image processing, which aims to learn a discrete latent representation by clustering multidimensional data into a finite set of representations. VQ-VAE (Van Den Oord et al., 2017)\cite{VQVAE} proposes to combine the VQ strategy with a variational autoencoder. There are two key differences between this approach and VAEs: first, the encoder network produces discrete codes instead of continuous ones to obtain a compressed discrete latent space; second, the prior is learned rather than being static; which make it capable of modelling very long term dependencies. SoundStream(Zeghidour et al., 2021) \cite{residualVQ} proposes the residual VQ and employs multiple vector quantizers to iteratively quantize the residuals of the waveform.VQ has also been combined with adversarial learning to synthesize high-resolution images, for example, VQGAN (Esser et al., 2021)\cite{VQGAN}. Subsequently, ViT-VQGAN(Yu et al., 2022)\cite{VQGAN_use_cosine_sim} propose to reduce the dimensionality of the codebook and l2-normalize the codebook and TE-VQGAN(Shin et al., 2023)\cite{orthogonal} incorporate a regularization term into the loss function to enforce orthogonality among the codebook embeddings. Considering veiwing time series as several discrete tokens may be potentially useful, our framework uniquely leverages VQ to enhance the capabilities of transformers in time series forecasting.

%end color blue
%}

%\subsection{Modeling both local and global context} 
%The receptive field of a CNN is restricted by the size of the convolutional kernel, making it more suitable for local information modeling. On the other hand, Self-Attention (SA) computes attention weights for each position with respect to all positions, effectively taking into account the relationships between each point. Consequently, SA appears more appropriate for global modeling. However, point-wise representation might inhibit the model from summarizing a long historical signal, and long input SA may be prone to overfitting.

%In order to capture both global and local information and model more granular information effectively, an increasing number of research works have adopted a hybrid approach by combining these two structures. MUSE~\cite{zhao2019muse} investigates the integration of convolution and self-attention mechanisms to enable the learning of sequence representations that incorporate multiple scales. T2VLAD~\cite{WangZ021} designs an efficient global-local alignment method to search relevant video contents based on natural language descriptions. VOLO~\cite{yuan2022volo} not only focuses on global modeling at a coarse level, but also efficiently encodes finer-level features and contexts into token. In the field of time series forecasting, MICN~\cite{wang2023micn} proposes a local-global structure to implement information aggregation and long-term dependency modeling for time series, but both local information and global information are obtained through convolutional neural networks (CNNs), and two structures are composed in a serial manner.



% }


% \section{Time Series Representation in Legendre-Fourier Domain} \label{sec:theoretical}

% \subsection{Legendre Projection}
%  Given an input sequence, the function approximation problem aims to approximate the cumulative history at every time $t$. Using Legendre Polynomials projection, we can project a prolonged sequence of data onto a subspace of bounded dimension, leading to compression, or feature representation, for evolving historical data. Formally, given a smooth function $f$ observed online, we aim to maintain a fixed size compressed representation of its history $f(x)_{[t-\theta,t]}$, where $\theta$ specifies the window size. At every time point $t$, the approximation function $g^{(t)}(x)$ is defined with respect to the measure $\mu^{(t)} =\frac{1}{\theta}\mathbbm{I}_{[t-\theta,t]}(x)$. In this paper, we use Legendre Polynomials of degree at most $N-1$ to build the function $g^{(t)}(x)$, i.e.
%   \begin{align}
%   g^{(t)}(x)=\sum_{n=1}^N c_{n}(t) P_{n}\left(\frac{2(x-t)}{\theta}+1\right), \label{eq:1}
%  \end{align}
%  where $P_n(\cdot)$ is the $n$-th order Legendre Polynomials. Coefficients $c_{n}(t)$ are captured by the following dynamic equation:
% \begin{align}%\notag
%  \frac{d}{d t} c(t) &=-\frac{1}{\theta} A c(t)+\frac{1}{\theta} B f(t).
% \end{align}
% where the definition of $A$ and $B$ can be found in~\cite{LMU}. Using Legendre Polynomials as a basis allows us to accurately approximate smooth functions, as indicated by the following theorem.

% \begin{theorem} [\it Similar to Proposition 6 in \cite{Hippo}]
%  If $f(x)$ is $L$-Lipschitz, then $\|f_{[t-\theta,t]}(x)-g^{(t)}(x)\|_{\mu^{(t)}}\le \mathcal{O}(\theta L/\sqrt{N})$. Moreover, if $f(x)$ has $k$-th order bounded derivatives, we have $\|f_{[t-\theta,t]}(x)-g^{(t)}(x)\|_{\mu^{(t)}}\le \mathcal{O}(\theta^kN^{-k+1/2})$.
% \end{theorem}
% According to Theorem 1, without any surprise, the larger the number of Legendre Polynomials basis, the more accurate the approximation will be, which unfortunately may lead to the overfitting of noisy signals in history. As shown in Section \ref{sec_exp}, directly feeding deep learning modules, such as MLP, RNN, and vanilla Attention without modification, with the above features will not yield state-of-the-art performance, primarily due to the noisy signals in history. That is why we introduce, in the following subsection, a Frequency Enhanced Layer with Fourier transforms for feature selection.  

% %The above theorem implies that if we pick proper $N$, the $g^(t)(x)$ function will be good enough to memorize the function $f_{[t-\theta, t]}(x)$ and we could use coefficient of $c_n(t)$ of $g^{(t)}(x)$ as the proper representation for the time series.

% Before we close this subsection, we note that unlike~\cite{S4}, a fixed window size is used for function approximation and feature extraction. This is because a longer history of data may lead to a larger accumulation of noises from history. To make it precise, we consider an auto-regressive setting with random noise. Let $\{x_t\}\in \mathbbm{R}^d$ be the time sequence with $x_{t+1} = Ax_t + b + \epsilon_t$ for $t=1,2,...$, where $A\in\mathbbm{R}^{d\times d}$, $b \in \mathbbm{R}^d$, and $\epsilon_t\in\mathbbm{R}^{d}$ is random noise sampled from $N(0, {\sigma^2 I})$. As indicated by the following theorem, given $x_t$, the noise will accumulate in $x_{t-\theta}$ over time at the rate of $\sqrt{\theta}$, where $\theta$ is the window size.

% \begin{theorem}
% Let $A$ be an unitary matrix and $\epsilon_t$ be $\sigma^2$-subgaussian random noise.  We have $x_{t} = A^{\theta}x_{t-\theta} + \sum_{i=1}^{\theta-1}A^{i}b + \mathcal{O}(\sigma \sqrt{\theta})$.
% \end{theorem}
 

% \subsection{Fourier Transform}
% % {\color{red} (TODO: to be finished??)} \Xue{(Sure, will try to finish it today or tomorrow...)}
% % $$x_{t+1} = Ax_t + b =  (A^{n-1}+A^{n-2}+...+I)bx_0 + O(b)$$
% % $$x_{t+1} = Ax_t + b +\epsilon_t = (A^{n-1}+A^{n-2}+...+I)bx_0 +O(b) + \sum \epsilon_t = O(\sqrt{T}\log T)$$
% Because white noise has a completely flat power spectrum, it is commonly believed that the time series data enjoys a particular spectral bias, which is not generally randomly distributed in the whole spectrum.
% % \Xue{(may need some references)}
% Due to the stochastic transition environment, the real output trajectories of the forecasting task contain large volatilization and people usually only predict the mean path of them. The relatively more smooth solutions thus are preferred. According to Eq.~\eqref{eq:1},  the approximation function $g^{(t)}(x)$ can be stabilized via smoothing the coefficients $c_n(t)$ in both $t$ and $n$. This observation helps us design an efficient data-driven way to tune the coefficients $c_n(t)$. As smoothing in $n$ can be simply implemented via multiplying learnable scalars to each channel, we mainly discuss smoothing $c_n(t)$ in $t$ via Fourier transformation. The spectral bias implies the spectrum of $c_n(t)$ mainly locates in the low-frequency regime and has weak signal strength in the high-frequency regime. To simplify our analysis, let us assume the Fourier coefficients of $c_{n}(t)$ as $a_{n}(t)$. Per spectral bias, we assume that there exists a $s, a_{\min}>0$, such that for all $n$ we have $t> s$, $|a_{n}(t)|\le a_{\min}$. An idea to sample coefficients is to keep the first $k$ dimensions and randomly sample the remaining dimensions instead of the fully random sampling strategy. We characterize the approximation quality via the following theorem:

% \begin{theorem}
% \label{thm_Fourier} 
% Let $A\in\mathbbm{R}^{d\times n}$ be the Fourier coefficients matrix of an input matrix $X\in\mathbbm{R}^{d\times n}$, and $\mu(A)$, the coherence measure of matrix $A$, is $\Omega(k/n)$. We assume there exist $s$ and  a positive $ a_{\min}$ such that the elements in last $d-s$ columns of $A$ is smaller than $a_{\min}$. If we keep the first $s$ columns selected and randomly choose $\mathcal{O}(k^2/\epsilon^2 - s)$ columns from the remaining parts, with high probability
% \[
%     \|A - P(A)\|_F \leq \mathcal{O}\left[(1 + \epsilon)a_{\min}\cdot\sqrt{(n-s)d}\right],
% \]
% where  $P(A)$ denotes the matrix projecting $A$ onto the column selected column space.
% \end{theorem}
% Theorem~\ref{thm_Fourier} implies that when $a_{\min}$ is small enough, the selected space can be considered almost the same as the original one.

==> sections/2_related_work_concise.tex <==
\begin{figure*}[t]
\centering
%\setlength{\abovecaptionskip}{0.2cm}
% \scalebox{0.70}{
\includegraphics[width=0.85\linewidth]{graphs_vq/SVQ.png}
\vskip -0.1in
\caption{Sparse-VQ Block(SVQ).}
\label{fig:SVQ}
% \vskip -0.2in
\end{figure*}

\begin{figure*}[t]
\centering
%\setlength{\abovecaptionskip}{0.2cm}
%\scalebox{0.80}{
\includegraphics[width=0.85\linewidth]{graphs_vq/model.png}
\vskip -0.1in
\caption{Classic model with incorporation of VQ(left) and Sparse-VQ Model Overview(right). $\mu_x$ and $\sigma_x$ represent the mean and variance of the data, which are used in the RevIN method.}
\label{fig:model_structure}
\vskip -0.1in
\end{figure*}

\section{Related Work}
\label{sec_related_works_concise}
In light of space constraints, here we present a concise summary of related work on time series forecasting, distribution shift, and vector quantization.% For a more detailed review, please refer to Appendix \ref{sec_appendix_related_works}.

\subsection{Time Series Forecasting}
Time series forecasting has progressed from traditional statistical algorithms like ARIMA~\cite{box_arima2} and Holt-Winter~\cite{Holt-Winter18} to machine learning models including DeepAR~\cite{DBLP:journals/corr/FlunkertSG17-deepAR} and Prophet~\cite{Taylor2018ForecastingAS}. The advent of deep learning has led to the adoption of sophisticated neural networks such as TCN~\cite{TCN} and LSTM~\cite{hochreiter_long_1997_lstm}, with notable contributions from N-BEATS~\cite{nbeats}, which excelled in the M4 competition. Transformer-based models, including Informer~\cite{haoyietal-informer-2021}, Reformer~\cite{KitaevKL20-reformer}, and Autoformer~\cite{Autoformer}, have significantly improved time series forecasting. Innovations like TimesNet~\cite{TIMESNET}, FiLM~\cite{zhou2022film}, FEDformer~\cite{FedFormer}, and Pyraformer~\cite{liu2022pyraformer} continue to refine these techniques. Pretrained models such as FPT~\cite{zhou2023onefitsall} showcase the adaptability of language or vision models to time series tasks, cementing Transformer-based methods as a top-tier approach~\cite{Wen2022transformers, Shao2023exploring}.

\subsection{Distribution Shift}
Addressing distribution shifts in non-stationary time series data is a persistent challenge. To tackle this issue, researchers mainly utilize domain adaptation~\cite{Tzeng17Domain_Adaptation, Ganin16domain_adaptation, Wang18Domain_Adaptation} and generalization strategies~\cite{Wang2021GeneralizingTU, Li18DomainGeneralization, pmlr-v28-muandet13, Lu2022DomaininvariantFE} to mitigate the distribution shift. Adaptive RNNs~\cite{Du2021AdaRNNAL}, RevIN~\cite{reversible}, and DIVERSIFY~\cite{lu2023outofdistribution} have emerged as novel solutions, leveraging period segmentation, normalization techniques, and out-of-distribution learning to cope with varying distributions.

\subsection{Vector Quantization}
Vector quantization (VQ) has been a key compression strategy in signal and image processing, with VQ-VAE~\cite{VQVAE} combining it with variational autoencoders for discrete and learnable priors. Developments such as SoundStream's residual VQ~\cite{residualVQ}, VQGAN~\cite{VQGAN}, and its extensions ViT-VQGAN~\cite{VQGAN_use_cosine_sim} and TE-VQGAN~\cite{orthogonal} have pushed VQ into new domains. Recent research has demonstrated the potential of applying Vector Quantization (VQ) to time series forecasting~\cite{Rasul2022VQARVQ}. However, our comprehensive study suggests that the conventional approach of pre-quantization may not enhance performance. Instead, implementing Vector Quantization after the enrichment of the signal by the encoder proves to be more beneficial.

%Our framework leverages VQ to enhance transformer capabilities in time series forecasting, opening new avenues for discrete tokenization of series data.

==> sections/7_sparse_representation.tex <==
\section{Sparse VQ representation}
\label{sec:eff_sparse_reg}

To differentiate the performance of the sparse regression technique from that of the traditional cluster-based approach in quantization, we evaluate the minimal count of codewords, denoted by $N(\mathcal{U}, \epsilon)$, required to represent any vector within a unit sphere $\mathcal{U}$ with an approximation error smaller than $\epsilon$. The following proposition illustrates that with sparse regression, $N(\mathcal{U}, \epsilon)$ can be significantly reduced from $O(1/\epsilon^n)$ to $O(1/\epsilon^q)$, where $q \ll n$ for vectors in a high-dimensional space.

\begin{proposition}
\label{proposition}
For a cluster-based scheme, $N(\mathcal{U}, \epsilon)$ is no less than $1/\epsilon^n$, whereas for the sparse regression technique, $N(\mathcal{U},\epsilon)$ has an upper bound of $(4n/\epsilon)^q$, where
\[
q \geq \max\left(3, \frac{\log(4/\epsilon)}{\log\log(2n/\eta)}\right),
\]
provided that the count of non-zero coefficients used in sparse regression is at least
\[
    \frac{4n}{\epsilon \left(\log K + q\log (4n) - (q+1)\log \epsilon \right)}.
\]
\end{proposition}

\begin{proof}
\renewcommand{\qedsymbol}{}
To establish an upper limit for $N(\mathcal{U}, \epsilon)$ using clustering, the covering number for a unit sphere $\mathcal{U}$ is considered, which necessitates at least $1/\epsilon^n$ codewords for approximate representation within an error of $\epsilon$. Let $Vf$, where $V = (v_1, \ldots, v_l)$, $v_j \sim \mathcal{N}(0, I_n/l)$, and $f \in \Omega_t$ is a $t$-sparse unit vector. We have:
\[
\Pr\left(\|VV^{\top} - I\|_2 \geq \lambda \right) \leq 2n\exp\left(-\frac{l\lambda^2}{3n}\right),
\]
which implies
\[
\|VV^{\top} - I\|_2 \leq \Gamma := \sqrt{\frac{n}{l}\log\frac{2n}{\eta}}
\]
with a probability of at least $1 - \eta$. Consequently, $\|f' - f\|_2 \geq (1+\Gamma)^{-1} \|Vf - Vf'\|_2$. Given the $t$-sparse unit vector covering number is capped by $(Dl/t\epsilon)^t$, we deduce:
\[
\left(\frac{Dl}{t\epsilon}\right)^t \geq \left(1 + \frac{2}{\epsilon}\right)^n(1+\Gamma)^n,
\]
Selecting $l = (4n/\epsilon)^q$ ensures:
\[
(1+\Gamma)^n \leq \exp\left(n\Gamma\right) \leq e,
\]
which results in $t\log(D'l/\epsilon) \geq 2n/\epsilon + t\log t$, with $D' = De$. 
With the assumption that $t \geq 4n/[\epsilon(\log K + q\log(4n) - (q+1)\log\epsilon)]$, it holds that $t\log t \leq 2n/\epsilon$, thereby concluding that $l \geq (4n/\epsilon)^q$.
\end{proof}

%Due to the space limitation, we postpone the proof in Appendix~\ref{app:proof}. 

%%%Due to page constraints, the proof has been relegated to Appendix~\ref{app:proof}, which elaborates on the derivation based on the work ~\cite{chen2023svq}.




==> tables/full_bench_multi.tex <==
%\resizebox{!}{\.5\paperheight}{
% \vskip -0.2in
\begin{table*}[h]
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{multivariate long-term series forecasting results on six datasets with various input length and prediction length $O \in \{96,192,336,720\}$ (For ILI dataset, we set prediction length $O \in \{24,36,48,60\}$). A lower MSE indicates better performance. All experiments are repeated 5 times.}\vspace{-1mm}
\scalebox{0.60}{
\begin{tabular}{c|c|cccccccccccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FiLM}&\multicolumn{2}{c|}{FEDformer}&\multicolumn{2}{c|}{Autoformer}&\multicolumn{2}{c|}{S4}&\multicolumn{2}{c|}{Informer}&\multicolumn{2}{c|}{LogTrans}&\multicolumn{2}{c}{Reformer}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTm2$}} &96 & \textbf{0.165} & \textbf{0.256} &0.203 &0.287 &0.255  &0.339 &0.705 &0.690 &0.365  &0.453  &0.768  &0.642  &0.658  &0.619    \\
                        & 192 & \textbf{0.222} & \textbf{0.296} &0.269  &0.328  &0.281 &0.340 &0.924 &0.692 &0.533  &0.563  &0.989  &0.757  &1.078  &0.827    \\
                        & 336 & \textbf{0.277} & \textbf{0.333} & 0.325 &0.366 &0.339  &0.372 &1.364 &0.877 &1.363&0.887  &1.334  &0.872  &1.549  &0.972     \\
                        & 720 & \textbf{0.371} & \textbf{0.389} &0.421 &0.415 &0.422  &0.419 &0.877 &1.074 &3.379  &1.338 & 3.048 &1.328  &2.631  &1.242      \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Electricity$}} &96  &\textbf{0.154}  &\textbf{0.267}  &0.183 &0.297 &0.201  &0.317 &0.304 &0.405 &0.274  &0.368  &0.258  &0.357  &0.312  &0.402    \\
                        & 192 &\textbf{0.164} & \textbf{0.258} & 0.195 &0.308 &0.222  &0.334 &0.313 &0.413 &0.296 &0.386  &0.266 &0.368  &0.348  &0.433    \\
                        & 336 & \textbf{0.188} & \textbf{0.283} &0.212 &0.313 &0.231 &0.338 &0.290 &0.381 &0.300  &0.394  &0.280 &0.380  &0.350  & 0.433    \\
                        & 720 & 0.236 & \textbf{0.332} &\textbf{0.231} &0.343 &0.254  &0.361 &0.262 &0.344 &0.373  &0.439 &0.283  &0.376  &0.340  &0.420     \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Exchange$}} &96  & \textbf{0.086} & \textbf{0.204} &0.139 &0.276 &0.197  &0.323 &1.292 &0.849 &0.847  &0.752  &0.968  &0.812  &1.065  &0.829    \\
                        & 192 & \textbf{0.188} & \textbf{0.292} &0.256 &0.369 &0.300  &0.369 &1.631 &0.968 &1.204   &0.895 &1.040  &0.851  &1.188  & 0.906   \\
                        & 336 & \textbf{0.356} & \textbf{0.433} &0.426 &0.464 &0.509  &0.524 &2.225 &1.145 &1.672  &1.036  &1.659  &1.081  &1.357  &0.976     \\
                        & 720 & \textbf{0.727} & \textbf{0.669} &1.090 &0.800 &1.447  &0.941 &2.521 &1.245 &2.478  &1.310  &1.941  &1.127  &1.510  &1.016     \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Traffic$}} &96  &\textbf{0.416}& \textbf{0.294} &0.562 &0.349 &0.613  &0.388 &0.824 &0.514 &0.719  &0.391  &0.684  &0.384  &0.732  &0.423    \\
                        & 192 & \textbf{0.408} & \textbf{0.288} &0.562 &0.346 &0.616&0.382 &1.106 &0.672 &0.696 &0.379  &0.685  &0.390  &0.733  &0.420    \\
                        & 336 & \textbf{0.425} & \textbf{0.298} &0.570 &0.323 &0.622  &0.337 &1.084 &0.627 &0.777  &0.420  &0.733  &0.408  &0.742  &0.420     \\
                        & 720 & \textbf{0.520} &\textbf{0.353} &0.596 &0.368 &0.660  &0.408 &1.536 &0.845 &0.864  &0.472  &0.717  &0.396  &0.755  &0.423     \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Weather$}} & 96 & \textbf{0.199} & \textbf{0.262} &0.217  &0.296  &0.266  &0.336 &0.406 &0.444 &0.300  &0.384  &0.458  &0.490  &0.689  &0.596    \\
                        & 192 & \textbf{0.228} & \textbf{0.288} &0.276  &0.336  &0.307  &0.367 &0.525 &0.527 &0.598  &0.544  &0.658  &0.589  &0.752  &0.638    \\
                        & 336 &\textbf{0.267} &\textbf{0.323} & 0.339  &0.380  &0.359  &0.395 &0.531 &0.539 &0.578  &0.523  &0.797  &0.652  &0.639  &0.596    \\
                        & 720 &\textbf{0.319} & \textbf{0.361} &0.403  &0.428 &0.578 &0.578 &0.419  &0.428  &1.059  &0.741  &0.869  &0.675  &1.130  &0.792    \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ILI$}} & 24 & \textbf{1.970} & \textbf{0.875} &2.203  &0.963  &3.483 &1.287 &4.631 &1.484 &5.764  &1.677  &4.480  &1.444  &4.400 &1.382    \\
                        & 36 & \textbf{1.982} & \textbf{0.859} &2.272  &0.976  &3.103  &1.148 &4.123 &1.348 &4.755  &1.467  &4.799  &1.467  &4.783  &1.448    \\
                        & 48 & \textbf{1.868} & \textbf{0.896} &2.209  &0.981  &2.669  &1.085 &4.066 &1.36 &4.763  &1.469  &4.800  &1.468  &4.832  &1.465    \\
                        & 60 & \textbf{2.057} & \textbf{0.929} &2.545  &1.061  &2.770  &1.125 &4.278 &1.41 &5.264  &1.564  &5.278  &1.560  &4.882  &1.483    \\
\bottomrule
\end{tabular}
\label{tab:multi-benchmarks}
}
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
%}

==> tables/full_bench_uni.tex <==
\begin{table*}[h]
% \begin{adjustwidth}{-1.5in}{-1in}
\centering
%\begin{small}
\caption{Univariate long-term forecasting results on six datasets with various input length and prediction horizon $O \in \{96,192,336,720\}$. A lower MSE indicates better performance. All experiments are repeated 5 times.}
\vskip 0.05in
\scalebox{0.60}{
\begin{tabular}{c|c|cccccccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FiLM}&\multicolumn{2}{c|}{FEDformer}&\multicolumn{2}{c|}{Autoformer}&\multicolumn{2}{c|}{S4}&\multicolumn{2}{c|}{Informer}&\multicolumn{2}{c|}{LogTrans}&\multicolumn{2}{c}{Reformer}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTm2$}} 
& 96 & 0.065 &\textbf{0.189}  &\textbf{0.063} &0.189 & 0.065 & 0.189 &0.153 &0.318 & 0.088 & 0.225 & 0.075 & 0.208 & 0.076  &0.214   \\
& 192 & \textbf{0.094} & \textbf{0.233} &0.102 &0.245 & 0.118 & 0.256 &0.183 &0.350 & 0.132 &0.283 & 0.129 &0.275  & 0.132  & 0.290   \\
& 336 & \textbf{0.124} & \textbf{0.274} &0.130 &0.279 & 0.154 & 0.305 &0.204 & 0.367 &0.180 &0.336 & 0.154 &0.302  & 0.160  & 0.312    \\
& 720 & \textbf{0.173} & \textbf{0.323} &0.178 &0.325 & 0.182 &0.335 &0.482 &0.567  &0.300  &0.435 & 0.160 &0.321  & 0.168  &0.335     \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Electricity$}} 
& 96  & \textbf{0.154} & \textbf{0.247} &0.253 &0.370  &0.341 &0.438 &0.351 &0.452 & 0.484& 0.538 &0.288& 0.393& 0.274 & 0.379   \\
& 192 & \textbf{0.166} & \textbf{0.258} &0.282 &0.386 &0.345 &0.428 &0.373 &0.455 & 0.557& 0.558 &0.432 & 0.483 & 0.304 &0.402   \\
& 336 & \textbf{0.188} & \textbf{0.283} &0.346 &0.431 &0.406 &0.470 &0.408 &0.477 & 0.636& 0.613 &0.430 &0.483 & 0.370 &0.448  \\
& 720 & \textbf{0.249} & \textbf{0.341} &0.422 &0.484 &0.565 &0.581 &0.472 &0.517 & 0.819& 0.682 &0.491 &0.531 & 0.460 &0.511   \\
\midrule

\multirow{4}{*}{\rotatebox{90}{$Exchange$}} 
&96  & \textbf{0.110} & \textbf{0.259} &0.131 &0.284 & 0.241 & 0.387 &0.344 &0.482  & 0.591  &0.615  &0.237 &0.377  &0.298  &0.444    \\
& 192 & \textbf{0.207} & \textbf{0.352} &0.277 &0.420 &0.300  &0.369 &0.362 &0.494  &1.183   &0.912 &0.738  &0.619  &0.777  & 0.719   \\
& 336 & \textbf{0.327} & \textbf{0.461} &0.426 &0.511 &0.509  &0.524 &0.499 &0.594  &1.367  &0.984  &2.018  &1.070  &1.832  &1.128     \\
& 720 & \textbf{0.811} & \textbf{0.708} &1.162 &0.832 &1.260  &0.867 &0.552 & 0.614 &1.872  &1.072  &2.405  &1.175  &1.203  &0.956     \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Traffic$}} 
&96  & \textbf{0.144} & \textbf{0.215} &0.170 &0.263  &0.246 &0.346 &0.194 &0.290 & 0.257 & 0.353 &0.226 &0.317 &  0.313 & 0.383\\
& 192 & \textbf{0.120} & \textbf{0.199} &0.173 &0.265 &0.266 &0.370 &0.172 &0.272 & 0.299 & 0.376 &0.314 &0.408 & 0.386 & 0.453\\
& 336 & \textbf{0.128} & \textbf{0.212} &0.178 &0.266 &0.263 &0.371 &0.178 &0.278 & 0.312 & 0.387 &0.387 &0.453 & 0.423 & 0.468\\
& 720 & \textbf{0.153} & \textbf{0.252} &0.187 &0.286 &0.269 &0.372 &0.263 &0.386 & 0.366 & 0.436 &0.491 &0.437 & 0.378 & 0.433\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Weather$}}
& 96  & \textbf{0.0012} & \textbf{0.026} & 0.0035 & 0.046 & 0.011 &0.081 &0.0061 &0.065 & 0.0038 & 0.044 & 0.0046 &0.052 & 0.012 & 0.087 \\
& 192 & \textbf{0.0014}& \textbf{0.029}&0.0054 &0.059 &0.0075 &0.067 &0.0067 &0.067 & 0.0023 & 0.040 &0.0056 & 0.060 & 0.0098 & 0.079  \\
& 336 & \textbf{0.0015} & \textbf{0.030} &0.0041 &0.050 &0.0063 &0.062 &0.0025 &0.0381 & 0.0041 & 0.049 &0.0060 &0.054& 0.0050 & 0.059 \\
& 720 & \textbf{0.0022} & \textbf{0.037} &0.015 &0.091 &0.0085 &0.070 &0.0074 &0.0736 & 0.0031 & 0.042 &0.0071 &0.063& 0.0041 & 0.049 \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ILI$}} 
& 24 & \textbf{0.629} & \textbf{0.538} &0.693 &0.629 &0.948 &0.732 &0.866 &0.584 & 5.282 &2.050 &3.607 & 1.662 & 3.838 & 1.720  \\
& 36 & \textbf{0.444} & \textbf{0.481} &0.554 &0.604 &0.634 &0.650 &0.622 &0.532 & 4.554 &1.916 &2.407 & 1.363 & 2.934 & 1.520 \\
& 48 & \textbf{0.557} & \textbf{0.584} &0.699 &0.696 &0.791 &0.752 &0.813 &0.679 & 4.273 &1.846 &3.106 & 1.575 & 3.754 & 1.749\\
& 60 & \textbf{0.641} & \textbf{0.644} &0.828 &0.770 &0.874 &0.797 &0.931 &0.747 & 5.214 &2.057 &3.698 & 1.733 & 4.162 & 1.847\\
\bottomrule
\end{tabular}
}
\label{tab:uni-benchmarks-large}
\vskip -0.10in
% \end{adjustwidth}
%\end{small}tab:multi-benchmarks
\end{table*}


==> tables/ks_test_small.tex <==

\begin{table}[h]
%\setlength{\uppercaptionskip}{0.pt}
%\setlength{\belowcaptionskip}{-0.pt}
%\vskip 0.15in
\centering
% \setlength{\belowcaptionskip}{2pt} 
\caption{P-values of Kolmogrov-Smirnov test of different Transformer models for long-term forecasting output on ETTm1 and ETTm2 dataset. Larger value indicates the hypothesis (the input sequence and forecasting output come from the same distribution) is less likely to be rejected. The largest results are highlighted.}
\begin{small}
% \begin{sc}
\vskip 0.05in
\scalebox{0.80}{
\begin{tabular}{c|c|cccccc}
\toprule
\multicolumn{2}{c|}{Methods}&Transformer&Informer&Autoformer&FEDformer&FiLM&True\\ %&\multicolumn{2}{c|}{Fedformer-f }\\%&\multicolumn{2}{c|}{}&\\
\midrule
\multirow{4}{*}{\rotatebox{90}{ETTm1}} 
& 96 & 0.0090 & 0.0055&0.020 & \textbf{0.048} & 0.016& {0.023} \\
& 192 & 0.0052 & 0.0029&0.015 & \textbf{0.028} & 0.0123& {0.013} \\
& 336 & 0.0022 & 0.0019&0.012 & \textbf{0.015} & 0.0046& {0.010} \\
% & 720 & 0.0023 & 0.0016 & \textbf{0.014} & \textbf{0.0036} \\
& 720 & 0.0023 & 0.0016&0.008 & \textbf{0.014} & 0.0024& {0.004} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{ETTm2}} 
% & 48 & 0.454 & & 0.366 & & 0.476 & & 0.356 \\
& 96 & 0.0012 & 0.0008& \textbf{0.079} &{0.071} & 0.022 & {0.087} \\%& \textbf{0.379} & \textbf{0.419}\\
& 192 & 0.0011 & 0.0006& \textbf{0.047} &{0.045}  &0.020 & {0.060} \\%& \textbf{0.426} & \textbf{0.441}\\
% & 288 & 0.634 & & 0.430 & & 0.571 & & 0.379 \\
& 336 & 0.0005 & 0.00009& 0.027 &\textbf{0.028} &0.012 & {0.042} \\%& \textbf{0.445} & \textbf{0.459}\\
% & 672 & 0.606 & & 0.528 & & 0.544 & & 0.501\\
& 720 & 0.0008& 0.0002& \textbf{0.023} & {0.021} &0.0081 & {0.023} \\
% \multicolumn{2}{c|}{Count}& 0 & 0 & 3 & 5 & 7& NA \\
%& \textbf{0.543} & \textbf{0.490}\\
%& -96 & 0.0012 & 0.0009 & 0.0001 & 0.0037 & \textbf{0.039} & \textbf{0.012} \\
\bottomrule
\end{tabular}
}
\label{tab:KStest_small}
% \end{sc}
\end{small}
%\end{center}
\vskip -0.1in
\end{table}




==> tables/tab_LPU_boosting.tex <==
%\resizebox{!}{\.5\paperheight}{
\vskip -0.1in
% \begin{wraptable}

% \begin{wraptable}[12]{r}{0.7\textwidth}
\begin{table*}[h]
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Boosting effect of LPU layer for common deep learning backbones: MLP, LSTM, CNN and Attention.`+` indicates degraded performance.}\vspace{-1mm}
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccccccccccccc}
%\begin{tabular}{c|c|cccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FEL}&\multicolumn{2}{c|}{MLP}&\multicolumn{2}{c|}{LSTM}&\multicolumn{2}{c|}{lagged-LSTM}&\multicolumn{2}{c|}{CNN}&\multicolumn{2}{c}{Attention}\\
\midrule
% \multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE&\\
\multicolumn{2}{c|}{Compare} & LPU  & Linear& LPU  & Linear & LPU  & Linear & LPU  & Linear & LPU  & Linear & LPU  & Linear\\
\midrule

\multirow{4}{*}{\rotatebox{90}{ETTm1}} 

&96  &\textbf{0.030}  & +38\%   & 0.034  & +8.0\%  & 0.049 & +73\% & 0.093 & -21\% & 0.116   & -50\%   & 0.243  & -81\% \\
& 192  &\textbf{0.047} & +9.5\% & 0.049  & +30\%  & 0.174 & +32\% & 0.331 & -48\% & 0.101   & +20\%    & 0.387  & -86\% \\
& 336 & \textbf{0.063} & +5.8\% & 0.061  & +64\%  & 0.119 & +84\% & 0.214 & -19\% & 0.122   & +25\%    & 1.652  & +12\% \\
& 720 &\textbf{0.081} & +1.4\%  & 0.082  & +62\%  & 0.184 & +32\% & 0.303 & -6.5\%  & 0.108   & +13\%    & 4.782  & -61\% \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Electricity}} 
% &96  &\textbf{0.213}  &\textbf{0.328}  &+15\%  & +6.8\% & +11\% & +5.2\%  & +11\%    & +5.2\% & +11\% & +4.8\%  &--& -- & +136\% & +58\%  \\
% & 192 &\textbf{0.268} & \textbf{0.373} &-4.6\% & -3.8\% & +7.8\%  & +3.9\%   & +6.8\%    & +3.5\% & -5.3\% & -3.9\%  &--& --  & +32\%  & +16\% \\
% & 336 & \textbf{0.307}& \textbf{0.417}&-4.2\%  & -5.0\% & -3.9\%  & -6.0\%   & -7.2\%    & -8.0\%   & -8.5\% & -9.0\%   &--& -- & +0.1\% & -5.0\% \\
% & 720 & \textbf{0.321}&\textbf{0.423} &+2.9\%  & +2.8\% & +10\%  &  +6.8\%  & +3.0\%   & +1.7\%  & +207\% & +85\%      &--& --  & 37\%  & 22\% \\

&96  &\textbf{0.213}  & +136\%  & 0.431  & +121\%   & 0.291 & +55.6\% & 0.739 & -33\% & 0.310  & +43\%  & 0.805 & +23\% \\%&--& --
& 192 &\textbf{0.268} & +32\%   & 0.291 & +239\%   & 0.353  & +17\% & 0.535 & +15\% & 0.380  & +12\%  & 0.938 & +14\% \\%&--& --  \\
& 336 & \textbf{0.307}& +0.1\%  & 0.296 & +235\%   & 0.436  & -6.7\% & 0.517 & +23\% & 0.359  & +29\% & 2.043 & -54\% & \\%&--& -- \\
& 720 & \textbf{0.321}& +37\%   & 0.339 & +196\%   & 0.636  & -11\% & 0.492 & +28\% & 0.424  & +18\%  & 9.115 & +298\% \\ %&--& --  \\
 
\bottomrule
\end{tabular}
\label{tab:boosting}
}
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
% \end{wraptable}
%}

==> tables/tab_LPU_boosting_full.tex <==
%\resizebox{!}{\.5\paperheight}{
\vskip -0.1in
% \begin{wraptable}

%\begin{wraptable}[12]{r}{0.7\textwidth}
\begin{table*}[h]
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{(Full Benchmark) Boosting effect of LPU layer for common deep learning backbones: MLP, LSTM, CNN and Attention.`+` indicates degraded performance.}\vspace{-1mm}
\scalebox{0.80}{
\begin{tabular}{c|c|cccccccccccccccccc}
%\begin{tabular}{c|c|cccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FEL}&\multicolumn{2}{c|}{MLP}&\multicolumn{2}{c|}{LSTM}&\multicolumn{2}{c|}{lagged-LSTM}&\multicolumn{2}{c|}{CNN}&\multicolumn{2}{c}{Attention}\\
\midrule
% \multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE&\\
\multicolumn{2}{c|}{Compare} & LPU  & Linear& LPU  & Linear & LPU  & Linear & LPU  & Linear & LPU  & Linear & LPU  & Linear\\
\midrule

\multirow{4}{*}{\rotatebox{90}{ETTm1}} 

&96  &\textbf{0.030}  & +38\%   & 0.034  & +8.0\%  & 0.049 & +73\% & 0.093 & -21\% & 0.116   & -50\%   & 0.243  & -81\% \\
& 192  &\textbf{0.047} & +9.5\% & 0.049  & +30\%  & 0.174 & +32\% & 0.331 & -48\% & 0.101   & +20\%    & 0.387  & -86\% \\
& 336 & 0.063 & +5.8\% & \textbf{0.061}  & +64\%  & 0.119 & +84\% & 0.214 & -19\% & 0.122   & +25\%    & 1.652  & +12\% \\
& 720 &\textbf{0.081} & +1.4\%  & 0.082  & +62\%  & 0.184 & +32\% & 0.303 & -6.5\%  & 0.108   & +13\%    & 4.782  & -61\% \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Electricity}} 

&96  &\textbf{0.213}  & +136\%  & 0.431  & +121\%   & 0.291 & +56\% & 0.739 & -33\% & 0.310  & +43\%  & 0.805 & +23\% \\%&--& --
& 192 &\textbf{0.268} & +32\%   & 0.291 & +239\%   & 0.353  & +17\% & 0.535 & +15\% & 0.380  & +12\%  & 0.938 & +14\% \\%&--& --  \\
& 336 & 0.307& +0.1\%  & \textbf{0.296} & +235\%   & 0.436  & -6.7\% & 0.517 & +23\% & 0.359  & +29\% & 2.043 & -54\% & \\%&--& -- \\
& 720 & \textbf{0.321}& +37\%   & 0.339 & +196\%   & 0.636  & -11\% & 0.492 & +28\% & 0.424  & +18\%  & 9.115 & +298\% \\ %&--& --  \\
               
\midrule
\multirow{4}{*}{\rotatebox{90}{$Exchange$}} 
& 96  & 0.130 & +7.5\% & \textbf{0.110} & -18\% & 0.224 & +6.0\% & 0.521 & -58\% & 0.244 & -18\% & 0.338 & +872\% \\
& 192 & \textbf{0.205} & +39\% & 0.257 & -36\% & 0.787 & -35\% & 1.742 & -66\% & 0.630 & +2.1\% & 0.930 & +278\% \\
& 336 & 0.467 & +9.2\% & \textbf{0.461} & -33\% & 0.964 & +24\% & 2.281 & -38\% & 3.231 & -85\% & 1.067 & +69\%\\
& 720 & \textbf{1.003} & +26\% & 1.981 & -61\% & 2.703 & -29\% & 1.457 & +34\% & 5.531 & +9.7\% & 0.631 & +1831\% \\
\midrule

\multirow{4}{*}{\rotatebox{90}{$Traffic$}} 
&96  &\textbf{0.312} & +18\% & 0.376 & +277\% & 0.215 & +1.2\% & 0.216 & +10\% & 0.543 & -33\% & 0.429 & +210\% \\
& 192 & \textbf{0.141} & +9.6\% & 0.199 & +598\% & 0.177 & +19\% & 0.186 & +17\% & 0.451 & +9.0\% & 0.476 & +176\% \\
& 336 & \textbf{0.143} & +2.5\% & 0.195 & +613\% & 0.192 & +19\% & 0.190 & +11\% & 0.346 & +44\% & 0.377 & +260\% \\
& 720 & \textbf{0.215} & +30\% & 0.240 & +475\% & 0.234 & -1.7\% & 0.250 & +15\% & 0.348 &  +47\% & 0.773 & +171\%\\
\midrule

\multirow{4}{*}{\rotatebox{90}{$Weather$}} 
& 96 & 0.0073 & -38\% & 0.006  & -33\% & 0.006 & -23\% & 0.0070 & -17\% & \textbf{0.0022} & +167\% & 0.0065 &-11\%\\
& 192 & 0.0106 & -64\% & 0.007 & -14\% & 0.0074 & -11\% & \textbf{0.0063} & -19\% & 0.007 & -24\% & 0.0075 & -12\%\\
& 336 & 0.0079 & -37\% & 0.006 & +4.9\% & 0.0056 & +12\% & \textbf{0.0055} & +12\% & 0.0056 & +0.5\% & 0.222 & -69\% \\
& 720 &0.0063 & +0.4\% & 0.006 & +7.6\% & \textbf{0.0062} & +5.3\% & 0.103 & -36\% &0.006 & +4.2\% & 0.037 & -81\% \\
                        
\midrule
\multirow{4}{*}{\rotatebox{90}{$ILI$}} 
& 24 & 1.393 &	+6.1\% & \textbf{1.220} & +36\% & 2.306 & +66\% & 4.189 & -9.2\% & 2.264 & -22\% & 2.249 & +217\% \\
& 36 & 1.242 & -22\% & \textbf{1.185} & +56\% & 2.950 & +44\% & 2.516 & +42\% & 1.841 & -3.0\% & 5.026 & +45\% \\
& 48 & 1.448 & -28\% & \textbf{1.079} & +79\% & 3.385 & +38\% & 3.501 & +16\% & 1.654 & +23\% & 2.838 & +115\% \\
& 60 & 2.089 & -18\% & \textbf{0.986} & +96\%  & 4.031 & +18\% & 4.258 & +10\% & 1.290 & +176\% & 4.978 & +250\% \\
\bottomrule
\end{tabular}
\label{tab:boosting}
}
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
%\end{wraptable}
%}


==> tables/tab_ablation_FEL.tex <==
%\resizebox{!}{\.5\paperheight}{
\begin{table*}[ht]
\vskip -0.05in
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Ablation studies of FEL layer. The FEL layer is replaced with 4 different variants: MLP, LSTM, CNN, and Transformer. S4 is also introduced as a variant. The experiments are performed on ETTm1 and Electricity. The metric of variants is presented in relative value (’+’ indicates degraded performance, ’-’ indicates improved performance).}\vspace{-1mm}
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccccccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FilM}&\multicolumn{2}{c|}{LPU+MLP}&\multicolumn{2}{c|}{LPU+LSTM}&\multicolumn{2}{c|}{LPU+CNN}&\multicolumn{2}{c|}{LPU+attention}&\multicolumn{2}{c}{S4}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE&\\
\midrule

\multirow{4}{*}{\rotatebox{90}{ETTm1}} 

&96  &\textbf{0.029} &\textbf{0.127}  &+0.0\%   & +0.0\%   & +12.1\% & +7.1\%    & +13.5\%   & +9.5\%   & +1.7\%  & +1.6\% &-- & -- \\
& 192  &\textbf{0.041} &\textbf{0.153}  &-1.5\% & -0.6\%  & +12.2\% & +8.5\%  & +10.8\%   & +7.8\%    & +2.0\%  & +3.3\% &-- & -- \\
& 336 & \textbf{0.053} & \textbf{0.175} &-1.7\% & -1.7\%  & +4.5\% & +4.0\%    & +10.8\%    & +6.3\%    & +4.5\% & +2.9\% &-- & --  \\
& 720 &\textbf{0.071}& \textbf{0.205}   &-0.9\%  & -1.0\%  & +5.5\% & +3.4\%  & +8.6\%    & +4.9\%    & +13.8\% & +7.8\% &-- & --  \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Electricity}} 

&96  &\textbf{0.154}  &\textbf{0.247}  &+155\%  & +81\%   & +160\% & +84\%    & +330\%  & +155\%  & +242\% & +119\% & 128\% & 83\% \\%&--& -- & \\
& 192 &\textbf{0.166} & \textbf{0.258} &+59\% & +39\%   & +121\%  & +67\%   & +224\%  & +117\%  & +264\% & +131\% & 124\% & 76\% \\%&--& --  \\
& 336 & \textbf{0.188}& \textbf{0.283} &+55\%  & +35\%   & +150\%  & +74\%   & +128\%  & +71\% & +183\% & +95\% & 117\% & 69\% \\%&--& -- \\
& 720 & \textbf{0.249}&\textbf{0.341}  &+33\%  & +25\%   & +154\%  & +73\%   & +192\%  & +95\%  & +312\% & +138\% & 89\% & 51\% \\ %&--& --  \\
                        
\bottomrule
\end{tabular}
\label{tab:ablation_FEL}
}
% \end{adjustwidth}
%\end{footnotesize}

\vskip -0.05in
\end{table*}
%}

==> tables/tab_ablation_FEL_full.tex <==
%\resizebox{!}{\.5\paperheight}{
\begin{table*}[!h]
\vskip -0.05in
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{: (Full Benchmark)Ablation studies of FEL layer. The FEL layer is replaced with 4 different variants: MLP, LSTM, CNN, and Transformer.The experiments are performed on ETTm1 and Electricity. The metric of variants is presented in relative value (’+’ indicates degraded performance, ’-’ indicates improved performance).}\vspace{-1mm}
\scalebox{0.8}{
\begin{tabular}{c|c|ccccccccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FilM}&\multicolumn{2}{c|}{LPU+MLP}&\multicolumn{2}{c|}{LPU+LSTM}&\multicolumn{2}{c|}{LPU+CNN}&\multicolumn{2}{c|}{LPU+attention}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& \\
\midrule

\multirow{4}{*}{\rotatebox{90}{ETTm1}} 

&96  &\textbf{0.029} &\textbf{0.127}  &+0.0\%   & +0.0\%   & +12.1\% & +7.1\%    & +13.5\%   & +9.5\%   & +1.7\%  & +1.6\%  \\
& 192  &\textbf{0.041} &\textbf{0.153}  &-1.5\% & -0.6\%  & +12.2\% & +8.5\%  & +10.8\%   & +7.8\%    & +2.0\%  & +3.3\%  \\
& 336 & \textbf{0.053} & \textbf{0.175} &-1.7\% & -1.7\%  & +4.5\% & +4.0\%    & +10.8\%    & +6.3\%    & +4.5\% & +2.9\%   \\
& 720 &\textbf{0.071}& \textbf{0.205}   &-0.9\%  & -1.0\%  & +5.5\% & +3.4\%  & +8.6\%    & +4.9\%    & +13.8\% & +7.8\%   \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Electricity}} 

&96  &\textbf{0.154}  &\textbf{0.247}  &+155\%  & +81\%   & +160\% & +84\%    & +330\%  & +155\%  & +242\% & +119\%  \\%&--& -- & \\
& 192 &\textbf{0.166} & \textbf{0.258} &+59\% & +39\%   & +121\%  & +67\%   & +224\%  & +117\%  & +264\% & +131\%  \\%&--& --  \\
& 336 & \textbf{0.188}& \textbf{0.283} &+55\%  & +35\%   & +150\%  & +74\%   & +128\%  & +71\% & +183\% & +95\%  \\%&--& -- \\
& 720 & \textbf{0.249}&\textbf{0.341}  &+33\%  & +25\%   & +154\%  & +73\%   & +192\%  & +95\%  & +312\% & +138\%  \\ %&--& --  \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Exchange}} 

&96  &\textbf{0.110}  &\textbf{0.247}  &-13\%  & -12\%   & +51\% & +17\%    & +4.6\%  & -1.2\%  & -4.6\% & -5.8\%  \\%&--& -- & \\
& 192 &\textbf{0.207} & \textbf{0.352} &+7.2\% & +0.0\%   & +69\%  & +32\%   & +29\%  & +12\%  & +22\% & +11\%  \\%&--& --  \\
& 336 & \textbf{0.327}& \textbf{0.461} &+48\%  & +13\%   & +62\%  & +20\%   & +68\%  & +24\% & +72\% & +23\%  \\%&--& -- \\
& 720 & \textbf{0.811}&\textbf{0.708}  &+29\%  & +14\%   & +24\%  & +9.6\%   & +38\%  & +12\%  & +64\% & +27\%  \\ %&--& --  \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Traffic}} 

&96  &\textbf{0.144}  &\textbf{0.215}  &+69\%  & +47\%   & +13\% & +15\%    & +300\%  & +176\%  & +271\% & +161\%  \\%&--& -- & \\
& 192 &\textbf{0.120} & \textbf{0.199} &+17\% & +7.5\%   & +31\%  & +24\%   & +258\%  & +149\%  & +1572\% & +355\%  \\%&--& --  \\
& 336 & \textbf{0.128}& \textbf{0.212} &+6.2\%  & +7.6\%   & +16\%  & +15\%   & +151\%  & +102\% & +1514\% & +368\%  \\%&--& -- \\
& 720 & \textbf{0.153}&\textbf{0.252}  &+38\%  & +28\%   & +11\%  & +7.9\%   & +250\%  & +126\%  & +1048\% & +349\%  \\ %&--& --  \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Weather}} 

&96  &\textbf{0.0012}  &\textbf{0.026}  &+17\%  & +6.2\%   & +16\% & +6.9\%    & +19\%  & +8.1\%  & +21\% & +8.9\%  \\%&--& -- & \\
& 192 &\textbf{0.0014} & \textbf{0.029} &-1.4\% & -2.4\%   & +5.0\%  & +1.7\%   & 0.7\%  & -0.7\%  & +4.3\% & +1.4\%  \\%&--& --  \\
& 336 & \textbf{0.0015}& \textbf{0.030} &+0.0\%  & -0.6\%   & +3.3\%  & +1.3\%   & +2.0\%  & +0.0\% & +3.3\% & +1.3\%  \\%&--& -- \\
& 720 & \textbf{0.0022}&\textbf{0.037}  &+4.6\%  & -0.3\%   & +4.1\%  & -1.6\%   & 3.6\%  & 0.0\%  & +0.0\% & -3.8\%  \\ %&--& --  \\

\midrule
\multirow{4}{*}{\rotatebox{90}{ILI}} 

&96  &\textbf{0.629}  &\textbf{0.538}  &+51\%  & +45\%   & -2.5\% & 9.5\%    & +20\%  & +29\%  & +112\% & +59\%  \\%&--& -- & \\
& 192 &\textbf{0.444} & \textbf{0.481} &+99\% & +58\%   & +25\%  & +24\%   & +84\%  & +56\%  & +360\% & +142\%  \\%&--& --  \\
& 336 & \textbf{0.557}& \textbf{0.584} &+33\%  & +31\%   & +21\%  & +16\%   & +58\%  & +30\% & +702\% & +94\%  \\%&--& -- \\
& 720 & \textbf{0.641}&\textbf{0.644}  &+8.4\%  & +5.4\%   & +23\%  & +18\%   & +42\%  & +22\%  & +74\% & +34\%  \\ %&--& --  \\
\bottomrule
\end{tabular}
\label{tab:ablation_FEL_full}
}
% \end{adjustwidth}
%\end{footnotesize}

\vskip -0.05in
\end{table*}
%}

==> tables/tab_ablation_FNO.tex <==
%\resizebox{!}{\.5\paperheight}{
\begin{table*}[ht]
\vskip -0.05in
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Ablation studies of FEL layer. The FEL layer is replaced with 4 different variants: MLP, LSTM, CNN, and Transformer. S4 is also introduced as a variant. The experiments are performed on ETTm1 and Electricity. The metric of variants is presented in relative value (’+’ indicates degraded performance, ’-’ indicates improved performance).}\vspace{-1mm}
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccccccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FilM}&\multicolumn{2}{c|}{LPU+MLP}&\multicolumn{2}{c|}{LPU+LSTM}&\multicolumn{2}{c|}{LPU+CNN}&\multicolumn{2}{c|}{LPU+attention}&\multicolumn{2}{c}{S4}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE&\\
\midrule

\multirow{4}{*}{\rotatebox{90}{ETTm1}} 

&96  &\textbf{0.030} &\textbf{0.128}  &+14\%   & +6.6\%   & +62\% & +31\%    & +286\%   & +118\%   & +709\%  & +166\% &-- & -- \\
& 192  &\textbf{0.047} &\textbf{0.160}  &+3.8\% & +2.2\%  & +271\% & +122\%  & +116\%   & +58\%    & +727\%  & +136\% &-- & -- \\
& 336 & \textbf{0.063} & \textbf{0.185} &-3.7\% & -2.1\%  & +90\% & +51\%    & +94\%    & +48\%    & +2524\% & +286\% &-- & --  \\
& 720 &\textbf{0.081}& \textbf{0.215}   &+0.9\%  & -0.6\%  & +127\% & +65\%  & +33\%    & +17\%    & +5783\% & +299\% &-- & --  \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Electricity}} 
% &96  &\textbf{0.213}  &\textbf{0.328}  &+15\%  & +6.8\% & +11\% & +5.2\%  & +11\%    & +5.2\% & +11\% & +4.8\%  &--& -- & +136\% & +58\%  \\
% & 192 &\textbf{0.268} & \textbf{0.373} &-4.6\% & -3.8\% & +7.8\%  & +3.9\%   & +6.8\%    & +3.5\% & -5.3\% & -3.9\%  &--& --  & +32\%  & +16\% \\
% & 336 & \textbf{0.307}& \textbf{0.417}&-4.2\%  & -5.0\% & -3.9\%  & -6.0\%   & -7.2\%    & -8.0\%   & -8.5\% & -9.0\%   &--& -- & +0.1\% & -5.0\% \\
% & 720 & \textbf{0.321}&\textbf{0.423} &+2.9\%  & +2.8\% & +10\%  &  +6.8\%  & +3.0\%   & +1.7\%  & +207\% & +85\%      &--& --  & 37\%  & 22\% \\

&96  &\textbf{0.213}  &\textbf{0.328}  &+103\%  & +40\%   & +37\% & +20\%    & +46\%  & +23\%  & +278\% & +105\% & 65\% & 38\% \\%&--& -- & \\
& 192 &\textbf{0.268} & \textbf{0.373} &+8.7\% & +0.01\%   & +32\%  & +14\%   & +42\%  & +21\%  & +249\% & +81\% & 39\% & 22\% \\%&--& --  \\
& 336 & \textbf{0.307}& \textbf{0.417} &-3.7\%  & -8.5\%   & +42\%  & +13\%   & +17\%  & +6.0\% & +564\% & +90\% & 33\% & 15\% \\%&--& -- \\
& 720 & \textbf{0.321}&\textbf{0.423}  &+5.7\%  & +1.4\%   & +98\%  & +36\%   & +32\%  & +18\%  & +2739\% & +117\% & 47\% & 22\% \\ %&--& --  \\
                        
                        
% \midrule
% \multirow{4}{*}{\rotatebox{90}{$Exchange$}} &96  & \textbf{0.079} & \textbf{0.204} &0.139 &0.276 &0.197  &0.323 &1.292 &0.849 &0.847  &0.752  &0.968  &0.812  &1.065  &0.829    \\
%                         & 192 & \textbf{0.159} & \textbf{0.292} &0.256 &0.369 &0.300  &0.369 &1.631 &0.968 &1.204   &0.895 &1.040  &0.851  &1.188  & 0.906   \\
%                         & 336 & \textbf{0.270} & \textbf{0.398} &0.426 &0.464 &0.509  &0.524 &2.225 &1.145 &1.672  &1.036  &1.659  &1.081  &1.357  &0.976     \\
%                         & 720 & \textbf{0.830} & \textbf{0.721} &1.090 &0.800 &1.447  &0.941 &2.521 &1.245 &2.478  &1.310  &1.941  &1.127  &1.510  &1.016     \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{$Traffic$}} &96  &\textbf{0.453}& \textbf{0.305} &0.562 &0.349 &0.613  &0.388 &0.824 &0.514 &0.719  &0.391  &0.684  &0.384  &0.732  &0.423    \\
%                         & 192 & \textbf{0.463} & \textbf{0.308} &0.562 &0.346 &0.616&0.382 &1.106 &0.672 &0.696 &0.379  &0.685  &0.390  &0.733  &0.420    \\
%                         & 336 & \textbf{0.483} & \textbf{0.321} &0.570 &0.323 &0.622  &0.337 &1.084 &0.627 &0.777  &0.420  &0.733  &0.408  &0.742  &0.420     \\
%                         & 720 & \textbf{0.562} & 0.383 &0.596 &\textbf{0.368} &0.660  &0.408 &1.536 &0.845 &0.864  &0.472  &0.717  &0.396  &0.755  &0.423     \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{$Weather$}} & 96 & \textbf{0.199} & \textbf{0.262} &0.217  &0.296  &0.266  &0.336 &0.406 &0.444 &0.300  &0.384  &0.458  &0.490  &0.689  &0.596    \\
%                         & 192 & \textbf{0.228} & \textbf{0.288} &0.276  &0.336  &0.307  &0.367 &0.525 &0.527 &0.598  &0.544  &0.658  &0.589  &0.752  &0.638    \\
%                         & 336 &\textbf{0.267} &\textbf{0.323} & 0.339  &0.380  &0.359  &0.395 &0.531 &0.539 &0.578  &0.523  &0.797  &0.652  &0.639  &0.596    \\
%                         & 720 &\textbf{0.319} & \textbf{0.361} &0.403  &0.428 &0.578 &0.578 &0.419  &0.428  &1.059  &0.741  &0.869  &0.675  &1.130  &0.792    \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{$ILI$}} & 24 & \textbf{1.970} & \textbf{0.875} &2.203  &0.963  &3.483 &1.287 &4.631 &1.484 &5.764  &1.677  &4.480  &1.444  &4.400 &1.382    \\
%                         & 36 & \textbf{1.982} & \textbf{0.859} &2.272  &0.976  &3.103  &1.148 &4.123 &1.348 &4.755  &1.467  &4.799  &1.467  &4.783  &1.448    \\
%                         & 48 & \textbf{1.868} & \textbf{0.896} &2.209  &0.981  &2.669  &1.085 &4.066 &1.36 &4.763  &1.469  &4.800  &1.468  &4.832  &1.465    \\
%                         & 60 & \textbf{2.057} & \textbf{0.929} &2.545  &1.061  &2.770  &1.125 &4.278 &1.41 &5.264  &1.564  &5.278  &1.560  &4.882  &1.483    \\
\bottomrule
\end{tabular}
\label{tab:ablation_FNO}
}
% \end{adjustwidth}
%\end{footnotesize}

\vskip -0.05in
\end{table*}
%}

==> tables/tab_ablation_HiPPO.tex <==
%\resizebox{!}{\.5\paperheight}{
\begin{table*}[h]

\vskip -0.05in
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Ablation studies of LPU layer. The original LPU block (whose projection and reconstruction matrix are fixed) is replaced with 6 variants (\textbf{Fixed} means the matrix are not trainable. \textbf{Trainable} means the matrix is initialized with original parameters and trainable. \textbf{Random Init} means the matrix is initialized randomly and trainable). The experiments are performed on ETTm1 and Electricity with different input lengths. The metric of variants is presented in relative value (`+` indicates degraded performance, `-` indicates improved performance).}
\vspace{-1mm}
\resizebox{\columnwidth}{!}{
\scalebox{0.60}{

\begin{tabular}{c|c|cccccccccccccccccc}
\toprule

\multicolumn{2}{c|}{Index}&\multicolumn{2}{c|}{Original}&\multicolumn{2}{c|}{Variant 1}&\multicolumn{2}{c|}{Variant 2}&\multicolumn{2}{c|}{Variant 3}&\multicolumn{2}{c|}{Variant 4}&\multicolumn{1}{c|}{Variant 5}&\multicolumn{2}{c}{Variant 6}\\
\midrule

\multicolumn{2}{c|}{Projection}&\multicolumn{4}{c|}{Fixed}&\multicolumn{6}{c|}{Trainable}&\multicolumn{1}{c|}{Random Init}&\multicolumn{2}{c}{Linear}\\
\midrule
\multicolumn{2}{c|}{Reconstruction}&\multicolumn{2}{c|}{Fixed}&\multicolumn{2}{c|}{Trainable}&\multicolumn{2}{c|}{Fixed}&\multicolumn{2}{c|}{Trainable}&\multicolumn{2}{c|}{Random Init}&\multicolumn{1}{c|}{--}&\multicolumn{2}{c}{Linear}\\

\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& -- & MSE  & MAE \\
\midrule
% \multirow{4}{*}{\rotatebox{90}{$ETTm2$}} &96 & \textbf{0.165} & \textbf{0.256} &0.203 &0.287 &0.255  &0.339 &0.705 &0.690 &0.365  &0.453  &0.768  &0.642  &0.658  &0.619    \\
%                         & 192 & \textbf{0.240} & \textbf{0.313} &0.269  &0.328  &0.281 &0.340 &0.924 &0.692 &0.533  &0.563  &0.989  &0.757  &1.078  &0.827    \\
%                         & 336 & \textbf{0.286} & \textbf{0.345} & 0.325 &0.366 &0.339  &0.372 &1.364 &0.877 &1.363&0.887  &1.334  &0.872  &1.549  &0.972     \\
%                         & 720 & \textbf{0.393} & \textbf{0.410} &0.421 &0.415 &0.422  &0.419 &0.877 &1.074 &3.379  &1.338 & 3.048 &1.328  &2.631  &1.242      \\
% \midrule
\multirow{4}{*}{\rotatebox{90}{ETTm1}} 

&96  &\textbf{0.030} &\textbf{0.128}    &+6.0\%  & +3.1\% & +4.6\% & +3.1\%  & +4.7\%   & +2.7\%   & +0.7\% & +0.6\%  & NaN & +38\% & +22\%  \\
& 192  &\textbf{0.047} &\textbf{0.160}  &-2.6\%  & -1.3\%    & +2.5\% & +1.8\%  & -0.4\%   & +0.4\%   & -3.0\% & -1.0\%  & NaN  & +9.5\%  & +8.7\% \\
& 336 & \textbf{0.063} & \textbf{0.185} &+4.2\% & +1.8\%    & -2.4\% & -0.4\%  & -6.3\%   & -2.5\%    & +2.2\% & +1.4\%   & NaN & +5.8\% & +5.0\% \\
& 720 &\textbf{0.081}& \textbf{0.215}   &-0.4\%     & -0.6\%     &+24\%    & +12\%  & +11\%    & +5.9\%   & NaN & NaN       & NaN      & +1.4\%  & +2.2\% \\

\midrule

\multirow{4}{*}{\rotatebox{90}{Electricity}}
&96  &\textbf{0.213}  &\textbf{0.328}  &+15\%  & +6.8\% & +11\% & +5.2\%  & +11\%    & +5.1\% & +11\% & +4.8\%  &NaN & +136\% & +58\%  \\
& 192 &\textbf{0.268} & \textbf{0.373} &-4.6\% & -3.8\% & +7.8\%  & +3.9\%   & +6.8\%    & +3.5\% & -5.3\% & -3.9\%  &NaN  & +32\%  & +16\% \\
& 336 & \textbf{0.307}& \textbf{0.417}&-4.2\%  & -5.0\% & -3.9\%  & -6.0\%   & -7.2\%    & -8.0\%   & -8.5\% & -9.0\%   &NaN & +0.1\% & -5.0\% \\
& 720 & \textbf{0.321}&\textbf{0.423} &+2.9\%  & +2.8\% & +10\%  &  +6.8\%  & +3.0\%   & +1.7\%  & +207\% & +85\%      &NaN  & 37\%  & 22\% \\

\bottomrule
\end{tabular}
\label{tab:ablation_HiPPO}
}}
% \end{adjustwidth}
%\end{footnotesize}
\vskip -0.05in
\end{table*}

%}

==> tables/tab_ablation_normalize.tex <==
%\resizebox{!}{\.5\paperheight}{
\begin{table*}[h]
\vskip -0.15in
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Ablation studies of Normalization and Multiscale. Multiscale use 3 branches with: $T$, $2T$, and $4T$ as input sequence length. T is the predicted sequence length}\vspace{-1mm}
\scalebox{0.7}{
\begin{tabular}{c|c|cccccccccccccccccc}
\toprule
\multicolumn{2}{c|}{Dataset}&\multicolumn{2}{c|}{ETTm2}&\multicolumn{2}{c|}{Electricity}&\multicolumn{2}{c|}{Exchange}&\multicolumn{2}{c|}{Traffic}&\multicolumn{2}{c|}{Weather}&\multicolumn{2}{c}{Illness}&\multicolumn{2}{c}{}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & Relative & MSE & Relative & MSE & Relative & MSE & Relative & MSE & Relative & MSE & Relative &\\
\midrule


\multirow{4}{*}{\rotatebox{90}{Methods}} 

&Original  &0.301 & +16\% & 0.195 & +4.8\% & 0.534 & + 60\% & 0.528 & +19\% & 0.264 & +4.9\% & 3.55 & + 80\% \\

& Normalization & 0.268 & +3.6\% & 0.199 & +6.4\% & 0.456 & +36\% & 0.656 & +48\% & 0.256 & +1.5\% & 3.36 & +70\% \\	
% &\textbf{0.047} &\textbf{0.160}  &-12\%  & -10\% & +2.5\% & +1.8\% & -0.4\%    & +0.4\%   & -\% & -\%  &--& --  \% \\
& Multiscale & 0.259 & + 0.19\% &	0.187 &   +0\%	& 0.335	 & 0\% & 0.541 & +22\% & 0.253 & +0.50\% &	2.41 & +22\% \\
& With both & 0.271	& +4.7\% &	0.189	& +1.5\% & 0.398 & +19\% & 0.442 & +0\% &  0.253 & +0.4\% & 1.97 & +0\% \\
% & 720 &\textbf{0.081}& \textbf{0.215}   &-0.\%     & -0.\%    & +\%    &  +\%   & +11\%    & +5.9\%   & -- & --       &--& - \\

% \midrule
% \multirow{4}{*}{\rotatebox{90}{$Electricity$}} 
% % &96  &\textbf{0.213}  &\textbf{0.328}  &+15\%  & +6.8\% & +11\% & +5.2\%  & +11\%    & +5.2\% & +11\% & +4.8\%  &--& -- & +136\% & +58\%  \\
% % & 192 &\textbf{0.268} & \textbf{0.373} &-4.6\% & -3.8\% & +7.8\%  & +3.9\%   & +6.8\%    & +3.5\% & -5.3\% & -3.9\%  &--& --  & +32\%  & +16\% \\
% % & 336 & \textbf{0.307}& \textbf{0.417}&-4.2\%  & -5.0\% & -3.9\%  & -6.0\%   & -7.2\%    & -8.0\%   & -8.5\% & -9.0\%   &--& -- & +0.1\% & -5.0\% \\
% % & 720 & \textbf{0.321}&\textbf{0.423} &+2.9\%  & +2.8\% & +10\%  &  +6.8\%  & +3.0\%   & +1.7\%  & +207\% & +85\%      &--& --  & 37\%  & 22\% \\

% &96  &\textbf{0.213}  &\textbf{0.328}  &+100\%  & +100\%   & +37\% & +20\%    & +46\%  & +23\%  & +11\% & +4.8\%  \\%&--& -- & \\
% & 192 &\textbf{0.268} & \textbf{0.373} &+8.7\% & +0.01\%   & +32\%  & +14\%   & +42\%  & +21\%  & -5.3\% & -3.9\%  \\%&--& --  \\
% & 336 & \textbf{0.307}& \textbf{0.417} &-3.7\%  & -8.5\%   & +42\%  & +13\%   & +17\%  & +6.0\% & -8.5\% & -9.0\% \\%&--& -- \\
% & 720 & \textbf{0.321}&\textbf{0.423}  &+5.7\%  & +1.4\%   & +98\%  & +36\%   & +32\%  & +18\%  & +207\% & +85\% \\ %&--& --  \\
                        

\bottomrule
\end{tabular}
\label{tab:ablation_normalize}
}
\vskip -0.05in
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
%}

==> tables/tab_ett_m.tex <==

\begin{table*}[h]
\centering
% \begin{small}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Multivariate long-term forecasting results on ETT full benchmark. The best results are highlighted in bold. A lower MSE indicates better performance. All experiments are repeated 5 times.}
\vskip 0.05in
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccccccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FiLM}&\multicolumn{2}{c|}{FEDformer}&\multicolumn{2}{c|}{Autoformer}&\multicolumn{2}{c|}{S4}&\multicolumn{2}{c|}{Informer}&\multicolumn{2}{c|}{LogTrans}&\multicolumn{2}{c}{Reformer}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTh1$}}
& 96 &\textbf{0.371} &\textbf{0.394} &0.376 &0.419  & 0.449& 0.459 &0.949 &0.777 & 0.865 & 0.713& 0.878& 0.740& 0.837& 0.728\\
& 192 &\textbf{0.414} &\textbf{0.423} &0.420 &0.448  & 0.500& 0.482 &0.882 &0.745 & 1.008 & 0.792& 1.037& 0.824& 0.923& 0.766\\
& 336 &\textbf{0.442} &\textbf{0.445} &0.459 &0.465  & 0.521& 0.496 &0.965 &0.75 & 1.107 & 0.809& 1.238& 0.932& 1.097& 0.835\\
& 720 &\textbf{0.465} &\textbf{0.472} &0.506 &0.507  & 0.514& 0.512 &1.074&0.814 & 1.181 &0.865&  1.135& 0.852& 1.257& 0.889\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTh2$}}
& 96  &\textbf{0.284} &\textbf{0.348} &0.346 &0.388 & 0.358& 0.397 &1.551&	0.968 & 3.755& 1.525& 2.116& 1.197 &2.626 &1.317\\
& 192 &\textbf{0.357} &\textbf{0.400} &0.429 &0.439 & 0.456& 0.452 &2.336	 &1.229 & 5.602& 1.931& 4.315& 1.635 &11.12 &2.979\\
& 336 &\textbf{0.377} &\textbf{0.417} &0.482 &0.480 & 0.482& 0.486 &2.801	 &1.259 & 4.721& 1.835& 1.124& 1.604 &9.323 &2.769\\
& 720 &\textbf{0.439} &\textbf{0.456} & 0.463 & 0.474 & 0.515& 0.511 &2.973	 &1.333 & 3.647& 1.625& 3.188& 1.540 &3.874 &1.697\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTm1$}}
& 96  &\textbf{0.302} &\textbf{0.345} &0.378 &0.418 & 0.505& 0.475 &0.640	 &0.584 & 0.672& 0.571& 0.600& 0.546 &0.538 &0.528\\
& 192 &\textbf{0.338} &\textbf{0.368} & 0.426 & 0.441 & 0.553& 0.496 &0.570	 &0.555 & 0.795& 0.669& 0.837& 0.700 &0.658 &0.592\\
& 336 &\textbf{0.373} &\textbf{0.388} & 0.445 & 0.459 & 0.621& 0.537 &0.795& 0.691& 1.212& 0.871& 1.124& 0.832 &0.898 &0.721\\
& 720 &\textbf{0.420} &\textbf{0.420} & 0.543 & 0.490 & 0.671& 0.561 &0.738 &0.655 & 1.166& 0.823& 1.153& 0.820 &1.102 &0.841\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTm2$}} &96 &\textbf{0.165} &\textbf{0.256} & 0.203 & 0.287 &0.255  &0.339  &0.705	 &0.690  &0.365  &0.453  &0.768  &0.642  &0.658  &0.619 \\
                        & 192 &\textbf{0.222} &\textbf{0.296} & 0.269 & 0.328 &0.281 &0.340  &0.924	 &0.692 &0.533  &0.563  &0.989  &0.757  &1.078  &0.827 \\
                        & 336 &\textbf{0.277} &\textbf{0.333} & 0.325 & 0.366  &0.339  &0.372  &1.364	 & 0.877 &1.363&0.887  &1.334  &0.872  &1.549  &0.972 \\
                        & 720 &\textbf{0.371} &\textbf{0.389} & 0.421 & 0.415  &0.422  &0.419  &2.074 &1.074  &3.379  &1.338 & 3.048 &1.328  &2.631  &1.242 \\
\bottomrule
\end{tabular}
}
\label{tab:multi-benchmarks-ett}
% \end{adjustwidth}
% \end{small}
% \vskip -0.1in
\end{table*}



==> tables/tab_ett_u.tex <==

\begin{table*}[h]
\centering
% \begin{small}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Univariate long-term forecasting results on ETT full benchmark. The best results are highlighted in bold. A lower MSE indicates better performance. All experiments are repeated 5 times.}
\vskip 0.05in
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccccccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FiLM}&\multicolumn{2}{c|}{FEDformer}&\multicolumn{2}{c|}{Autoformer}&\multicolumn{2}{c|}{S4}&\multicolumn{2}{c|}{Informer}&\multicolumn{2}{c|}{LogTrans}&\multicolumn{2}{c}{Reformer}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE\\
\midrule

\multirow{4}{*}{\rotatebox{90}{$ETTh1$}}
&96 &\textbf{0.055}&\textbf{0.178}&0.079 &0.215 &0.071 &0.206 &0.316 &0.490 &	0.193&	0.377&	0.283&	0.468&	0.532&	0.569\\
&192 &\textbf{0.072}&\textbf{0.207}&0.104 &0.245 & 0.114&	0.262 & 0.345&0.516 &	0.217&	0.395&	0.234&	0.409&	0.568&	0.575\\
&336 &\textbf{0.083}&\textbf{0.229}&0.119 &0.270 &0.107&0.258 &0.825 &0.846 &	0.202&	0.381&	0.386&	0.546&	0.635&	0.589\\
&720 &\textbf{0.090}&\textbf{0.240}&0.127 &0.280 &0.126&0.283 &0.190 &0.355 &	0.183&	0.355&	0.475&	0.628&	0.762&	0.666\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTh2$}}
&96 &\textbf{0.127}&0.272&0.128 &\textbf{0.271} & 0.153&	0.306 & 0.381&0.501 &	0.213&	0.373&	0.217&	0.379&	1.411&	0.838\\
&192 &\textbf{0.182}&0.335&0.185 &\textbf{0.330} & 0.204&	0.351 & 0.332&0.458 &	0.227&	0.387&	0.281&	0.429&	5.658&	1.671\\
&336 &\textbf{0.204}&\textbf{0.367}&0.231 &0.378 & 0.246&	0.389 & 0.655&0.670 &	0.242&	0.401&	0.293&	0.437&	4.777&	1.582\\
&720 &\textbf{0.241}&\textbf{0.396}&0.278 &0.420 & 0.268&	0.409 & 0.630&0.662 &	0.291&	0.439&	0.218&	0.387&	2.042&	1.039\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTm1$}}
&96 &\textbf{0.029}&\textbf{0.127}&0.033 &0.140 & 0.056&	0.183 & 0.651&0.733 &	0.109&	0.277&	0.049&	0.171&	0.296&	0.355\\
&192 &\textbf{0.041}&\textbf{0.153}&0.058 &0.186 & 0.081&	0.216 & 0.190& 0.372&	0.151&	0.310&	0.157&	0.317&	0.429&	0.474\\
&336 &\textbf{0.053}&\textbf{0.175}&0.071 &0.209 & 0.076&	0.218 & 0.428&0.581 &	0.427&	0.591&	0.289&	0.459&	0.585&	0.583\\
&720 &\textbf{0.071}&\textbf{0.205}&0.102 &0.250 & 0.110&	0.267 & 0.254&0.433 &	0.438&	0.586&	0.430&	0.579&	0.782&	0.730\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTm2$}} 
& 96 &0.065&\textbf{0.189}&\textbf{0.063} &0.189 & 0.065 & 0.189  & 0.153&0.318 & 0.088 & 0.225 & 0.075 & 0.208 & 0.076  &0.214   \\
& 192 &\textbf{0.094}&\textbf{0.233}& 0.102 & 0.245 & 0.118 & 0.256  &0.183 &0.350 & 0.132 &0.283 & 0.129 &0.275  & 0.132  & 0.290   \\
& 336 &\textbf{0.124}&\textbf{0.274}& 0.130 & 0.279 & 0.154 & 0.305  &0.204 &0.367  &0.180 &0.336 & 0.154 &0.302  & 0.160  & 0.312    \\
& 720 &\textbf{0.173}&\textbf{0.323}& 0.178 & 0.325 & 0.182 &0.335  &0.482 &0.567  &0.300  &0.435 & 0.160 &0.321  & 0.168  &0.335     \\
\bottomrule
\end{tabular}
}
\label{tab:uni-benchmarks-ett}
% \end{adjustwidth}
% \end{small}
\end{table*}

==> tables/tab_low_ran_approximation_full.tex <==
%\resizebox{!}{\.5\paperheight}{
\begin{table*}[h]

%\begin{wraptable}[9]{r}{0.6\textwidth}
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Low-rank Approximation (LRA) univariate forecasting study for frequency enhanced layer: Comp. K=0 means default version without LRA, 1 means the largest compression using K=1.}
%\resizebox{\columnwidth}{!}{
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccccc}
\toprule

\multicolumn{2}{c|}{Comp. K}&\multicolumn{2}{c|}{0}&\multicolumn{2}{c|}{16}&\multicolumn{2}{c|}{4}&\multicolumn{2}{c}{1}\\

\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE \\
\midrule

% \multirow{4}{*}{\rotatebox{90}{$Exchange$}} 

% &96  &\textbf{0.079} &\textbf{0.204}    &0.083  &0.209  &0.082  &0.208   &0.087    &0.217     \\
% & 192  &\textbf{0.159} &\textbf{0.292}  &0.166  &0.304  &0.166  &0.304   &0.172    &0.309      \\
% & 336 & \textbf{0.270} & \textbf{0.398} &0.340  &0.436  &0.300  &0.413   &0.349    &0.452      \\
% & 720 &\textbf{0.788}& \textbf{0.680}   &1.158  &0.806  &1.147  &0.801   &0.915   &0.719      \\
\multirow{4}{*}{\rotatebox{90}{$ETTm2$}} 

&96&0.065&0.189&0.064&0.185&\textbf{0.064}&\textbf{0.185}&0.064&0.186 \\

&192&0.094&0.233&0.094&0.231&0.093&0.231&\textbf{0.093}&\textbf{0.231} \\

&336&0.124&0.274&0.124&0.270&\textbf{0.124}&\textbf{0.269}&0.124&0.271 \\

&720&0.173&0.323&0.173&0.322&\textbf{0.173}&\textbf{0.322}&0.177&0.328 \\
\midrule

\multirow{4}{*}{\rotatebox{90}{$Electricity$}} 

&96&\textbf{0.154}&\textbf{0.247}&0.211&0.324&0.216&0.331&0.277&0.387 \\

&192&\textbf{0.166}&\textbf{0.258}&0.251&0.352&0.246&0.347&0.334&0.421 \\

&336&\textbf{0.188}&\textbf{0.283}&0.276&0.369&0.302&0.396&0.363&0.440 \\

&720&\textbf{0.249}&\textbf{0.341}&0.336&0.429&0.342&0.436&0.411&0.481 \\

\midrule

\multirow{4}{*}{\rotatebox{90}{$Exchange$}} 

&96&0.110&0.259&0.119&0.273&\textbf{0.104}&\textbf{0.247}&0.105&0.251 \\

&192&0.207&0.352&0.196&0.355&\textbf{0.195}&\textbf{0.349}&0.212&0.372 \\

&336&\textbf{0.327}&\textbf{0.461}&0.388&0.497&0.373&0.491&0.407&0.506 \\

&720&\textbf{0.811}&\textbf{0.708}&0.908&0.767&1.288&0.941&1.840&1.153 \\
\midrule

\multirow{4}{*}{\rotatebox{90}{$Traffic$}} 

&96&\textbf{0.144}&\textbf{0.215}&0.146&0.223&0.154&0.237&0.267&0.373 \\

&192&\textbf{0.120}&\textbf{0.199}&0.121&0.201&0.138&0.231&0.218&0.333 \\

&336&0.128&0.212&\textbf{0.120}&\textbf{0.206}&0.132&0.227&0.216&0.335 \\

&720&\textbf{0.153}&\textbf{0.252}&0.155&0.257&0.154&0.257&0.246&0.366 \\

\midrule

\multirow{4}{*}{\rotatebox{90}{$Weather$}} 

&96&0.0012&0.026&0.0011&0.025&\textbf{0.001}&\textbf{0.025}&0.001&0.025 \\

&192&0.0014&0.029&0.0014&0.028&\textbf{0.001}&\textbf{0.028}&0.001&0.028 \\

&336&0.0015&0.03&0.0015&0.030&\textbf{0.001}&\textbf{0.029}&0.002&0.030 \\

&720&0.0022&0.037&0.0022&0.037&\textbf{0.002}&\textbf{0.037}&0.002&0.037 \\
\midrule

\multirow{4}{*}{\rotatebox{90}{$ILI$}} 

&96&0.629&0.538&\textbf{0.599}&\textbf{0.556}&0.628&0.558&0.630&0.579 \\

&192&\textbf{0.444}&\textbf{0.481}&0.487&0.533&0.508&0.561&0.570&0.612 \\

&336&0.557&0.584&\textbf{0.553}&\textbf{0.565}&0.703&0.696&0.722&0.706 \\

&720&\textbf{0.641}&\textbf{0.644}&0.648&0.641&0.900&0.780&1.493&1.032 \\

\midrule
\multicolumn{2}{c|}{Parameter size}&\multicolumn{2}{c|}{100\%}&\multicolumn{2}{c|}{6.4\%}&\multicolumn{2}{c|}{1.6\%}&\multicolumn{2}{c}{0.4\%}\\
% \multirow{4}{*}{\rotatebox{90}{$Exchange$}}
% &96  &\textbf{0.079}  &\textbf{0.204}  &+15\%  & +6.8\% & +11\% & +5.2\%  & +11\%    & +5.1\% \\
% & 192 &\textbf{0.159} & \textbf{0.292} &-4.6\% & -3.8\% & +7.8\%  & +3.9\%   & +6.8\%    & +3.5\%  \\
% & 336 & \textbf{0.270}& \textbf{0.398}&-4.2\%  & -5.0\% & -3.9\%  & -6.0\%   & -7.2\%    & -8.0\% \\
% & 720 & \textbf{0.830}&\textbf{0.721} &+2.9\%  & +2.8\% & +10\%  &  +6.8\%  & +3.0\%   & +1.7\% \\
\bottomrule
\end{tabular}
\label{tab:FEL_LRA_FULL}
}
%}
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
%\end{wraptable}
%}

==> tables/tab_low_rank_approximation.tex <==
%\resizebox{!}{\.5\paperheight}{
\begin{table*}[h]

%\begin{wraptable}[9]{r}{0.6\textwidth}
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Low-rank Approximation (LRA) study for frequency enhanced layer: Comp. K=0 means default version without LRA, 1 means the largest compression using K=1.}
%\resizebox{\columnwidth}{!}{
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccccc}
\toprule

\multicolumn{2}{c|}{Comp. K}&\multicolumn{2}{c|}{0}&\multicolumn{2}{c|}{16}&\multicolumn{2}{c|}{4}&\multicolumn{2}{c}{1}\\

\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE \\
\midrule

% \multirow{4}{*}{\rotatebox{90}{$Exchange$}} 

% &96  &\textbf{0.079} &\textbf{0.204}    &0.083  &0.209  &0.082  &0.208   &0.087    &0.217     \\
% & 192  &\textbf{0.159} &\textbf{0.292}  &0.166  &0.304  &0.166  &0.304   &0.172    &0.309      \\
% & 336 & \textbf{0.270} & \textbf{0.398} &0.340  &0.436  &0.300  &0.413   &0.349    &0.452      \\
% & 720 &\textbf{0.788}& \textbf{0.680}   &1.158  &0.806  &1.147  &0.801   &0.915   &0.719      \\
\multirow{4}{*}{\rotatebox{90}{$ETTh1$}} 

&96  &\textbf{0.371} &\textbf{0.394}    &0.371  &0.397  &0.373  &0.399   & 0.391   & 0.418    \\
& 192  &0.414 &\textbf{0.423}  &0.414  &0.425  &\textbf{0.413}  &0.426   &  0.437  &  0.445    \\
& 336 & \textbf{0.442} & 0.445 &0.452  &0.451  &0.445  &\textbf{0.444}   &0.460    &0.458       \\
& 720 &\textbf{0.454}& \textbf{0.451}   &0.460  &0.472  &0.461  &0.471   &0.464    &0.476      \\

\midrule

\multirow{4}{*}{\rotatebox{90}{$Weather$}} 

&96  &\textbf{0.199} &\textbf{0.262}    &0.200  &0.266  &0.199  &0.263   &0.198    &0.261      \\
& 192  &0.228 &0.288  &0.232  &0.298  &0.227  &0.287   &\textbf{0.226}    &\textbf{0.285}       \\
& 336 & 0.267 & 0.323 &0.266  &0.320  &\textbf{0.253}  &\textbf{0.314}   &0.264    &0.316       \\
& 720 &0.319& 0.361   &\textbf{0.314}  &\textbf{0.352}  &0.319  &0.361   &0.314    &0.354      \\

\midrule
\multicolumn{2}{c|}{Parameter size}&\multicolumn{2}{c|}{100\%}&\multicolumn{2}{c|}{6.4\%}&\multicolumn{2}{c|}{1.6\%}&\multicolumn{2}{c}{0.4\%}\\
% \multirow{4}{*}{\rotatebox{90}{$Exchange$}}
% &96  &\textbf{0.079}  &\textbf{0.204}  &+15\%  & +6.8\% & +11\% & +5.2\%  & +11\%    & +5.1\% \\
% & 192 &\textbf{0.159} & \textbf{0.292} &-4.6\% & -3.8\% & +7.8\%  & +3.9\%   & +6.8\%    & +3.5\%  \\
% & 336 & \textbf{0.270}& \textbf{0.398}&-4.2\%  & -5.0\% & -3.9\%  & -6.0\%   & -7.2\%    & -8.0\% \\
% & 720 & \textbf{0.830}&\textbf{0.721} &+2.9\%  & +2.8\% & +10\%  &  +6.8\%  & +3.0\%   & +1.7\% \\
\bottomrule
\end{tabular}
\label{tab:FEL_LRA}
}
%}
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
%\end{wraptable}
%}

==> tables/tab_lra_3d.tex <==
%\resizebox{!}{\.5\paperheight}{

% \begin{wraptable}[11]{r}{0.6\textwidth}
\vskip -0.15in
% \begin{wraptable}{r}{0.6\textwidth}
\begin{table*}[h]
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Low-rank Approximation (LRA) study for Frequency Enhanced Layer (FEL): Comp. K=0 means default version without LRA, 1 means the largest compression using K=1.}\vspace{-1.5mm}
%\resizebox{\columnwidth}{!}{
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccccc}
\toprule

\multicolumn{2}{c|}{Comp. K}&\multicolumn{2}{c|}{0}&\multicolumn{2}{c|}{16}&\multicolumn{2}{c|}{4}&\multicolumn{2}{c}{1}\\

\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE \\
\midrule

% \multirow{4}{*}{\rotatebox{90}{$Exchange$}} 

% &96  &\textbf{0.079} &\textbf{0.204}    &0.083  &0.209  &0.082  &0.208   &0.087    &0.217     \\
% & 192  &\textbf{0.159} &\textbf{0.292}  &0.166  &0.304  &0.166  &0.304   &0.172    &0.309      \\
% & 336 & \textbf{0.270} & \textbf{0.398} &0.340  &0.436  &0.300  &0.413   &0.349    &0.452      \\
% & 720 &\textbf{0.788}& \textbf{0.680}   &1.158  &0.806  &1.147  &0.801   &0.915   &0.719      \\
\multirow{4}{*}{\rotatebox{90}{ETTh1}} 

&96  &\textbf{0.371} &\textbf{0.394}    &0.371  &0.396  &0.371  &0.398   & 0.400   & 0.421    \\
& 192  &0.414 &\textbf{0.423}  &0.411  &0.423  &0.414  &0.426   & 0.435   & 0.444    \\
& 336 & \textbf{0.442} & 0.445 &0.443  &0.446  &0.443  & 0.444  & 0.492   &  0.478     \\
& 720 &\textbf{0.454}& \textbf{0.451}   &0.464  &0.474  &0.468  &0.478   & 0.501   & 0.499      \\

\midrule

\multirow{4}{*}{\rotatebox{90}{Weather}} 
&96  &\textbf{0.199} &\textbf{0.262}   &0.199  &0.263  &0.197  &0.262   &0.198    & 0.263     \\
& 192  &0.228 &0.288  &0.225  &0.285  &0.226  &0.285   &0.225    & 0.286      \\
& 336 & 0.267 & 0.323 &0.266  &0.321  &0.263  &0.314   & 0.264   &  0.316      \\
& 720 &0.319& 0.361  &0.314 &0.355  &0.315  & 0.354   &0.318    & 0.357   \\
\midrule
% \multirow{4}{*}{\rotatebox{90}{$Exchange$}} 

% &96  &\textbf{0.079} &\textbf{0.204}    &0.079  &0.202  &0.081  &0.206   &0.084    &0.211     \\
% & 192  &\textbf{0.159} &\textbf{0.292}  &0.152  &0.287  &0.163  &0.299   &0.176    &0.313     \\
% & 336 & \textbf{0.270} & \textbf{0.398} &0.301  &0.411  &0.340  &0.439   &0.368    &0.459      \\
% & 720 &\textbf{0.788}& \textbf{0.680}   &0.952  &0.726  &1.229  &0.833   &1.705    &1.021     \\
% \midrule

\multicolumn{2}{c|}{Parameter size}&\multicolumn{2}{c|}{100\%}&\multicolumn{2}{c|}{1.95\%}&\multicolumn{2}{c|}{0.41\%}&\multicolumn{2}{c}{0.10\%}\\
% \multirow{4}{*}{\rotatebox{90}{$Exchange$}}
% &96  &\textbf{0.079}  &\textbf{0.204}  &+15\%  & +6.8\% & +11\% & +5.2\%  & +11\%    & +5.1\% \\
% & 192 &\textbf{0.159} & \textbf{0.292} &-4.6\% & -3.8\% & +7.8\%  & +3.9\%   & +6.8\%    & +3.5\%  \\
% & 336 & \textbf{0.270}& \textbf{0.398}&-4.2\%  & -5.0\% & -3.9\%  & -6.0\%   & -7.2\%    & -8.0\% \\
% & 720 & \textbf{0.830}&\textbf{0.721} &+2.9\%  & +2.8\% & +10\%  &  +6.8\%  & +3.0\%   & +1.7\% \\
\bottomrule
\end{tabular}
\label{tab:FEL_LRA}
}
%}
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
% \end{wraptable}
%}

==> tables/tab_mean_std.tex <==
\vspace{-.2cm}
\begin{table}[ht]
%\setlength{\uppercaptionskip}{0.pt}
%\setlength{\belowcaptionskip}{-0.pt}
% \label{sample-table-kstest}
%\vskip 0.15in
\centering
% \setlength{\belowcaptionskip}{2pt} 
\caption{MSE with error bars (Mean and STD) for FiLM and FEDformer baseline for multivariate long-term forecasting. All experiments are repeated 5 times.}
\begin{small}
% \begin{sc}
\scalebox{0.75}{
\begin{tabular}{c|c|ccccc}
\toprule
\multicolumn{2}{c|}{MSE}& ETTm2 & Electricity & Exchange & Traffic\\ %&\multicolumn{2}{c|}{Fedformer-f }\\%&\multicolumn{2}{c|}{}&\\
\midrule
\multirow{4}{*}{\rotatebox{90}{FiLM}} 
& 96 & 0.165 $\pm$ 0.0051 & 0.153$\pm$ 0.0014 & 0.079$\pm$ 0.002 & 0.416$\pm$ 0.010 \\
& 192 & 0.222 $\pm$ 0.0038 & 0.165$\pm$ 0.0023 & 0.159$\pm$ 0.011 & 0.408$\pm$ 0.007 \\
& 336 & 0.277 $\pm$ 0.0021 & 0.186$\pm$ 0.0018 & 0.270$\pm$ 0.018 & 0.425$\pm$ 0.007 \\
& 720 & 0.371 $\pm$ 0.0066 & 0.236$\pm$ 0.0022 & 0.536$\pm$ 0.026 & 0.520$\pm$ 0.003 \\
\midrule
\multirow{4}{*}{\rotatebox{90}{FED-f}} 
& 96 & 0.203 $\pm$ 0.0042 & 0.194 $\pm$ 0.0008 & 0.148 $\pm$ 0.002 & 0.217 $\pm$ 0.008 \\
& 192 & 0.269 $\pm$ 0.0023 & 0.201$\pm$ 0.0015 & 0.270$\pm$ 0.008 & 0.604 $\pm$ 0.004 \\
& 336 & 0.325 $\pm$ 0.0015 & 0.215$\pm$ 0.0018 & 0.460$\pm$ 0.016 & 0.621 $\pm$ 0.006 \\
& 720 & 0.421 $\pm$ 0.0038 & 0.246$\pm$ 0.0020 & 1.195$\pm$ 0.026 & 0.626 $\pm$ 0.003 \\
\bottomrule
\end{tabular}
}
\label{tab:std}
% \end{sc}
\end{small}
%\end{center}
\vskip -0.1in
\end{table}




==> tables/tab_mode_selection_policy.tex <==
% \begin{wraptable}[16]{r}{0.6\textwidth}
\begin{table*}[h]

% \begin{wraptable}[11]{r}{0.5\textwidth}
\vskip -0.1in

\centering
\caption{Mode selection policy study for frequency enhanced layer. Lowest: select the lowest $m$ frequency mode; Random: select $m$ random frequency mode; Low random: select the $0.8*m$ lowest frequency mode and $0.2*m$ random high frequency mode.}\vspace{-1.5mm}
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccc}
\toprule
\multicolumn{2}{c|}{Policy}&\multicolumn{2}{c|}{Lowest}&\multicolumn{2}{c|}{Random}&\multicolumn{2}{c}{Low random}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE \\
\midrule

\multirow{4}{*}{\rotatebox{90}{Exchange}} 

&96  &\textbf{0.086} &\textbf{0.204}    &0.086  &0.208  &0.087  &0.210        \\
& 192  &0.188 &\textbf{0.292}  &\textbf{0.187}  &0.318  &0.207  &0.340      \\
& 336 & 0.356 & \textbf{0.433} &0.358  &0.437  &\textbf{0.353}  &0.461   \\
& 720 &\textbf{0.727}& \textbf{0.669}   &0.788  &0.680  &0.748  &0.674   \\

\midrule

\multirow{4}{*}{\rotatebox{90}{Weather}} 

&96  &0.199 &0.262 &0.197  &0.256  &\textbf{0.196}  &\textbf{0.254}   \\
& 192  &\textbf{0.228} &\textbf{0.288}  &0.234  &0.300  &0.234  &0.301   \\
& 336 & 0.267 & 0.323 &0.266  &0.319  &\textbf{0.263}  &\textbf{0.316}   \\
& 720 &0.319& 0.361 &0.317  &0.356  &\textbf{0.316}  &\textbf{0.354}  \\

\bottomrule

\end{tabular}
\label{tab:mode}
}
\end{table*}
% \end{wraptable}


==> tables/tab_mode_selection_policy_full.tex <==
% \begin{wraptable}[16]{r}{0.6\textwidth}
\begin{table*}[h]

% \begin{wraptable}[11]{r}{0.5\textwidth}
\vskip -0.1in

\centering
\caption{Mode selection policy study for frequency enhanced layer. Lowest: select the lowest $m$ frequency mode; Random: select $m$ random frequency mode; Low random: select the $0.8*m$ lowest frequency mode and $0.2*m$ random high frequency mode.}\vspace{-1.5mm}
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccc}
\toprule
\multicolumn{2}{c|}{Policy}&\multicolumn{2}{c|}{Lowest}&\multicolumn{2}{c|}{Random}&\multicolumn{2}{c}{Low random}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE \\
\midrule
\multirow{4}{*}{\rotatebox{90}{ETTm2}} 
&96&\textbf{0.065}&\textbf{0.189}&0.066&0.189&0.066&0.190 \\

&192&\textbf{0.094}&\textbf{0.233}&0.096&0.235&0.096&0.235 \\

&336&\textbf{0.124}&0.274&0.125&\textbf{0.270}&0.128&0.275 \\

&720&0.173&0.323&\textbf{0.173}&\textbf{0.322}&0.173&0.323 \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Electricity}} 
&96&\textbf{0.154}&\textbf{0.247}&0.175&0.0.260&0.176&0.262 \\

&192&\textbf{0.166}&\textbf{0.258}&0.177&0.266&0.168&0.273 \\

&336&\textbf{0.188}&\textbf{0.283}&0.199&0.289&0.192&0.299 \\

&720&\textbf{0.249}&\textbf{0.341}&0.269&0.364&0.270&0.362 \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Exchange}} 
&96&0.11&0.259&0.110&0.256&\textbf{0.106}&\textbf{0.249} \\

&192&0.207&0.352&\textbf{0.196}&\textbf{0.351}&0.207&0.357 \\

&336&\textbf{0.327}&\textbf{0.461}&0.451&0.522&0.373&0.484 \\

&720&0.811&0.708&0.835&0.714&\textbf{0.604}&\textbf{0.628} \\


\midrule
\multirow{4}{*}{\rotatebox{90}{Traffic}} 
&96&\textbf{0.144}&\textbf{0.215}&0.145&0.216&0.145&0.217 \\

&192&0.12&0.199&0.119&0.198&\textbf{0.118}&\textbf{0.197} \\

&336&0.128&0.212&\textbf{0.122}&\textbf{0.207}&0.122&0.209 \\

&720&0.153&0.252&\textbf{0.142}&\textbf{0.238}&0.155&0.259 \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Weather}} 
&96&\textbf{0.0012}&\textbf{0.026}&0.0012&0.027&0.0012&0.026 \\

&192&\textbf{0.0014}&\textbf{0.029}&0.0014&0.029&0.0014&0.029 \\

&336&\textbf{0.0015}&\textbf{0.03}&0.0015&0.030&0.0015&0.030 \\

&720&\textbf{0.0022}&\textbf{0.037}&0.0023&0.037&0.0023&0.037 \\

\midrule
\multirow{4}{*}{\rotatebox{90}{ILI}} 
&96&0.629&0.538&0.639&0.542&\textbf{0.626}&\textbf{0.537} \\

&192&\textbf{0.444}&\textbf{0.481}&0.448&0.490&0.447&0.494 \\

&336&\textbf{0.557}&\textbf{0.584}&0.560&0.590&0.557&0.587 \\

&720&\textbf{0.641}&\textbf{0.644}&0.641&0.647&0.643&0.650 \\



\bottomrule

\end{tabular}
\label{tab:mode_full}
}
\end{table*}
% \end{wraptable}


==> tables/tab_noise_injection.tex <==
%\resizebox{!}{\.5\paperheight}{
\begin{table*}[h]
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Noise injection studies. A 0.3*$\mathcal{N}\left(0,1\right)$ Gaussian noise is introduced into our training/testing. We conduct 4 sets of experiments with/without noise in training and test phases. The experiments are performed on ETTm1 and Electricity with different output lengths. The metric of variants is presented in relative value ('+' indicates degraded performance, and '-' indicates improved performance).}
%\resizebox{\columnwidth}{!}{
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccc}
\toprule

\multicolumn{2}{c|}{Training}&\multicolumn{4}{c|}{noise}&\multicolumn{4}{c}{with noise}\\
\midrule
\multicolumn{2}{c|}{Testing}&\multicolumn{2}{c|}{without noise}&\multicolumn{2}{c|}{with noise}&\multicolumn{2}{c|}{without noise}&\multicolumn{2}{c}{with noise}\\

\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE \\
\midrule
% \multirow{4}{*}{\rotatebox{90}{$ETTm2$}} &96 & \textbf{0.165} & \textbf{0.256} &0.203 &0.287 &0.255  &0.339 &0.705 &0.690 &0.365  &0.453  &0.768  &0.642  &0.658  &0.619    \\
%                         & 192 & \textbf{0.240} & \textbf{0.313} &0.269  &0.328  &0.281 &0.340 &0.924 &0.692 &0.533  &0.563  &0.989  &0.757  &1.078  &0.827    \\
%                         & 336 & \textbf{0.286} & \textbf{0.345} & 0.325 &0.366 &0.339  &0.372 &1.364 &0.877 &1.363&0.887  &1.334  &0.872  &1.549  &0.972     \\
%                         & 720 & \textbf{0.393} & \textbf{0.410} &0.421 &0.415 &0.422  &0.419 &0.877 &1.074 &3.379  &1.338 & 3.048 &1.328  &2.631  &1.242      \\
% \midrule
\multirow{4}{*}{\rotatebox{90}{$ETTh1$}} 

&96  &\textbf{0.371} &\textbf{0.394}    &-1.6\%  & -2.0\% & -0.0\% & -0.0\%  & -1.6\%   & -2.0\%     \\
& 192  &\textbf{0.414} &\textbf{0.423}  &-0.5\%  & -1.4\%    & +0.5\% & -0.0\%  & -0.5\%   & -1.4\%    \\
& 336 & \textbf{0.442} & \textbf{0.445} &-1.8\% & -0.9\%    & -0.9\% & +1.3\%  & -3.2\%   & -1.6\%     \\
& 720 &\textbf{0.465}& \textbf{0.472}   &+0.2\%     & -0.2\%     &+0.9\%    & +0.9\%  & -0.6\%    & -0.4\%    \\

% \midrule

% \multirow{4}{*}{\rotatebox{90}{$Exchange$}}
% &96  &\textbf{0.079}  &\textbf{0.204}  &+15\%  & +6.8\% & +11\% & +5.2\%  & +11\%    & +5.1\% \\
% & 192 &\textbf{0.159} & \textbf{0.292} &-4.6\% & -3.8\% & +7.8\%  & +3.9\%   & +6.8\%    & +3.5\%  \\
% & 336 & \textbf{0.270}& \textbf{0.398}&-4.2\%  & -5.0\% & -3.9\%  & -6.0\%   & -7.2\%    & -8.0\% \\
% & 720 & \textbf{0.830}&\textbf{0.721} &+2.9\%  & +2.8\% & +10\%  &  +6.8\%  & +3.0\%   & +1.7\% \\
\bottomrule
\end{tabular}
\label{tab:ablation_noise}
}
%}
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
%}

==> tables/tab_parameter_size.tex <==
\begin{table}[h]
\centering
% \setlength{\belowcaptionskip}{2pt} 
\caption{Parameter size of baseline models and FiLM with different low-rank approximations: the models are trained and tested on ETT dataset; the subscript number denotes $k$ in low-rank approximation.}
\begin{small}
% \begin{sc}
\vskip 0.05in
\begin{tabular}{c|ccccccc}
\toprule
Methods&Transformer&Autoformer&FEDformer&FiLM&$\mathrm{FiLM}_{16}$ & $\mathrm{FiLM}_4$ & $\mathrm{FiLM}_1$\\
\midrule
Parameter(M) & 0.0069 & 0.0069& 0.0098& 1.50 & 0.0293 &0.0062& 0.00149 \\
%&\multicolumn{2}{c|}{Fedformer-f }\\%&\multicolumn{2}{c|}{}&\\
\bottomrule
\end{tabular}
\label{tab:size}
% \end{sc}
\end{small}
%\end{center}
\vskip -0.1in
\end{table}


==> tables/tab_rebuttal_nhits.tex <==
%\resizebox{!}{\.5\paperheight}{
% \vskip -0.2in
\begin{table*}[h!]
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{multivariate long-term series forecasting results on six datasets with various input length and prediction length $O \in \{96,192,336,720\}$ (For ILI dataset, we set prediction length $O \in \{24,36,48,60\}$). Supplementary results of non-Transformer baselines (N-Hits and a seasonal-naive model).}
% \vspace{-1mm}
\scalebox{0.8}{
\begin{tabular}{c|c|cccccccccccccccc|}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FiLM}&\multicolumn{2}{c|}{N-Hits}&\multicolumn{2}{c|}{FEDformer}&\multicolumn{2}{c|}{Autoformer}&\multicolumn{2}{c|}{Seasonal-naive}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTm2$}} 
                        &96 & \textbf{0.165} & 0.256 & 0.176 & \textbf{0.255} &0.203 &0.287 &0.255  &0.339  &0.262 &0.300 \\
                        & 192 & \textbf{0.222} & \textbf{0.296} & 0.245 & 0.305 & 0.269  &0.328  &0.281 &0.340  &0.319 &0.337\\
                        & 336 & \textbf{0.277} & \textbf{0.333} & 0.295 & 0.346 & 0.325 &0.366 &0.339  &0.372  &0.375 &0.371\\
                        & 720 & \textbf{0.371} & \textbf{0.389} & 0.401 & 0.426 & 0.421 &0.415 &0.422  &0.419 &0.469 &0.422\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Electricity$}} 
                        &96  &0.154  &0.267 & \textbf{0.147} & \textbf{0.249}  &0.183 &0.297 &0.201  &0.317 &0.211 &0.278\\
                        & 192 &\textbf{0.164} & \textbf{0.258} & 0.167 & 0.269 & 0.195 &0.308 &0.222  &0.334 &0.214 &0.282\\
                        & 336 & 0.188 & \textbf{0.283} & \textbf{0.186} & 0.290 & 0.212 &0.313 &0.231 &0.338 &0.226 &0.294\\
                        & 720 & 0.236 & \textbf{0.332} & 0.243 & 0.340 &\textbf{0.231} &0.343 &0.254  &0.361 &0.265 & 0.324\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Exchange$}} 
                        &96  & \textbf{0.086} & \textbf{0.204} &0.092 & 0.211 & 0.139 & 0.276 & 0.197 &0.323 &0.086 &0.204 \\
                        & 192 & \textbf{0.189} & \textbf{0.292} & 0.208 & 0.322 &0.256 &0.369 & 0.300 & 0.369 &0.172 &0.295\\
                        & 336 & \textbf{0.356} & \textbf{0.433} & 0.371 & 0.443 & 0.426 &0.464 & 0.509 & 0.524 &0.311 &0.401\\
                        & 720 & \textbf{0.727} & \textbf{0.669} & 0.888 & 0.723 &  1.090 &0.800 & 1.447 & 0.941 &0.832 &0.686\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Traffic$}} 
                        &96  & 0.416& 0.294 & \textbf{0.402} & \textbf{0.282} & 0.562 &0.349 &0.613  &0.388 &1.219 &0.497\\
                        & 192 & \textbf{0.408} & \textbf{0.288} &0.420 & 0.297 & 0.562 &0.346 &0.616&0.382 &1.089 &0.456\\
                        & 336 & \textbf{0.425} & \textbf{0.298} &0.448 & 0.313 & 0.570 &0.323 &0.622  &0.337 &1.147 &0.473\\
                        & 720 & \textbf{0.520} &\textbf{0.353} &0.539 & 0.353 & 0.596 &0.368 &0.660  &0.408 &1.181 &0.486\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Weather$}} 
                        & 96 & 0.199 & 0.262 & \textbf{0.158} & \textbf{0.195} & 0.217  &0.296  &0.266  &0.336 &0.315 &0.288\\
                        & 192 & 0.228 & 0.288 & \textbf{0.211} & \textbf{0.247} & 0.276  &0.336  &0.307  &0.367 &0.341 &0.305\\
                        & 336 &\textbf{0.267} & 0.323 & 0.274 & \textbf{0.300} & 0.339  &0.380  &0.359  &0.395 &0.381 &0.331\\
                        & 720 &\textbf{0.319} & 0.361 &0.351 & \textbf{0.353} & 0.403  &0.428 &0.578 &0.578 &0.440 &0.370 \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ILI$}} 
                        & 24 & 1.970 & 0.875 & \textbf{1.862} & \textbf{0.869} & 2.203  &0.963  &3.483 &1.287 &6.581 &1.699 \\
                        & 36 & \textbf{1.982} & \textbf{0.859} &2.071 & 0.969 & 2.272  &0.976  &3.103  &1.148 &7.121 &1.882 \\
                        & 48 & \textbf{1.868} & \textbf{0.896} &2.346 & 1.042 & 2.209  &0.981  &2.669  &1.085 &6.567 &1.797 \\
                        & 60 & \textbf{2.057} & \textbf{0.929} &2.560 & 1.073 & 2.545  &1.061  &2.770  &1.125 &5.885 &1.675 \\
\bottomrule
\end{tabular}
\label{tab:multi-benchmarks}
}
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
%}


% %\resizebox{!}{\.5\paperheight}{
% % \vskip -0.2in
% \begin{table*}[h]
% \centering
% %\begin{footnotesize}
% % \begin{adjustwidth}{-1.5in}{-1in}
% \caption{Univariate Benchmark}
% % \vspace{-1mm}
% \scalebox{0.8}{
% \begin{tabular}{c|c|cccccccccccccc|}
% \toprule
% \multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FiLM}&\multicolumn{2}{c|}{N-Hits}&\multicolumn{2}{c|}{N-BEATS}&\multicolumn{2}{c|}{FEDformer}&\multicolumn{2}{c|}{Autoformer}\\
% \midrule
% \multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE & MSE  & MAE\\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{$ETTm2$}} 
% & 96 & 0.065 & 0.189  & 0.066 & \textbf{0.185} & 0.082 & 0.219 &\textbf{0.063} &0.189 & 0.065 & 0.189 \\
% & 192& 0.094 & 0.233 & \textbf{0.087} & \textbf{0.223} & 0.120 & 0.268 &0.102 &0.245 & 0.118 & 0.256 \\
% & 336 & 0.124 & \textbf{0.274} & \textbf{0.106} &0.251&0.226 & 0.370& 0.130 &0.279 & 0.154 & 0.305  \\
% & 720 & \textbf{0.173} & 0.323 &0.178 &\textbf{0.312} &0.188 & 0.338 & 0.312&0.325 & 0.182 &0.335 \\
% \midrule

% \multirow{4}{*}{\rotatebox{90}{$Exchange$}} 
% &96  & 0.110 & 0.259 & \textbf{0.093} & \textbf{0.223} & 0.156 & 0.299 & 0.131 &0.284 & 0.241 & 0.387\\
% & 192 & \textbf{0.207} & 0.352& 0.230 & \textbf{0.313} &0.669  &0.665& 0.277 &0.420  &0.300  &0.369 \\
% & 336 & \textbf{0.327} & \textbf{0.461} &0.370 &0.486 &0.611 &0.605 &0.486&0.511 &0.509  &0.524 \\
% & 720 & 0.811 & 0.708 &\textbf{0.728} & \textbf{0.569}& 1.111 &0.860& 1.162 &0.832 &1.260  &0.867 \\
% % \midrule
% % \multirow{4}{*}{\rotatebox{90}{$Traffic$}} 
% %                         &96  & 0.416& 0.294 & \textbf{0.402} & \textbf{0.282} & 0.562 &0.349 &0.613  &0.388 \\
% %                         & 192 & \textbf{0.408} & \textbf{0.288} &0.420 & 0.297 & 0.562 &0.346 &0.616&0.382\\
% %                         & 336 & \textbf{0.425} & \textbf{0.298} &0.448 & 0.313 & 0.570 &0.323 &0.622  &0.337\\
% %                         & 720 & \textbf{0.520} &\textbf{0.353} &0.539 & 0.353 & 0.596 &0.368 &0.660  &0.408 \\
% % \midrule
% % \multirow{4}{*}{\rotatebox{90}{$Weather$}} 
% %                         & 96 & 0.199 & 0.262 & \textbf{0.158} & \textbf{0.195} & 0.217  &0.296  &0.266  &0.336\\
% %                         & 192 & 0.228 & 0.288 & \textbf{0.211} & \textbf{0.247} & 0.276  &0.336  &0.307  &0.367\\
% %                         & 336 &\textbf{0.267} & 0.323 & 0.274 & \textbf{0.300} & 0.339  &0.380  &0.359  &0.395 \\
% %                         & 720 &\textbf{0.319} & 0.361 &0.351 & \textbf{0.353} & 0.403  &0.428 &0.578 &0.578 \\
% % \midrule
% % \multirow{4}{*}{\rotatebox{90}{$ILI$}} 
% %                         & 24 & 1.970 & 0.875 & \textbf{1.862} & \textbf{0.869} & 2.203  &0.963  &3.483 &1.287 \\
% %                         & 36 & \textbf{1.982} & \textbf{0.859} &2.071 & 0.969 & 2.272  &0.976  &3.103  &1.148 \\
% %                         & 48 & \textbf{1.868} & \textbf{0.896} &2.346 & 1.042 & 2.209  &0.981  &2.669  &1.085 \\
% %                         & 60 & \textbf{2.057} & \textbf{0.929} &2.560 & 1.073 & 2.545  &1.061  &2.770  &1.125 \\
% \bottomrule
% \end{tabular}
% \label{tab:multi-benchmarks}
% }
% % \end{adjustwidth}
% %\end{footnotesize}
% \end{table*}
%}

==> tables/tab_signal_recovery.tex <==
%\resizebox{!}{\.5\paperheight}{
\begin{table*}[h]
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Ablation studies of FEL layer. The FEL layer is replaced with 4 different variants: MLP, LSTM, CNN, Transformer. S4 is also introduced as a variant. The experiments are performed on ETTm1 and Electricity. The metric of variants is presented in relative value (’+’ indicates degraded performance, ’-’ indicates improved performance).}
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccccccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FilM}&\multicolumn{2}{c|}{LPU+MLP}&\multicolumn{2}{c|}{LPU+LSTM}&\multicolumn{2}{c|}{LPU+CNN}&\multicolumn{2}{c|}{LPU+attention}&\multicolumn{2}{c}{S4}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE&\\
\midrule

\multirow{4}{*}{\rotatebox{90}{$ETTm1$}} 

&96  &\textbf{0.030} &\textbf{0.128}  &+14\%   & +6.6\%   & +62\% & +31\%    & +286\%   & +118\%   & +709\%  & +166\% &-- & -- \\
% & 192  &\textbf{0.047} &\textbf{0.160}  &+3.8\% & +2.2\%  & +271\% & +122\%  & +116\%   & +58\%    & +727\%  & +136\% &-- & -- \\
% & 336 & \textbf{0.063} & \textbf{0.185} &-3.7\% & -2.1\%  & +90\% & +51\%    & +94\%    & +48\%    & +2524\% & +286\% &-- & --  \\
% & 720 &\textbf{0.081}& \textbf{0.215}   &+0.9\%  & -0.6\%  & +127\% & +65\%  & +33\%    & +17\%    & +5783\% & +299\% &-- & --  \\

% \midrule
% \multirow{4}{*}{\rotatebox{90}{$Electricity$}} 
% % &96  &\textbf{0.213}  &\textbf{0.328}  &+15\%  & +6.8\% & +11\% & +5.2\%  & +11\%    & +5.2\% & +11\% & +4.8\%  &--& -- & +136\% & +58\%  \\
% % & 192 &\textbf{0.268} & \textbf{0.373} &-4.6\% & -3.8\% & +7.8\%  & +3.9\%   & +6.8\%    & +3.5\% & -5.3\% & -3.9\%  &--& --  & +32\%  & +16\% \\
% % & 336 & \textbf{0.307}& \textbf{0.417}&-4.2\%  & -5.0\% & -3.9\%  & -6.0\%   & -7.2\%    & -8.0\%   & -8.5\% & -9.0\%   &--& -- & +0.1\% & -5.0\% \\
% % & 720 & \textbf{0.321}&\textbf{0.423} &+2.9\%  & +2.8\% & +10\%  &  +6.8\%  & +3.0\%   & +1.7\%  & +207\% & +85\%      &--& --  & 37\%  & 22\% \\

% &96  &\textbf{0.213}  &\textbf{0.328}  &+103\%  & +40\%   & +37\% & +20\%    & +46\%  & +23\%  & +278\% & +105\% & 65\% & 38\% \\%&--& -- & \\
% & 192 &\textbf{0.268} & \textbf{0.373} &+8.7\% & +0.01\%   & +32\%  & +14\%   & +42\%  & +21\%  & +249\% & +81\% & 39\% & 22\% \\%&--& --  \\
% & 336 & \textbf{0.307}& \textbf{0.417} &-3.7\%  & -8.5\%   & +42\%  & +13\%   & +17\%  & +6.0\% & +564\% & +90\% & 33\% & 15\% \\%&--& -- \\
% & 720 & \textbf{0.321}&\textbf{0.423}  &+5.7\%  & +1.4\%   & +98\%  & +36\%   & +32\%  & +18\%  & +2739\% & +117\% & 47\% & 22\% \\ %&--& --  \\
                        
                        
\bottomrule
\end{tabular}
\label{tab:ablation_FNO}
}
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
%}

==> tables/useless_tabs/tab_hyperparam.tex <==

\begin{table*}[h]
\centering
% \begin{small}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Univariate long sequence time-series forecasting results on ETTm1, parameter sensitivity}
\vskip 0.05in
\scalebox{0.85}{
\begin{tabular}{c|c|cccccccccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FEDformer-f}&\multicolumn{2}{c|}{FEDformer-w}&\multicolumn{2}{c|}{Autoformer}&\multicolumn{2}{c|}{Informer}&\multicolumn{2}{c|}{LogTrans}&\multicolumn{2}{c}{Reformer}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE\\
\midrule

\multirow{4}{*}{\rotatebox{90}{$ETTh1$}}
&96 &0.079 &0.215 &0.080 &0.214 &\textbf{0.071} &\textbf{0.206}&	0.193&	0.377&	0.283&	0.468&	0.532&	0.569\\
&192 &\textbf{0.104} &\textbf{0.245} &0.105 &0.256 & 0.114&	0.262&	0.217&	0.395&	0.234&	0.409&	0.568&	0.575\\
&336 &0.119 &0.270 &0.120 &0.269 &\textbf{0.107}&\textbf{0.258}&	0.202&	0.381&	0.386&	0.546&	0.635&	0.589\\
&720 &0.142 &0.299 &0.127 &0.280 &\textbf{0.126}&\textbf{0.283}&	0.183&	0.355&	0.475&	0.628&	0.762&	0.666\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTh2$}}
&96 &\textbf{0.128} &\textbf{0.271} &0.156 &0.306 & 0.153&	0.306&	0.213&	0.373&	0.217&	0.379&	1.411&	0.838\\
&192 &\textbf{0.185} &\textbf{0.330} &0.238 &0.380 & 0.204&	0.351&	0.227&	0.387&	0.281&	0.429&	5.658&	1.671\\
&336 &\textbf{0.231} &\textbf{0.378} &0.271 &0.412 & 0.246&	0.389&	0.242&	0.401&	0.293&	0.437&	4.777&	1.582\\
&720 &0.278 &0.420 &0.288 &0.438 & \textbf{0.268}&	\textbf{0.409}&	0.291&	0.439&	0.218&	0.387&	2.042&	1.039\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTm1$}}
&96 &\textbf{0.033} &\textbf{0.140} &0.036 &0.149 & 0.056&	0.183&	0.109&	0.277&	0.049&	0.171&	0.296&	0.355\\
&192 &\textbf{0.058} &\textbf{0.186} &0.069 &0.206 & 0.081&	0.216&	0.151&	0.310&	0.157&	0.317&	0.429&	0.474\\
&336 &0.084 &0.231 &\textbf{0.071} &\textbf{0.209} & 0.076&	0.218&	0.427&	0.591&	0.289&	0.459&	0.585&	0.583\\
&720 &\textbf{0.102} &0.250 &0.105 &\textbf{0.248} & 0.110&	0.267&	0.438&	0.586&	0.430&	0.579&	0.782&	0.730\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTm2$}} 
& 96 & 0.067 & 0.198 &\textbf{0.063} &\textbf{0.189} & 0.065 & 0.189 & 0.088 & 0.225 & 0.075 & 0.208 & 0.076  &0.214   \\
& 192 & \textbf{0.102} & \textbf{0.245} &0.110 &0.252 & 0.118 & 0.256 & 0.132 &0.283 & 0.129 &0.275  & 0.132  & 0.290   \\
& 336 & \textbf{0.130} & \textbf{0.279} &0.147 &0.301 & 0.154 & 0.305  &0.180 &0.336 & 0.154 &0.302  & 0.160  & 0.312    \\
& 720 & \textbf{0.178} & \textbf{0.325} &0.219 &0.368 & 0.182 &0.335  &0.300  &0.435 & 0.160 &0.321  & 0.168  &0.335     \\
\bottomrule
\end{tabular}
}
\label{tab:uni-benchmarks-ett}
% \end{adjustwidth}
% \end{small}
\end{table*}

% \begin{table*}[t]
% \centering
% % \begin{small}
% % \begin{adjustwidth}{-1.5in}{-1in}
% \caption{Univariate long sequence time-series forecasting results on ETT full benchmark. The best results are highlighted in bold.}
% \vskip 0.05in
% \scalebox{0.85}{
% \begin{tabular}{c|c|cccccccccccccccc}
% \toprule
% \multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FEDformer-f}&\multicolumn{2}{c|}{FEDformer-w}&\multicolumn{2}{c|}{Autoformer}&\multicolumn{2}{c|}{Informer}&\multicolumn{2}{c|}{LogTrans}&\multicolumn{2}{c}{Reformer}\\
% \midrule
% \multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE\\
% \midrule

% \multirow{4}{*}{\rotatebox{90}{$ETTh1$}}
% &96 &0.079 &0.215 &0.080 &0.214 &\textbf{0.071} &\textbf{0.206}&	0.193&	0.377&	0.283&	0.468&	0.532&	0.569\\
% &192 &\textbf{0.104} &\textbf{0.245} &0.105 &0.256 & 0.114&	0.262&	0.217&	0.395&	0.234&	0.409&	0.568&	0.575\\
% &336 &0.119 &0.270 &0.120 &0.269 &\textbf{0.107}&\textbf{0.258}&	0.202&	0.381&	0.386&	0.546&	0.635&	0.589\\
% &720 &0.142 &0.299 &0.127 &0.280 &\textbf{0.126}&\textbf{0.283}&	0.183&	0.355&	0.475&	0.628&	0.762&	0.666\\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{$ETTh2$}}
% &96 &\textbf{0.128} &\textbf{0.271} &0.156 &0.306 & 0.153&	0.306&	0.213&	0.373&	0.217&	0.379&	1.411&	0.838\\
% &192 &\textbf{0.185} &\textbf{0.330} &0.238 &0.380 & 0.204&	0.351&	0.227&	0.387&	0.281&	0.429&	5.658&	1.671\\
% &336 &\textbf{0.231} &\textbf{0.378} &0.271 &0.412 & 0.246&	0.389&	0.242&	0.401&	0.293&	0.437&	4.777&	1.582\\
% &720 &0.278 &0.420 &0.288 &0.438 & \textbf{0.268}&	\textbf{0.409}&	0.291&	0.439&	0.218&	0.387&	2.042&	1.039\\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{$ETTm1$}}
% &96 &\textbf{0.033} &\textbf{0.140} &0.036 &0.149 & 0.056&	0.183&	0.109&	0.277&	0.049&	0.171&	0.296&	0.355\\
% &192 &\textbf{0.058} &\textbf{0.186} &0.069 &0.206 & 0.081&	0.216&	0.151&	0.310&	0.157&	0.317&	0.429&	0.474\\
% &336 &0.084 &0.231 &\textbf{0.071} &\textbf{0.209} & 0.076&	0.218&	0.427&	0.591&	0.289&	0.459&	0.585&	0.583\\
% &720 &\textbf{0.102} &0.250 &0.105 &\textbf{0.248} & 0.110&	0.267&	0.438&	0.586&	0.430&	0.579&	0.782&	0.730\\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{$ETTm2$}} 
% & 96 & 0.067 & 0.198 &\textbf{0.063} &\textbf{0.189} & 0.065 & 0.189 & 0.088 & 0.225 & 0.075 & 0.208 & 0.076  &0.214   \\
% & 192 & \textbf{0.102} & \textbf{0.245} &0.110 &0.252 & 0.118 & 0.256 & 0.132 &0.283 & 0.129 &0.275  & 0.132  & 0.290   \\
% & 336 & \textbf{0.130} & \textbf{0.279} &0.147 &0.301 & 0.154 & 0.305  &0.180 &0.336 & 0.154 &0.302  & 0.160  & 0.312    \\
% & 720 & \textbf{0.178} & \textbf{0.325} &0.219 &0.368 & 0.182 &0.335  &0.300  &0.435 & 0.160 &0.321  & 0.168  &0.335     \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:uni-benchmarks-ett}
% % \end{adjustwidth}
% % \end{small}
% \end{table*}


==> tables_iTran/Interpolation.tex <==
%\resizebox{!}{\.5\paperheight}{
%\vskip -0.1in
\begin{table}[h]
\centering
\begin{sc}

% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Interpolation Ablation: Univariate long-term series forecasting results on Electricity with input length $L = 96$ and prediction length $T \in \{96, 192, 336, 720\}$. 
}
%\vspace{-2mm}
\scalebox{0.72}{
\begin{tabular}{cc|cccccccc}

\toprule
&{Methods} &\multicolumn{2}{c|}{96} &\multicolumn{2}{c|}{192} &\multicolumn{2}{c|}{336}  &\multicolumn{2}{c}{720} \\% &\multicolumn{2}{c|}{FEDformer} &\multicolumn{2}{c|}{Autoformer} &\multicolumn{2}{c|}{Informer} &\multicolumn{2}{c|}{LogTrans} &\multicolumn{2}{c}{Reformer}\\

\midrule
&{Metric} & MSE  & MAE & MSE & MAE & MSE  & MAE & MSE  & MAE \\%& MSE  & MAE& MSE  & MAE& MSE  & MAE & MSE  & MAE & MSE & MAE\\
\midrule

&{Spline} & 0.257           & 0.361           & 0.289       & 0.376      & 0.347       & 0.413      & 0.403      & 0.459       \\%& 0.73  & 0.592 & 0.796 & 0.62  & 1.163 & 0.791 & 1.597 & 0.979 & 1.264 & 0.826 \\


\midrule

&{TwoAver}  & 0.255           & 0.360           & 0.287       & 0.375      & 0.335       & 0.408      & 0.406      & 0.461\\%& 0.266 & 0.353 & 0.346 & 0.404 & 1.281 & 0.929 & 0.934 & 0.746 & 1.289 & 0.904 \\

\midrule

&{FourAver} & 0.254           & 0.360           & 0.287       & 0.376      & 0.343       & 0.411      & 0.409      & 0.462  \\%& 0.676 & 0.423 & 0.833 & 0.502 & 1.591 & 0.832 & 1.309 & 0.685 & 1.618 & 0.851 \\


\midrule
&{Rbf} & 0.256           & 0.361           & 0.290       & 0.377      & 0.348       & 0.413      & 0.400      & 0.457 \\%& 0.309 & 0.353 & 0.31  & 0.353 & 0.584 & 0.527 & 0.457 & 0.458 & 0.447 & 0.453 \\

\midrule
&{No Interpolation} & 0.258           & 0.364           & 0.293       & 0.380      & 0.351       & 0.416      & 0.409      & 0.463 \\%& 1.741 & 1.005 & 1.893 & 1.038 & 4.183 & 1.622 & 3.847 & 1.558 & 2.594 & 1.320 \\



\midrule


%\multicolumn{2}{c|}{Average} & \textbf{0.316}  & \textbf{0.314} & 0.377 &0.375  &0.392 &0.383  &0.483 &0.445 &0.537 &0.480 &0.697 &0.537 &0.909 &0.675 &1.341 &0.789 &1.878 &0.994 &1.819 &0.966\\
% \midrule
% \multicolumn{2}{c|}{Average} & & & & & & & & & & & & & & & \\
\bottomrule
\end{tabular}
\label{tab:Interpolation_Ablation}
}
% \end{adjustwidth}
%\vskip 0.1in
\vskip -0.10in
\end{sc}
\end{table}
%}

==> tables_iTran/dataset.tex <==



%\resizebox{!}{\.5\paperheight}{
\vskip -0.1in
\begin{table}[h]
\centering

%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Detailed dataset description. }\vspace{-3mm}

\begin{center}
% \begin{small}
\begin{sc}
\scalebox{0.80}{
\begin{tabular}{c|cccccccccccccc}
\toprule  
Dataset & Dim & Train-Valid-Test Splits & Freq & Domain \\  
\midrule  

ETTh1/ETTh2 &{7} & {(8545,2881,2881)} & {Hourly} & {Electricity} \\  


% ETTh1 & \multirow{2}*{7} & \multirow{2}*{(8545,2881,2881)} & \multirow{2}*{Hourly} & \multirow{2}*{Electricity} \\  
% ETTh2 & ~ & ~ &  ~ &  ~ \\ % 假设ETTh2的详细信息也缺失  
\midrule 
Traffic & 862 & (12185,1757,3509) & Hourly & 
Transportation \\
\midrule 
ECL & 321 & (18317,2633,5261) & Hourly & Electricity \\  
\midrule 
Weather & 21 & (36792,5271,10540) & 10min & Weather \\   
\bottomrule  
\end{tabular}
\label{tab:dataset_descriptions}
}

\end{sc}
% \end{small}
\end{center}
\vskip -0.15in
% \end{adjustwidth}
%\end{footnotesize}
\end{table}
%}

==> tables_iTran/test.tex <==
%单变量，输入为96
\begin{table}[]
\begin{tabular}{clc|llll|llll|llll}
\hline
\multicolumn{3}{c|}{\multirow{2}{*}{Methods}}                          & \multicolumn{4}{c|}{Electricity} & \multicolumn{4}{c|}{Traffic} & \multicolumn{4}{c}{Weather} \\ \cline{4-15} 
\multicolumn{3}{c|}{}                                                  & 96           & 192  & 336   & 96   & 192   & 336      & 96   & 192   & 336     \\ \hline
\multicolumn{2}{c|}{\multirow{2}{*}{FEDformer}}   & Original           & 0.253/0.370  & 0.282/0.386     & 0.346/0.431      & 0.207/0.312    &  0.205/0.312     & 0.219/0.323         &   0.0062/0.062   & 0.0060/0.062     &   0.0041/0.050        \\ \cline{3-15} 
\multicolumn{2}{c|}{}                             & Sparse             & 0.244/0.363             &   0.281/0.386   & 0.342/0.429       &  0.217/0.330    &   0.233/0.338    & 0.214/0.324      &    XXX  &  XXX     & XXX          \\ \hline
\multicolumn{2}{c|}{\multirow{2}{*}{Informer}}    & Original           &    0.258/0.367          &   0.285/0.388   &  0.336/0.423       &  0.257/0.353    & 0.299/0.376      & 0.312/0.387          & 0.004/0.044     &    0.002/0.040   &   0.004/0.049      \\ \cline{3-15} 
\multicolumn{2}{c|}{}                             & Sparse             &              &      &      &     &      &       &       &       &      &       &       &      \\ \hline
\multicolumn{2}{c|}{\multirow{2}{*}{Autoformer}}  & Original           &  0.341/0.438            &  0.345/0.428    &  0.406/0.470     & 0.246/0.346     & 0.266/0.370      &0.263/0.371          &   0.011/0.081   &   0.0075/0.067    &  0.0063/0.062      \\ \cline{3-15} 
\multicolumn{2}{c|}{}                             & Sparse             &              &           &           &       &       &       &      &       &            \\ \hline

\end{tabular}
\end{table}

==> tables_vq/EncoderVQ.tex <==
%\resizebox{!}{\.5\paperheight}{
\vskip -0.1in
\begin{table}[h]
\centering

%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Univariate long-term series forecasting results of traditional transformer with Vector Quantization incorporated before the encoder(VQ-pre) and after the decoder(VQ-post). Input length $=512$ and prediction length $=96$. A lower MSE indicates better performance. All experiments are repeated three times.}\vspace{-3mm}

\begin{center}
% \begin{small}
\begin{sc}
\scalebox{0.85}{
\begin{tabular}{c|cccccccccccccc}
\toprule
% \multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{PatchTST(96)}&\multicolumn{2}{c|}{Attention}&\multicolumn{2}{c|}{Series-LG/GL}&\multicolumn{2}{c|}{Series-GL}&\multicolumn{2}{c}{Concatenate}\\
Methods &\multicolumn{2}{c|}{PatchTST} &\multicolumn{2}{c|}{VQ-pre}&\multicolumn{2}{c}{VQ-post}\\
\midrule
Metric & MSE  & MAE & MSE & MAE  & MSE & MAE  \\
\midrule

 ettm2    & \textbf{0.065}  & \textbf{0.187}  & 0.067  & 0.191  &0.068 &0.196 \\
 electricity      & \textbf{0.209}  & \textbf{0.321}  & 0.226  & 0.331  &0.237 &0.341 \\
 traffic   & 0.134  & 0.223  & \textbf{0.125}  & \textbf{0.203}  &0.135 &0.219 \\
 weather   & 0.0013 & 0.0265 & \textbf{0.0009} & \textbf{0.0217}  & \textbf{0.0009} &0.0223\\
 wind     & \textbf{2.563}  & \textbf{1.261}  & 2.875  & 1.295  &3.017 &1.322 \\
 nordpool  & \textbf{0.856}  & 0.714  & 0.912  & \textbf{0.712}  &0.950 &0.719 \\
 caiso     & 0.162  &0.279  & \textbf{0.161}  & \textbf{0.277}  &0.169 &0.284 \\


\midrule
\bottomrule
\end{tabular}
\label{tab:ablation_EncoderVQ}
}

\end{sc}
% \end{small}
\end{center}
\vskip -0.15in
% \end{adjustwidth}
%\end{footnotesize}
\end{table}
%}

==> tables_vq/PatchTST_woReverseNorm.tex <==
%\resizebox{!}{\.5\paperheight}{
% \vskip -0.2in
\begin{table*}[t]
\centering
\begin{sc}
%\color{blue}
\caption{Univariate forecasting results by PatchTST without ReverseNorm.}
\vspace{-1mm}
\scalebox{0.75}{

\begin{tabular}{c|c|cccccccccccccccccccc}

\toprule
\multicolumn{2}{c|}{woReverseNorm}
&\multicolumn{4}{c|}{traffic}&\multicolumn{4}{c|}{weather}&\multicolumn{4}{c}{ETTm2}\\
\midrule

\multicolumn{2}{c|}{PredLen} & 96 & 192  & 336 &720  & 96 & 192  & 336 & 720 & 96 & 192  & 336 & 720 \\

\midrule

\multirow{2}{*}{PatchTST\_wFFN} 
&MSE &\textbf{0.393} & \textbf{0.403} & \textbf{0.414} & \textbf{0.404} & 0.0450 & \textbf{0.0418} & \textbf{0.0347} & \textbf{0.0371} & \textbf{0.435} & \textbf{0.417} & \textbf{0.487} & \textbf{0.439} \\
&MAE &\textbf{0.454} & \textbf{0.460} & \textbf{0.468} & \textbf{0.462} & 0.1643 & \textbf{0.1622} & \textbf{0.1469} & \textbf{0.1517} & \textbf{0.455} & \textbf{0.433} & \textbf{0.464} & \textbf{0.425} \\

\midrule

\multirow{2}{*}{PatchTST\_woFFN}
&MSE &0.425          & 0.415          & 0.416          & 0.416          & \textbf{0.0442}          & 0.0463          & 0.0364          & 0.0376          & 0.569          & 0.619          & 0.602          & 0.591          \\
&MAE &0.479          & 0.470          & 0.470          & 0.467          & \textbf{0.1640}          & 0.1706          & 0.1505          & 0.1540          & 0.558          & 0.603          & 0.600          & 0.585      \\



\midrule
% \multicolumn{2}{c|}{Average} & & & & & & & & & & & & & & & \\
\bottomrule

\end{tabular}

}

\label{tab:PatchTST_woReverseNorm}
% \end{adjustwidth}
%\end{footnotesize}
\end{sc}
% \end{small}
%\vskip -0.1in
\end{table*}
%}







==> tables_vq/ablation_codebook_size.tex <==
%\resizebox{!}{\.5\paperheight}{
\vskip -0.05in
\begin{table}[h]
\centering

%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Sparse-VQ with different size of codebook. A lower MSE indicates better performance. All experiments are repeated three times on average.} %Input length $=512$ and prediction length $=720$ with hidden dimension $=16$. 
\vspace{-3mm}

\begin{center}
% \begin{small}
\begin{sc}
\scalebox{0.80}{
\begin{tabular}{cc|cccccccccc}
\toprule

&{Codebook Size} &\multicolumn{2}{c|}{10} &\multicolumn{2}{c|}{750}&\multicolumn{2}{c}{10000}\\
\midrule
&Metric & MSE  & MAE & MSE & MAE  & MSE & MAE \\
\midrule

&Caiso &0.500 & 0.471 & \textbf{0.451} & \textbf{0.454} & 0.480 &463  \\
\midrule
&Weather &0.315 & 0.341 & \textbf{0.306} & \textbf{0.322} & 0.322 & 0.349 \\
\midrule
&ETTm2 &0.372 & 0.393  & \textbf{0.356} & \textbf{0.376} & 0.367 & 0.389 \\


\midrule
\bottomrule
\end{tabular}
\label{tab:ablation_codebook_size}
}

\end{sc}
% \end{small}
\end{center}
%\vskip -0.20in
% \end{adjustwidth}
%\end{footnotesize}
\end{table}
%}

==> tables_vq/ablation_modules.tex <==
%\resizebox{!}{\.5\paperheight}{
% \vskip -0.2in
\begin{table*}[h]
\centering

%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Ablation study of FFN-free and Sparse-VQ in PatchTST. 4 cases are included: (a) both FFN-free and Sparse-VQ are included in model (SVQ+FFN-f); (b) only Vector Quantization (VQ+FFN-f); (c) only FFN-free(FFN-f);(d) neither of them is included (Original patchTST model). The best results are in bold. A lower MSE indicates better performance. All experiments are repeated 3 times.}\vspace{-3mm}

\begin{center}
% \begin{small}
\begin{sc}
\scalebox{1.0}{
\begin{tabular}{c|c|cccccccccccccccc}
\toprule
% \multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{PatchTST(96)}&\multicolumn{2}{c|}{Attention}&\multicolumn{2}{c|}{Series-LG/GL}&\multicolumn{2}{c|}{Series-GL}&\multicolumn{2}{c}{Concatenate}\\
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{SVQ+FFN-f}&\multicolumn{2}{c|}{VQ+FFN-f}&\multicolumn{2}{c|}{FFN-f}&\multicolumn{2}{c}{Original}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE\\
\midrule
\multirow{4}{*}{\rotatebox{90}{ETTm2}} 
&96 &\textbf{0.063} & \textbf{0.183} & \textbf{0.063} & 0.185 & 0.064 & 0.185 & 0.065 & 0.187 \\
&192 &\textbf{0.090} & \textbf{0.225} & 0.091 &0.227 & 0.093 & 0.228 & 0.093 & 0.230 \\
&336 &\textbf{0.118} & \textbf{0.262} & \textbf{0.118} & 0.263  & 0.119 & 0.263 & 0.122 & 0.267 \\
&720 &\textbf{0.172} & \textbf{0.320} & \textbf{0.172} & 0.322 & 0.173 & 0.323 & 0.173 & 0.324 \\


\midrule
\multirow{4}{*}{\rotatebox{90}{Electricity}} 
&96 &\textbf{0.194} & \textbf{0.304} & 0.196 & 0.306 & 0.198 & 0.309 & 0.209 & 0.321 \\
&192 &\textbf{0.226} & \textbf{0.325} & 0.229 & 0.330 & 0.231 & 0.330 & 0.246 & 0.344 \\
&336 &\textbf{0.263} & \textbf{0.358} & 0.269 & 0.363 & 0.271 & 0.364 & 0.280 & 0.370 \\
&720 &\textbf{0.298} & \textbf{0.404} & 0.317 & 0.413 & 0.322 & 0.417 & 0.332 & 0.424 \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Weather}}
&96 &\textbf{0.00091} & \textbf{0.0210} & 0.00113 & 0.0252 & 0.00111 & 0.0248 & 0.00132 & 0.0265 \\
&192 &\textbf{0.00113} & \textbf{0.0239} & 0.00128 & 0.0262 & 0.00132 & 0.0275 & 0.00144 & 0.0281 \\
&336 &\textbf{0.00130} & \textbf{0.0258} & 0.00148 & 0.0279 & 0.00150 & 0.0294 & 0.00152 & 0.0289 \\
&720 &\textbf{0.00178} & \textbf{0.0305} & 0.00202 & 0.0328 & 0.00204 & 0.0331 & 0.00209 & 0.0341 \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Traffic}}
&96 &\textbf{0.115} & \textbf{0.183} & 0.118 & 0.194 & 0.120 & 0.199 & 0.134 & 0.223 \\
&192 &\textbf{0.112} & \textbf{0.182} & 0.113 & 0.188 & 0.117 & 0.196 & 0.130 & 0.221 \\
&336 &\textbf{0.113} & \textbf{0.190} & 0.116 & 0.195 & 0.117 & 0.197 & 0.133 & 0.227 \\
&720 &\textbf{0.126} & \textbf{0.204} & 0.132 & 0.214 & 0.133 & 0.217 & 0.146 & 0.241 \\

\midrule
\bottomrule
\end{tabular}
\label{tab:appendix_modules}
}

\end{sc}
% \end{small}
\end{center}
\vskip 0.1in
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
%}

==> tables_vq/ablation_modules_average.tex <==
%\resizebox{!}{\.5\paperheight}{
%\vskip -0.05in
\begin{table}[h]
\centering

%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Ablation study of FFN-free and Sparse-VQ in PatchTST. 4 cases are included: (a) both FFN-free and Sparse-VQ are included in model (SVQ+FFN-f); (b) only Vector Quantization (VQ+FFN-f); (c) only FFN-free(FFN-f);(d) neither of them is included (Original patchTST model). All the results are averaged from 4 different prediction lengths $\in \{96,192,336,720\}$.
%A lower MSE indicates better performance. %Appendix~\ref{subsec_appendix_ablation} shows the full results. 
}\vspace{-3mm}

\begin{center}
% \begin{small}
\begin{sc}
\scalebox{0.70}{
\begin{tabular}{c|cccccccccccccccc}
\toprule
% \multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{PatchTST(96)}&\multicolumn{2}{c|}{Attention}&\multicolumn{2}{c|}{Series-LG/GL}&\multicolumn{2}{c|}{Series-GL}&\multicolumn{2}{c}{Concatenate}\\
{Methods}&\multicolumn{2}{c|}{SVQ+FFN-f}&\multicolumn{2}{c|}{VQ+FFN-f}&\multicolumn{2}{c|}{FFN-f}&\multicolumn{2}{c}{Original}\\
\midrule
{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE\\
\midrule
{ETTm2}
&\textbf{0.111} & \textbf{0.248} & \textbf{0.111} & 0.249 & 0.112 & 0.250 & 0.113 & 0.252 \\


\midrule
{Electricity}
&\textbf{0.245} & \textbf{0.348} & 0.253 & 0.353 & 0.256 & 0.355 & 0.267 & 0.365 \\

\midrule
{Weather}
&\textbf{0.0013} & \textbf{0.0253} & 0.0015 & 0.0280 & 0.0015 & 0.0287 & 0.0016 & 0.0294 \\

\midrule
{Traffic}
&\textbf{0.117} & \textbf{0.190} & 0.120 & 0.199 & 0.122 & 0.202 & 0.136 & 0.228 \\

\midrule
\bottomrule
\end{tabular}
\label{tab:ablation_modules_average}
}

\end{sc}
% \end{small}
\end{center}
\vskip -0.10in
% \end{adjustwidth}
%\end{footnotesize}
\end{table}
%}

==> tables_vq/ablation_noise_VQ.tex <==
%\resizebox{!}{\.5\paperheight}{

\begin{table*}[h]
%\vskip -0.15in
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}

\caption{Robustness analysis of univariate results conducted on four typical datasets. The degree of noise injected into the time series data is determined by $\eta$. A lower MSE indicates better performance. All experiments are repeated 3 times.}\vspace{-1mm}
\begin{center}
\begin{small}
\begin{sc}

\scalebox{1.0}{
\begin{tabular}{c|c|cccccccccccccccccc}
\toprule
\multicolumn{2}{c|}{Sparse-VQ}&\multicolumn{2}{c|}{Original}&\multicolumn{2}{c|}{$\eta=1\%$}&\multicolumn{2}{c|}{$\eta=5\%$}&\multicolumn{2}{c}{$\eta=10\%$}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE & MAE\\
\midrule
\multirow{4}{*}{\rotatebox{90}{ETTm2}} 
&96 &0.063 & 0.183 & 0.065 & 0.188 & 0.067 & 0.193 & 0.069 & 0.197 \\
&192 &0.090 & 0.225 & 0.091 & 0.228 & 0.093 & 0.231 & 0.094 & 0.233 \\
&336 &0.118 & 0.262 & 0.118  & 0.262 & 0.120  & 0.265 & 0.121  & 0.267 \\
&720 &0.172 & 0.322 & 0.173  & 0.323 & 0.174  & 0.323 & 0.173  & 0.323 \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Electricity}} 
&96  &0.196 & 0.306 & 0.198 & 0.309 & 0.202 & 0.303 & 0.209 & 0.322 \\
&192 &0.229 & 0.330 & 0.230 & 0.331 & 0.233 & 0.334 & 0.241 & 0.345 \\
&336 &0.269 & 0.363 & 0.271 & 0.365 & 0.274 & 0.367 & 0.283 & 0.379 \\
&720 &0.317 & 0.413 & 0.316 & 0.415 & 0.322 & 0.420 & 0.328 & 0.425 \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Traffic}} 
&96  &0.118 & 0.194 & 0.118 & 0.195 & 0.124 & 0.209 & 0.127 & 0.213 \\
&192  &0.115 & 0.192 & 0.116 & 0.194 & 0.120 & 0.203 & 0.136 & 0.240 \\
&336  &0.116 & 0.195 & 0.116 & 0.197 & 0.121 & 0.211 & 0.137 & 0.243 \\
&720  &0.132 & 0.214 & 0.132 & 0.217 & 0.136 & 0.226 & 0.153 & 0.259 \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Weather}}
&96  &0.00113 & 0.0252 & 0.00114 & 0.0253 & 0.00116 & 0.0260 & 0.00115 & 0.0256 \\
&192  &0.00128 & 0.0262 & 0.00128 & 0.0262 & 0.00128 & 0.0262 & 0.00128 & 0.0263 \\
&336  &0.00148 & 0.0279 & 0.00148 & 0.0280 & 0.00147 & 0.0280 & 0.00152 & 0.0298 \\
&720  &0.00202 & 0.0328 & 0.00203 & 0.0328 & 0.00202 & 0.0326 & 0.00200 & 0.0329 \\

\midrule
\bottomrule

\end{tabular}

}
\label{tab:ablation_noise_VQ}
\end{sc}
\end{small}
\end{center}
\vskip 0.2in
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
%}

==> tables_vq/ablation_noise_VQ_average.tex <==
%\resizebox{!}{\.5\paperheight}{

\begin{table}[h]
%\vskip -0.02in
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}

\caption{Robustness analysis of univariate results conducted on four typical datasets. The degree of noise injected into the time series data is determined by $\eta$. All the results are
averaged from 4 different prediction lengths $\in \{96, 192, 336, 720\}$.All experiments are repeated 3 times.% Appendix~\ref{subsec_appendix_robustness} shows the full results.
}\vspace{-2mm}
\begin{center}
\begin{small}
\begin{sc}

\scalebox{0.85}{
\begin{tabular}{c|cccccccccccccccccc}
\toprule
{VQ}&\multicolumn{2}{c|}{Original}&\multicolumn{2}{c|}{$\eta=1\%$}&\multicolumn{2}{c|}{$\eta=5\%$}&\multicolumn{2}{c}{$\eta=10\%$}\\
\midrule
{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE & MAE\\
\midrule
{ETTm2}
&0.111	&0.248	&0.112	&0.250	&0.114	&0.253	&0.114	&0.255\\

\midrule
{Electricity}
&0.253	&0.353	&0.254	&0.355	&0.258	&0.356	&0.265	&0.368 \\

\midrule
{Traffic}
&0.120	&0.199	&0.121	&0.201	&0.125	&0.212	&0.138	&0.239 \\

\midrule
{Weather}
&0.0015	&0.028	&0.0015	&0.028	&0.0015	&0.0282	&0.0015	&0.029 \\

\midrule
\bottomrule

\end{tabular}

}
\label{tab:ablation_noise_VQ_average}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
% \end{adjustwidth}
%\end{footnotesize}
\end{table}
%}

==> tables_vq/ablation_vq_boosting.tex <==
%\resizebox{!}{\.5\paperheight}{

\begin{table*}[h]
%\vskip -0.15in
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}

\caption{Results for boosting effect of sparse-VQ. We use FEDformer and Autoformer as backbones and leverage them with the Sparse-VQ. A lower MSE indicates better performance. All experiments are repeated 3 times.}%\vspace{-1mm}
\begin{center}
\begin{small}
\begin{sc}

\scalebox{1.0}{
\begin{tabular}{c|c|ccccccccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FEDformer}&\multicolumn{2}{c|}{FEDformer+SVQ}&\multicolumn{2}{c|}{Autoformer}&\multicolumn{2}{c}{Autoformer+SVQ}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE & MAE\\
\midrule
\multirow{4}{*}{\rotatebox{90}{ETTm2}} 
&96 &0.203 & 0.287 & \textbf{0.192} & \textbf{0.286} & 0.255 & 0.339 & \textbf{0.214} & \textbf{0.295} \\
&192 &0.269 & \textbf{0.328} & \textbf{0.263} & \textbf{0.328} & 0.281 & 0.340 & \textbf{0.271} & \textbf{0.328} \\
&336 &\textbf{0.325} & 0.366 & \textbf{0.325} & \textbf{0.365} & 0.339 & 0.372 & \textbf{0.326} & \textbf{0.365} \\
&720 &\textbf{0.421} & \textbf{0.415} &0.432 & 0.424 & 0.422 & 0.419 & \textbf{0.412} & \textbf{0.410} \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Electricity}} 
&96  &0.193 & 0.308 & \textbf{0.186} & \textbf{0.301} & 0.201 & 0.317 & \textbf{0.199} & \textbf{0.310} \\
&192  &0.201 & 0.315 & \textbf{0.197} & \textbf{0.311} & \textbf{0.222} & \textbf{0.334} & 0.235 & 0.341 \\
&336  &\textbf{0.214} & \textbf{0.329} & 0.218 & 0.333 & 0.231 & 0.338 & \textbf{0.226} & \textbf{0.337} \\
&720  &0.246 & 0.355 & \textbf{0.234} & \textbf{0.346} & \textbf{0.254} & 0.361 & 0.267 & \textbf{0.342} \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Traffic}} 
&96  &0.587 & 0.366 & \textbf{0.569} & \textbf{0.354} & 0.613 & 0.388 & \textbf{0.595} & \textbf{0.366} \\
&192  &\textbf{0.604} & \textbf{0.373} & 0.611 & 0.378 & 0.616 & 0.382 & \textbf{0.592} & \textbf{0.365} \\
&336  &0.621 & 0.383 & \textbf{0.615} & \textbf{0.377} & 0.622 & 0.337 & \textbf{0.611} & \textbf{0.336} \\
&720  &\textbf{0.626} & \textbf{0.382} & 0.630 & 0.383 & \textbf{0.660} & \textbf{0.408} & 0.703 & 0.450 \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Weather}}
&96 &0.217 & \textbf{0.296} & \textbf{0.209} & \textbf{0.296} & 0.266 & 0.336 & \textbf{0.224} & \textbf{0.299} \\
&192  &0.276 & 0.336 & \textbf{0.270} & \textbf{0.332} & 0.307 & 0.367 & \textbf{0.280} & \textbf{0.354} \\
&336  &0.339 & 0.38  & \textbf{0.319} & \textbf{0.375} & 0.359 & 0.395 & \textbf{0.330} & \textbf{0.372} \\
&720  &0.403 & 0.428 & \textbf{0.385} & \textbf{0.390} & 0.419 & 0.428 & \textbf{0.397} & \textbf{0.399} \\
\midrule
\bottomrule
\end{tabular}
\label{tab:ablation_vq_boosting}
}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
%}

==> tables_vq/ablation_vq_boosting_average.tex <==
%\resizebox{!}{\.5\paperheight}{

\begin{table}[h]
\vskip -0.02in
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}

\caption{Results for boosting effect of sparse-VQ.  All the results are averaged from 4 different prediction lengths $\in \{96, 192, 336, 720\}$. We use FEDformer and Autoformer as backbones and leverage them with the Sparse-VQ. %A lower MSE indicates better performance. All experiments are repeated 3 times. %Appendix~\ref{subsec_appendix_ablation} shows the full results.
}
\vspace{-0.9mm}
\begin{center}
\begin{small}
\begin{sc}

\scalebox{0.75}{
\begin{tabular}{c|ccccccccccccccc}
\toprule
{Methods}&\multicolumn{2}{c|}{FEDformer}&\multicolumn{2}{c|}{FED + SVQ}&\multicolumn{2}{c|}{Autoformer}&\multicolumn{2}{c}
{Auto + SVQ}\\
\midrule
{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE & MAE\\
\midrule
{ETTm2}
 &0.305 & \textbf{0.349} &\textbf{0.303} & 0.351 & 0.324 & 0.368 & \textbf{0.306} & \textbf{0.350} \\

\midrule
{Electricity}
 &0.214 & 0.327 & \textbf{0.209} & \textbf{0.323} & \textbf{0.227} & 0.338 & 0.232 & \textbf{0.333} \\

\midrule
{Traffic}
 &0.610 &0.376 & \textbf{0.606} & \textbf{0.373} & 0.628 & \textbf{0.379} & \textbf{0.625} & 0.389 \\

\midrule
{Weather}
 &0.309 & 0.360 & \textbf{0.296} & \textbf{0.348} & 0.338 & 0.382 & \textbf{0.308} & \textbf{0.356} \\
\midrule
\bottomrule
\end{tabular}
\label{tab:ablation_vq_boosting_average}
}
\end{sc}
\end{small}
\end{center}
%\vskip -0.2in
% \end{adjustwidth}
%\end{footnotesize}
\end{table}
%}

==> tables_vq/dataset.tex <==
\begin{table}[h]
%\color{blue}
\caption{Details of ten benchmark datasets.}
\label{tab:dataset}
%\vspace{-2mm}
\vskip -0.5in
\begin{center}
\begin{small}
\begin{sc}
\scalebox{0.90}{
\begin{tabular}{l|cccr}
\toprule
% Dataset & num & dim & freq \\
Dataset & Length & Dimension & Frequency \\
\midrule
ETTm2 & 69680$\approx$2 years & 7 & 15 min\\
%ETTh1/h2 & 17420$\approx$2 years & 7 & 1h\\
Electricity & 26304$\approx$3 years & 321 & 1h & \\
Traffic & 17544$\approx$2 years & 862 & 1h & \\
Weather & 52696$\approx$1 years & 21 & 10 min & \\
Wind & 48673$\approx$1 years & 7 & 15min & \\
Nordpool & 70128$\approx$8 years & 18 & 1h & \\
Caiso & 74472$\approx$8 years & 10 & 1h & \\
\midrule

\bottomrule
\end{tabular}
}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
%\vskip -0.1in
\end{table}

==> tables_vq/different_vq_strcture_concise.tex <==
%\resizebox{!}{\.5\paperheight}{
% \vskip -0.2in
\begin{table*}[t]
\centering

%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Univariate long-term series forecasting results of different sturcture of VQ. The best results are in bold. A lower MSE indicates better performance.The results are averaged from 4 different prediction lengths $\in \{96, 192, 336, 720\}$.% Appendix~\ref{appendix_various_vq} shows the full results.
}\vspace{-2mm}

\begin{center}
% \begin{small}
\begin{sc}
\scalebox{0.80}{
\begin{tabular}{c|ccccccccccccccccc}
\toprule
% \multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{PatchTST(96)}&\multicolumn{2}{c|}{Attention}&\multicolumn{2}{c|}{Series-LG/GL}&\multicolumn{2}{c|}{Series-GL}&\multicolumn{2}{c}{Concatenate}\\
Methods&\multicolumn{2}{c|}{$Sparse-VQ$}&\multicolumn{2}{c|}{$VQ$}&\multicolumn{2}{c|}{$VQ_{cosine}$}&\multicolumn{2}{c|}{$VQ_{kmeans}$}&\multicolumn{2}{c|}{$VQ_{recursive}$}&\multicolumn{2}{c}{$VQ_{AdaptiveCodebook}$}\\
\midrule
Metric & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE & MSE  & MAE\\
\midrule
ECL & \textbf{0.245} & \textbf{0.348} & 0.257  & 0.355   & 0.265  & 0.365  & 0.263           & 0.358      & 0.258   & 0.357    & 0.260          & 0.358      \\
 
 
\midrule
Traffic& \textbf{0.117} & \textbf{0.190} & 0.118  & 0.193   & 0.123  & 0.202  & 0.120           & 0.193      & 0.122   & 0.199     & \textbf{0.117} & 0.191      \\
 
 
\midrule
Weather& 0.0013         & \textbf{0.025} & 0.0013 & 0.0252   & 0.0013 & 0.0259 & \textbf{0.0012} & \textbf{0.025} & 0.0012 & 0.025   & 0.0013    & \textbf{0.025}   \\
 


\midrule
\bottomrule
\end{tabular}
\label{tab:different_vq_structure_concise}
}

\end{sc}
% \end{small}
\end{center}
\vskip -0.05in
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
%}

==> tables_vq/different_vq_structure.tex <==
%\resizebox{!}{\.5\paperheight}{
% \vskip -0.2in
\begin{table*}[t]
\centering

%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Univariate long-term series forecasting results of different sturcture of VQ. The best results are in bold. A lower MSE indicates better performance. All experiments are repeated 3 times.}\vspace{-1mm}

\begin{center}
% \begin{small}
\begin{sc}
\scalebox{0.80}{
\begin{tabular}{c|c|cccccccccccccccc}
\toprule
% \multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{PatchTST(96)}&\multicolumn{2}{c|}{Attention}&\multicolumn{2}{c|}{Series-LG/GL}&\multicolumn{2}{c|}{Series-GL}&\multicolumn{2}{c}{Concatenate}\\
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{$Sparse-VQ$}&\multicolumn{2}{c|}{$VQ$}&\multicolumn{2}{c|}{$VQ_{cosine}$}&\multicolumn{2}{c|}{$VQ_{kmeans}$}&\multicolumn{2}{c|}{$VQ_{recursive}$}&\multicolumn{2}{c}{$VQ_{AdaptiveCodebook}$}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE & MSE  & MAE\\
\midrule
\multirow{5}{*}{\rotatebox{90}{ECL}} 

 & 96  & 0.194          & 0.304          & 0.199  & 0.308   & 0.203  & 0.314  & 0.198           & 0.307     & 0.201   & 0.310    & 0.202          & 0.309       \\
 & 192 & 0.226          & 0.325          & 0.232  & 0.330    & 0.242  & 0.342  & 0.232           & 0.331     & 0.233   & 0.334     & 0.233          & 0.333    \\
 & 336 & 0.263          & 0.358          & 0.273  & 0.365    & 0.280  & 0.377  & 0.302           & 0.376       & 0.274   & 0.365  & 0.275          & 0.365     \\
 & 720 & 0.298          & 0.404          & 0.322  & 0.417    & 0.335  & 0.426  & 0.321           & 0.417     & 0.323   & 0.419     & 0.328          & 0.424      \\
 & Avg & \textbf{0.245} & \textbf{0.348} & 0.257  & 0.355   & 0.265  & 0.365  & 0.263           & 0.358      & 0.258   & 0.357    & 0.260          & 0.358      \\
 
 
\midrule
\multirow{5}{*}{\rotatebox{90}{Traffic}}
 & 96  & 0.115          & 0.183          & 0.116  & 0.186    & 0.119  & 0.193  & 0.117           & 0.186     & 0.118   & 0.190   & 0.115          & 0.182       \\
 & 192 & 0.112          & 0.182          & 0.113  & 0.185    & 0.118  & 0.194  & 0.113           & 0.185     & 0.116   & 0.191      & 0.111          & 0.184      \\
 & 336 & 0.113          & 0.190          & 0.113  & 0.194  & 0.118  & 0.201  & 0.115           & 0.190      & 0.116   & 0.196     & 0.114          & 0.192        \\
 & 720 & 0.126          & 0.204          & 0.129  & 0.208    & 0.136  & 0.221  & 0.133           & 0.211     & 0.137   & 0.220     & 0.127          & 0.205      \\
 & Avg & \textbf{0.117} & \textbf{0.190} & 0.118  & 0.193   & 0.123  & 0.202  & 0.120           & 0.193      & 0.122   & 0.199     & \textbf{0.117} & 0.191      \\
 
 
\midrule
\multirow{5}{*}{\rotatebox{90}{Weather}}
 & 96  & 0.0009         & 0.0210         & 0.0009 & 0.0212  & 0.0009 & 0.0218 & 0.0009          & 0.0211     & 0.0009  & 0.0214   & 0.0009         & 0.0212     \\
 & 192 & 0.0011         & 0.0239         & 0.0011 & 0.0235  & 0.0011 & 0.0240 & 0.0010          & 0.0235     & 0.0011  & 0.0238    & 0.0011         & 0.0233     \\
 & 336 & 0.0013         & 0.0258         & 0.0012 & 0.0255  & 0.0013 & 0.0261 & 0.0012          & 0.0255     & 0.0012  & 0.0258   & 0.0013         & 0.0257     \\
 & 720 & 0.0018         & 0.0305         & 0.0018 & 0.0304  & 0.0019 & 0.0316 & 0.0017          & 0.0303    & 0.0017  & 0.0302    & 0.0018         & 0.0305     \\
 & Avg & 0.0013         & \textbf{0.025} & 0.0013 & 0.0252   & 0.0013 & 0.0259 & \textbf{0.0012} & \textbf{0.025} & 0.0012 & 0.025   & 0.0013    & \textbf{0.025}   \\
 


\midrule
\bottomrule
\end{tabular}
\label{tab:different_vq_structure}
}

\end{sc}
% \end{small}
\end{center}
\vskip -0.15in
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
%}

==> tables_vq/few_shot_10.tex <==
%\resizebox{!}{\.5\paperheight}{
% \vskip -0.2in
\begin{table*}[t]
\centering
\begin{sc}

% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Few-shot learning results on 10\% data. We use prediction length $O \in {96, 192, 336, 720}$.A lower MSE indicates better performance, and the best results are highlighted in bold. ’-’ means that 10\% time series is not sufficient to constitute a training set.}\vspace{-1mm}
\scalebox{0.75}{
\begin{tabular}{c|c|ccccccccccccccccccc}

\toprule
\multicolumn{2}{c|}{Methods} &\multicolumn{2}{c|}{SVQ} &\multicolumn{2}{c|}{PatchTST} &\multicolumn{2}{c|}{OFA}  &\multicolumn{2}{c|}{Dlinear}  &\multicolumn{2}{c|}{FEDformer} &\multicolumn{2}{c|}{Autoformer} &\multicolumn{2}{c|}{Informer} &\multicolumn{2}{c|}{LogTrans} &\multicolumn{2}{c|}{Reformer}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE & MSE  & MAE & MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE & MSE  & MAE & MSE & MAE \\
\midrule
\multirow{5}{*}{\rotatebox{90}{ETTm1}} 
 & 96  & 0.333          & 0.365          & 0.41  & 0.419 & 0.39  & 0.404  & 0.352 & 0.392 & 0.578 & 0.518  & 0.774 & 0.614 & 1.162 & 0.785 & 1.555 & 0.910 & 1.442 & 0.847 \\
 & 192 & 0.370          & 0.388          & 0.437 & 0.434 & 0.429 & 0.423  & 0.382 & 0.412 & 0.617 & 0.546  & 0.754 & 0.592 & 1.172 & 0.793 & 1.883 & 1.033 & 1.444 & 0.862 \\
 & 336 & 0.413          & 0.416          & 0.476 & 0.454 & 0.469 & 0.439  & 0.419 & 0.434 & 0.998 & 0.775  & 0.869 & 0.677 & 1.227 & 0.908 & 2.095 & 1.110 & 1.45  & 0.866 \\
 & 720 & 0.476          & 0.452          & 0.681 & 0.556 & 0.569 & 0.498  & 0.49  & 0.477 & 0.693 & 0.579  & 0.81  & 0.63  & 1.207 & 0.797 & 2.389 & 1.167 & 1.366 & 0.85  \\
 & Avg & \textbf{0.398} & \textbf{0.405} & 0.501 & 0.466 & 0.464 & 0.441  & 0.411 & 0.429 & 0.722 & 0.605  & 0.802 & 0.628 & 1.192 & 0.821 & 1.981 & 1.055 & 1.426 & 0.856 \\


\midrule
\multirow{5}{*}{\rotatebox{90}{Electricity}} 
 & 96  & 0.145          & 0.243          & 0.14  & 0.238 & 0.139 & 0.237  & 0.15  & 0.253 & 0.231 & 0.323  & 0.261 & 0.348 & 1.259 & 0.919 & 0.649 & 0.584 & 0.993 & 0.784 \\
 & 192 & 0.162          & 0.259          & 0.16  & 0.255 & 0.156 & 0.252  & 0.164 & 0.264 & 0.261 & 0.356  & 0.338 & 0.406 & 1.16  & 0.873 & 0.667 & 0.594 & 0.938 & 0.753 \\
 & 336 & 0.188          & 0.284          & 0.18  & 0.276 & 0.175 & 0.27   & 0.181 & 0.282 & 0.36  & 0.445  & 0.41  & 0.474 & 1.157 & 0.872 & 0.711 & 0.620 & 0.925 & 0.745 \\
 & 720 & 0.245          & 0.325          & 0.241 & 0.323 & 0.233 & 0.317  & 0.223 & 0.321 & 0.53  & 0.585  & 0.715 & 0.685 & 1.203 & 0.898 & 0.833 & 0.690 & 1.004 & 0.79  \\
 & Avg & \textbf{0.185} & \textbf{0.278} & 0.18  & 0.273 & 0.176 & 0.269  & 0.18  & 0.28  & 0.346 & 0.427  & 0.431 & 0.478 & 1.195 & 0.891 & 0.715 & 0.622 & 0.965 & 0.768 \\


\midrule
\multirow{5}{*}{\rotatebox{90}{Traffic}}
 & 96  & 0.409          & 0.272          & 0.403 & 0.289 & 0.414 & 0.297  & 0.419 & 0.298 & 0.639 & 0.4    & 0.672 & 0.405 & 1.557 & 0.821 & 0.928 & 0.513 & 1.527 & 0.815 \\
 & 192 & 0.423          & 0.275          & 0.415 & 0.296 & 0.426 & 0.301  & 0.434 & 0.305 & 0.637 & 0.416  & 0.727 & 0.424 & 1.454 & 0.765 & 0.976 & 0.530 & 1.538 & 0.817 \\
 & 336 & 0.428          & 0.279          & 0.426 & 0.304 & 0.434 & 0.303  & 0.449 & 0.313 & 0.655 & 0.427  & 0.749 & 0.454 & 1.521 & 0.812 & 1.015 & 0.545 & 1.55  & 0.819 \\
 & 720 & 0.445          & 0.296          & 0.474 & 0.331 & 0.487 & 0.337  & 0.484 & 0.336 & 0.722 & 0.456  & 0.847 & 0.499 & 1.605 & 0.846 & 1.162 & 0.607 & 1.588 & 0.833 \\
 & Avg & \textbf{0.426} & \textbf{0.281} & 0.430 & 0.305 & 0.44  & 0.31   & 0.447 & 0.313 & 0.663 & 0.425  & 0.749 & 0.446 & 1.534 & 0.811 & 1.020 & 0.549 & 1.551 & 0.821 \\

 
 
\midrule
\multirow{5}{*}{\rotatebox{90}{Weather}} 
& 96  & 0.152          & 0.196          & 0.165 & 0.215 & 0.163 & 0.215  & 0.171 & 0.224 & 0.188 & 0.253  & 0.221 & 0.297 & 0.374 & 0.401 & 0.305 & 0.371 & 0.335 & 0.38  \\
 & 192 & 0.201          & 0.241          & 0.21  & 0.257 & 0.21  & 0.254  & 0.215 & 0.263 & 0.25  & 0.304  & 0.27  & 0.322 & 0.552 & 0.478 & 0.425 & 0.432 & 0.522 & 0.462 \\
 & 336 & 0.252          & 0.282          & 0.259 & 0.297 & 0.256 & 0.292  & 0.258 & 0.299 & 0.312 & 0.346  & 0.32  & 0.351 & 0.724 & 0.541 & 0.605 & 0.500 & 0.715 & 0.535 \\
 & 720 & 0.325          & 0.335          & 0.332 & 0.346 & 0.321 & 0.339  & 0.32  & 0.346 & 0.387 & 0.393  & 0.39  & 0.396 & 0.739 & 0.558 & 0.714 & 0.536 & 0.611 & 0.5   \\
 & Avg & \textbf{0.233} & \textbf{0.264} & 0.242 & 0.279 & 0.238 & 0.275  & 0.241 & 0.283 & 0.284 & 0.324  & 0.3   & 0.342 & 0.597 & 0.495 & 0.512 & 0.460 & 0.546 & 0.469 \\


\midrule
\multirow{5}{*}{\rotatebox{90}{Wind}}  
 & 96  & 0.907          & 0.627          & 1.070 & 0.717 & 1.075 & 0.718  & 1.012 & 0.697 & 1.490 & 0.911  & 1.464 & 0.905 & 5.424 & 1.935 & 3.858 & 1.649 & 2.570 & 1.331 \\
 & 192 & 1.150          & 0.757          & 1.331 & 0.836 & 1.342 & 0.843  & 1.266 & 0.820 & 1.671 & 0.977  & 1.850 & 1.047 & 4.793 & 1.823 & 3.062 & 1.440 & 2.953 & 1.439 \\
 & 336 & 1.398          & 0.869          & 1.574 & 0.937 & 1.545 & 0.928  & 1.474 & 0.911 & 1.822 & 1.041  & 1.976 & 1.101 & 4.313 & 1.740 & 3.111 & 1.467 & 2.923 & 1.428 \\
 & 720 & 1.606          & 0.957          & 1.743 & 1.005 & 1.749 & 1.004  & 1.635 & 0.975 & 1.836 & 1.056  & 1.947 & 1.084 & 3.976 & 1.662 & 3.069 & 1.456 & 2.975 & 1.440 \\
 & Avg & \textbf{1.265} & \textbf{0.803} & 1.430 & 0.874 & 1.428 & 0.873  & 1.347 & 0.851 & 1.705 & 0.996  & 1.809 & 1.034 & 4.627 & 1.790 & 3.275 & 1.503 & 2.855 & 1.410 \\

\midrule
\multirow{5}{*}{\rotatebox{90}{Nordpool}} 
 & 96  & 0.554          & 0.545          & 0.631 & 0.591 & 0.638 & 0.594  & 0.629 & 0.595 & 0.789 & 0.694  & 0.888 & 0.737 & 2.247 & 1.190 & 1.889 & 1.116 & 1.876 & 1.102 \\
 & 192 & 0.613          & 0.582          & 0.707 & 0.636 & 0.704 & 0.633  & 0.687 & 0.635 & 0.734 & 0.673  & 1.031 & 0.798 & 2.400 & 1.240 & 2.052 & 1.141 & 2.055 & 1.140 \\
 & 336 & 0.594          & 0.581          & 0.674 & 0.626 & 0.679 & 0.627  & 0.678 & 0.635 & 0.756 & 0.680  & 0.860 & 0.727 & 2.484 & 1.267 & 2.022 & 1.121 & 2.175 & 1.175 \\
 & 720 & 0.577          & 0.578          & 0.660 & 0.626 & 0.674 & 0.632  & 0.677 & 0.638 & 0.812 & 0.707  & 0.938 & 0.758 & 2.579 & 1.385 & 1.641 & 1.013 & 2.161 & 1.178 \\
 & Avg & \textbf{0.585} & \textbf{0.572} & 0.668 & 0.620 & 0.674 & 0.6215 & 0.668 & 0.626 & 0.773 & 0.689  & 0.929 & 0.755 & 2.428 & 1.271 & 1.901 & 1.098 & 2.067 & 1.149 \\

\midrule
\multirow{5}{*}{\rotatebox{90}{Caiso}} 
 & 96  & 0.210          & 0.290          & 0.246 & 0.328 & 0.243 & 0.329  & 0.247 & 0.329 & 0.499 & 0.514  & 0.664 & 0.607 & 1.641 & 0.902 & 1.229 & 0.808 & 1.226 & 0.790 \\
 & 192 & 0.285          & 0.349          & 0.320 & 0.382 & 0.317 & 0.382  & 0.315 & 0.380 & 0.539 & 0.534  & 0.835 & 0.671 & 1.801 & 0.945 & 1.269 & 0.820 & 1.317 & 0.822 \\
 & 336 & 0.334          & 0.384          & 0.377 & 0.421 & 0.376 & 0.421  & 0.365 & 0.413 & 0.634 & 0.583  & 0.795 & 0.655 & 2.076 & 1.026 & 1.442 & 0.858 & 1.401 & 0.846 \\
 & 720 & 0.436          & 0.444          & 0.525 & 0.509 & 0.547 & 0.523  & 0.494 & 0.499 & 0.807 & 0.667  & 0.884 & 0.705 & 2.361 & 1.230 & 1.560 & 0.891 & 1.735 & 0.942 \\
 & Avg & \textbf{0.316} & \textbf{0.367} & 0.367 & 0.41  & 0.371 & 0.414  & 0.355 & 0.405 & 0.620 & 0.5745 & 0.795 & 0.660 & 1.970 & 1.026 & 1.375 & 0.844 & 1.420 & 0.85\\ 
 
\midrule

%\multicolumn{2}{c|}{Average}& \textbf{0.308} & \textbf{0.305} 0.371 &0.367 &0.385  &0.376&0.511 &0.472 &0.687 &0.559 &0.674 &0.522 &0.912 &0.665 &1.137 &0.712 &1.850 &0.967 &1.888 &0.974  \\

% \midrule
% \multicolumn{2}{c|}{Average} & & & & & & & & & & & & & & & \\
\bottomrule
\end{tabular}
\label{tab:few_shot_10}
}
% \end{adjustwidth}
\vskip 0.1in
%\vskip -0.1in
\end{sc}
\end{table*}
%}

==> tables_vq/few_shot_5.tex <==
%\resizebox{!}{\.5\paperheight}{
% \vskip -0.2in
\begin{table*}[t]
\centering
\begin{sc}

% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Few-shot learning results on 5\% data. All the results are averaged from 4 different prediction lengths $O \in {96, 192, 336, 720}$.A lower MSE indicates better performance, and the best results are highlighted in bold. ’-’ means that 5\% time series is not sufficient to constitute a training set.}\vspace{-1mm}
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccccccccccccc}

\toprule
\multicolumn{2}{c|}{Methods} &\multicolumn{2}{c|}{SVQ} &\multicolumn{2}{c|}{PatchTST} &\multicolumn{2}{c|}{OFA}  &\multicolumn{2}{c|}{Dlinear}  &\multicolumn{2}{c|}{FEDformer} &\multicolumn{2}{c|}{Autoformer} &\multicolumn{2}{c|}{Informer} &\multicolumn{2}{c|}{LogTrans} &\multicolumn{2}{c|}{Reformer}\\

\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE & MSE  & MAE & MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE & MSE  & MAE & MSE & MAE\\
\midrule
\multirow{5}{*}{\rotatebox{90}{ETTm1}} 

&96  & 0.332  & 0.369   & 0.399 & 0.414 & 0.386 & 0.405 & 0.332 & 0.374 & 0.628 & 0.544 & 0.726 & 0.578 & 1.13  & 0.775 & 1.446 & 0.928 & 1.234 & 0.798 \\
&192 & 0.376  & 0.398   & 0.441 & 0.436 & 0.44  & 0.438 & 0.358 & 0.39  & 0.666 & 0.566 & 0.75  & 0.591 & 1.15  & 0.788 & 1.519 & 0.962 & 1.287 & 0.839 \\
&336 & 0.425  & 0.423   & 0.499 & 0.467 & 0.485 & 0.459 & 0.402 & 0.416 & 0.807 & 0.628 & 0.851 & 0.659 & 1.198 & 0.809 & 1.774 & 1.032 & 1.288 & 0.842 \\
&720 & 0.486  & 0.458   & 0.767 & 0.587 & 0.577 & 0.499 & 0.511 & 0.489 & 0.822 & 0.633 & 0.857 & 0.655 & 1.175 & 0.794 & 1.647 & 0.994 & 1.247 & 0.828 \\
&Avg & \textbf{0.405}  & \textbf{0.412}   & 0.526 & 0.476 & 0.472 & 0.45  & 0.400 & 0.417 & 0.73  & 0.592 & 0.796 & 0.62  & 1.163 & 0.791 & 1.597 & 0.979 & 1.264 & 0.826 \\


\midrule
\multirow{5}{*}{\rotatebox{90}{Electricity}} 
&96  & 0.147  & 0.246   & 0.145 & 0.244 & 0.143 & 0.241 & 0.15  & 0.251 & 0.235 & 0.322 & 0.297 & 0.367 & 1.265 & 0.919 & 0.816 & 0.687 & 1.414 & 0.855 \\
&192 & 0.164  & 0.262   & 0.163 & 0.26  & 0.159 & 0.255 & 0.163 & 0.263 & 0.247 & 0.341 & 0.308 & 0.375 & 1.298 & 0.939 & 0.778 & 0.666 & 1.24  & 0.919 \\
&336 & 0.189  & 0.285   & 0.183 & 0.281 & 0.179 & 0.274 & 0.175 & 0.278 & 0.267 & 0.356 & 0.354 & 0.411 & 1.302 & 0.942 & 0.889 & 0.717 & 1.253 & 0.921 \\
&720 & 0.242  & 0.334   & 0.233 & 0.323 & 0.233 & 0.323 & 0.219 & 0.311 & 0.318 & 0.394 & 0.426 & 0.466 & 1.259 & 0.919 & 1.251 & 0.912 & 1.249 & 0.921 \\
&Avg & \textbf{0.185} & \textbf{0.281} & 0.181 & 0.277 & 0.178 & 0.273 & 0.176 & 0.275 & 0.266 & 0.353 & 0.346 & 0.404 & 1.281 & 0.929 & 0.934 & 0.746 & 1.289 & 0.904 \\

\midrule
\multirow{5}{*}{\rotatebox{90}{Traffic}} 
&96  & 0.413  & 0.279   & 0.404 & 0.286 & 0.419 & 0.298 & 0.427 & 0.304 & 0.67  & 0.421 & 0.795 & 0.481 & 1.557 & 0.821 & 1.149 & 0.599 & 1.586 & 0.841 \\
&192 & 0.425  & 0.287   & 0.412 & 0.294 & 0.434 & 0.305 & 0.447 & 0.315 & 0.653 & 0.405 & 0.837 & 0.503 & 1.596 & 0.834 & 1.247 & 0.657 & 1.602 & 0.844 \\
&336 & 0.440  & 0.297   & 0.439 & 0.31  & 0.449 & 0.313 & 0.478 & 0.333 & 0.707 & 0.445 & 0.867 & 0.523 & 1.621 & 0.841 & 1.531 & 0.799 & 1.668 & 0.868 \\
&720 & -      & -       & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     & -     \\
&Avg & \textbf{0.426}  & \textbf{0.288}   & 0.418 & 0.296 & 0.434 & 0.305 & 0.45  & 0.317 & 0.676 & 0.423 & 0.833 & 0.502 & 1.591 & 0.832 & 1.309 & 0.685 & 1.618 & 0.851 \\


\midrule
\multirow{5}{*}{\rotatebox{90}{Weather}}
&96  & 0.161  & 0.205   & 0.171 & 0.224 & 0.175 & 0.23  & 0.184 & 0.242 & 0.229 & 0.309 & 0.227 & 0.299 & 0.497 & 0.497 & 0.356 & 0.408 & 0.406 & 0.435 \\
&192 & 0.219  & 0.256   & 0.23  & 0.277 & 0.227 & 0.276 & 0.228 & 0.283 & 0.265 & 0.317 & 0.278 & 0.333 & 0.62  & 0.545 & 0.489 & 0.479 & 0.446 & 0.45  \\
&336 & 0.289  & 0.308   & 0.294 & 0.326 & 0.286 & 0.322 & 0.279 & 0.322 & 0.353 & 0.392 & 0.351 & 0.393 & 0.649 & 0.547 & 0.517 & 0.482 & 0.465 & 0.459 \\
&720 & 0.361  & 0.361   & 0.384 & 0.387 & 0.366 & 0.379 & 0.364 & 0.388 & 0.391 & 0.394 & 0.387 & 0.389 & 0.57  & 0.522 & 0.465 & 0.463 & 0.471 & 0.468 \\
&Avg & \textbf{0.258}  & \textbf{0.283}   & 0.269 & 0.303 & 0.263 & 0.301 & 0.263 & 0.308 & 0.309 & 0.353 & 0.31  & 0.353 & 0.584 & 0.527 & 0.457 & 0.458 & 0.447 & 0.453 \\

\midrule
\multirow{5}{*}{\rotatebox{90}{Wind}}
&96  & 1.131  & 0.735   & 1.109 & 0.739 & 1.139 & 0.754 & 1.058 & 0.720 & 1.503 & 0.922 & 1.609 & 0.948 & 5.978 & 1.939 & 4.573 & 1.661 & 2.290 & 1.244 \\
&192 & 1.150  & 0.757   & 1.417 & 0.873 & 1.434 & 0.873 & 1.328 & 0.846 & 1.682 & 0.982 & 1.824 & 1.014 & 4.340 & 1.665 & 4.390 & 1.665 & 2.575 & 1.312 \\
&336 & 1.398  & 0.869   & 1.595 & 0.947 & 1.614 & 0.954 & 1.484 & 0.917 & 1.833 & 1.040 & 2.069 & 1.094 & 3.662 & 1.540 & 3.620 & 1.539 & 2.715 & 1.350 \\
&720 & 1.606  & 0.957   & 1.755 & 1.008 & 1.767 & 1.012 & 1.712 & 0.994 & 1.944 & 1.075 & 2.069 & 1.096 & 2.751 & 1.343 & 2.806 & 1.368 & 2.797 & 1.372 \\
&Avg & \textbf{1.321}  & \textbf{0.830}   & 1.469 & 0.892 & 1.489 & 0.898 & 1.396 & 0.869 & 1.741 & 1.005 & 1.893 & 1.038 & 4.183 & 1.622 & 3.847 & 1.558 & 2.594 & 1.320 \\

\midrule
\multirow{5}{*}{\rotatebox{90}{Nordpool}}
&96  & 0.554  & 0.545   & 0.668 & 0.610 & 0.687 & 0.619 & 0.659 & 0.612 & 0.936 & 0.751 & 0.952 & 0.763 & 4.267 & 1.690 & 2.675 & 1.335 & 1.929 & 1.121 \\
&192 & 0.613  & 0.582   & 0.729 & 0.647 & 0.766 & 0.661 & 0.728 & 0.650 & 0.923 & 0.752 & 1.052 & 0.809 & 3.568 & 1.535 & 2.195 & 1.202 & 2.015 & 1.149 \\
&336 & 0.719  & 0.647   & 0.721 & 0.649 & 0.766 & 0.665 & 0.728 & 0.659 & 0.959 & 0.775 & 1.069 & 0.815 & 2.552 & 1.287 & 1.976 & 1.133 & 2.012 & 1.149 \\
&720 & 0.728  & 0.658   & 0.724 & 0.660 & 0.789 & 0.680 & 0.725 & 0.662 & 0.999 & 0.787 & 0.904 & 0.750 & 2.246 & 1.206 & 1.836 & 1.083 & 2.004 & 1.150 \\
&Avg & \textbf{0.654}  & \textbf{0.608}   & 0.711 & 0.642 & 0.752 & 0.656 & 0.71  & 0.646 & 0.954 & 0.766 & 0.994 & 0.784 & 3.158 & 1.430 & 2.171 & 1.188 & 1.99  & 1.142 \\


\midrule
\multirow{5}{*}{\rotatebox{90}{Caiso}}
&96  & 0.209  & 0.289   & 0.262 & 0.344 & 0.269 & 0.357 & 0.262 & 0.346 & 0.515 & 0.529 & 0.636 & 0.595 & 1.485 & 0.879 & 1.452 & 0.875 & 1.290 & 0.812 \\
&192 & 0.285  & 0.347   & 0.330 & 0.393 & 0.323 & 0.393 & 0.327 & 0.394 & 0.579 & 0.562 & 0.680 & 0.610 & 1.721 & 0.949 & 1.586 & 0.902 & 1.405 & 0.850 \\
&336 & 0.348  & 0.386   & 0.388 & 0.435 & 0.379 & 0.433 & 0.378 & 0.431 & 0.651 & 0.601 & 0.699 & 0.613 & 1.829 & 0.977 & 1.643 & 0.905 & 1.465 & 0.876 \\
&720 & 0.432  & 0.442   & 0.564 & 0.533 & 0.558 & 0.539 & 0.560 & 0.534 & 0.866 & 0.703 & 0.901 & 0.712 & 2.106 & 1.057 & 1.975 & 1.006 & 1.573 & 0.909 \\
&Avg & \textbf{0.319}  & \textbf{0.366}   & 0.386 & 0.426 & 0.382 & 0.431 & 0.382 & 0.426 & 0.653 & 0.599 & 0.729 & 0.633 & 1.785 & 0.966 & 1.664 & 0.922 & 1.433 & 0.862\\

\midrule


%\multicolumn{2}{c|}{Average} & \textbf{0.316}  & \textbf{0.314} & 0.377 &0.375  &0.392 &0.383  &0.483 &0.445 &0.537 &0.480 &0.697 &0.537 &0.909 &0.675 &1.341 &0.789 &1.878 &0.994 &1.819 &0.966\\
% \midrule
% \multicolumn{2}{c|}{Average} & & & & & & & & & & & & & & & \\
\bottomrule
\end{tabular}
\label{tab:few_shot_5}
}
% \end{adjustwidth}
\vskip 0.1in
%\vskip -0.1in
\end{sc}
\end{table*}
%}

==> tables_vq/few_shot_5_average.tex <==
%\resizebox{!}{\.5\paperheight}{
%\vskip -0.2in
\begin{table*}[h]
\centering
\begin{sc}

% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Few-shot learning results on 5\% data. All the results are averaged from 4 different prediction lengths $\in \{96,192,336,720\}$ .A lower MSE indicates better performance, and the best results are highlighted in bold.% Full results are in Appendix \ref{subsec_appendix_few_shot}
}%\vspace{-1mm}
\scalebox{0.85}{
\begin{tabular}{cc|cccccccccccccccccc}

\toprule
&{Methods} &\multicolumn{2}{c|}{SVQ} &\multicolumn{2}{c|}{PatchTST} &\multicolumn{2}{c|}{OFA}  &\multicolumn{2}{c|}{Dlinear}  &\multicolumn{2}{c|}{FEDformer} &\multicolumn{2}{c|}{Autoformer} &\multicolumn{2}{c|}{Informer} &\multicolumn{2}{c|}{LogTrans} &\multicolumn{2}{c}{Reformer}\\

\midrule
&{Metric} & MSE  & MAE & MSE & MAE & MSE  & MAE & MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE & MSE  & MAE & MSE & MAE\\
\midrule

&{ETTm1} & \textbf{0.405}  & \textbf{0.412}   & 0.526 & 0.476 & 0.472 & 0.45  & 0.400 & 0.417 & 0.73  & 0.592 & 0.796 & 0.62  & 1.163 & 0.791 & 1.597 & 0.979 & 1.264 & 0.826 \\


\midrule

&{Electricity} & 0.185 & 0.281 &0.181 & 0.277 & 0.178 & \textbf{0.273} & \textbf{0.176} & 0.275 & 0.266 & 0.353 & 0.346 & 0.404 & 1.281 & 0.929 & 0.934 & 0.746 & 1.289 & 0.904 \\

\midrule

&{Traffic} & 0.426  & \textbf{0.288}   & \textbf{0.418} & 0.296 & 0.434 & 0.305 & 0.45  & 0.317 & 0.676 & 0.423 & 0.833 & 0.502 & 1.591 & 0.832 & 1.309 & 0.685 & 1.618 & 0.851 \\


\midrule
&{Weather} & \textbf{0.258}  & \textbf{0.283}   & 0.269 & 0.303 & 0.263 & 0.301 & 0.263 & 0.308 & 0.309 & 0.353 & 0.31  & 0.353 & 0.584 & 0.527 & 0.457 & 0.458 & 0.447 & 0.453 \\

\midrule
&{Wind} & \textbf{1.321}  & \textbf{0.830}   & 1.469 & 0.892 & 1.489 & 0.898 & 1.396 & 0.869 & 1.741 & 1.005 & 1.893 & 1.038 & 4.183 & 1.622 & 3.847 & 1.558 & 2.594 & 1.320 \\

\midrule
&{Nordpool} & \textbf{0.654}  & \textbf{0.608}   & 0.711 & 0.642 & 0.752 & 0.656 & 0.71  & 0.646 & 0.954 & 0.766 & 0.994 & 0.784 & 3.158 & 1.430 & 2.171 & 1.188 & 1.99  & 1.142 \\


\midrule
&{Caiso} & \textbf{0.319}  & \textbf{0.366}   & 0.386 & 0.426 & 0.382 & 0.431 & 0.382 & 0.426 & 0.653 & 0.599 & 0.729 & 0.633 & 1.785 & 0.966 & 1.664 & 0.922 & 1.433 & 0.862\\

\midrule


%\multicolumn{2}{c|}{Average} & \textbf{0.316}  & \textbf{0.314} & 0.377 &0.375  &0.392 &0.383  &0.483 &0.445 &0.537 &0.480 &0.697 &0.537 &0.909 &0.675 &1.341 &0.789 &1.878 &0.994 &1.819 &0.966\\
% \midrule
% \multicolumn{2}{c|}{Average} & & & & & & & & & & & & & & & \\
\bottomrule
\end{tabular}
\label{tab:few_shot_5_average}
}
% \end{adjustwidth}
%\vskip 0.1in
\vskip -0.05in
\end{sc}
\end{table*}
%}

==> tables_vq/full_bench_multi.tex <==
%\resizebox{!}{\.5\paperheight}{
% \vskip -0.2in
\begin{table*}[h]
\centering
\begin{sc}

%\begin{adjustwidth}{-1.5in}{-1in}
\caption{Multivariate long-term series forecasting results on four datasets with same input length $=512$ and various prediction lengths $\in \{96,192,336,720\}$ . A lower MAE indicates better performance. All experiments are repeated 3 times. %Full results of four ETT datasets are in Appendix \ref{subsec_appendix_long_forecasting} .
}\vspace{-2mm}
\scalebox{0.85}{
\begin{tabular}{c|c|cccccccccccccccccc}



\toprule
\multicolumn{2}{c|}{Methods} &\multicolumn{2}{c|}{SVQ} &\multicolumn{2}{c|}{PatchTST} &\multicolumn{2}{c|}{OFA}  &\multicolumn{2}{c|}{Dlinear}  &\multicolumn{2}{c|}{FEDformer} &\multicolumn{2}{c|}{Autoformer} &\multicolumn{2}{c|}{Informer} &\multicolumn{2}{c|}{LogTrans} &\multicolumn{2}{c}{Reformer}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE & MSE  & MAE & MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE & MSE  & MAE & MSE & MAE\\

\midrule
\multirow{5}{*}{\rotatebox{90}{ETTm2}} 

& 96  & 0.158 & 0.242 & 0.166 & 0.256 & 0.173 & 0.262 & 0.167 & 0.26  & 0.203 & 0.287 & 0.255 & 0.339 & 0.705 & 0.69  & 0.768 & 0.642 & 0.365 & 0.453 \\
 & 192 & 0.215 & 0.282 & 0.223 & 0.296 & 0.229 & 0.301 & 0.224 & 0.303 & 0.269 & 0.328 & 0.281 & 0.34  & 0.924 & 0.692 & 0.989 & 0.757 & 0.533 & 0.563 \\
 & 336 & 0.268 & 0.317 & 0.274 & 0.329 & 0.286 & 0.341 & 0.281 & 0.342 & 0.325 & 0.366 & 0.339 & 0.372 & 1.364 & 0.877 & 1.334 & 0.872 & 1.363 & 0.887 \\
 & 720 & 0.349 & 0.371 & 0.362 & 0.385 & 0.378 & 0.401 & 0.397 & 0.421 & 0.421 & 0.415 & 0.422 & 0.419 & 0.877 & 1.074 & 3.048 & 1.328 & 3.379 & 1.338 \\
 & Avg &\textbf{ 0.248} & \textbf{0.303} & 0.256 & 0.317 & 0.267 & 0.326 & 0.267 & 0.332 & 0.305 & 0.349 & 0.324 & 0.368 & 0.968 & 0.833 & 1.535 & 0.900 & 1.41  & 0.810 \\

\midrule
\multirow{5}{*}{\rotatebox{90}{Electricity}}
 & 96  & 0.127 & 0.216 & 0.129 & 0.222 & 0.139 & 0.238 & 0.14  & 0.237 & 0.183 & 0.297 & 0.201 & 0.317 & 0.304 & 0.405 & 0.258 & 0.357 & 0.274 & 0.368 \\
 & 192 & 0.144 & 0.233 & 0.147 & 0.24  & 0.153 & 0.251 & 0.153 & 0.249 & 0.195 & 0.308 & 0.222 & 0.334 & 0.313 & 0.413 & 0.266 & 0.368 & 0.296 & 0.386 \\
 & 336 & 0.161 & 0.251 & 0.163 & 0.259 & 0.169 & 0.266 & 0.169 & 0.267 & 0.212 & 0.313 & 0.231 & 0.338 & 0.29  & 0.381 & 0.28  & 0.38  & 0.3   & 0.394 \\
 & 720 & 0.197 & 0.284 & 0.197 & 0.29  & 0.206 & 0.297 & 0.203 & 0.301 & 0.231 & 0.343 & 0.254 & 0.361 & 0.262 & 0.344 & 0.283 & 0.376 & 0.373 & 0.439 \\
 & Avg &\textbf{ 0.157} & \textbf{0.246} & 0.159 & 0.253 & 0.167 & 0.263 & 0.166 & 0.264 & 0.205 & 0.315 & 0.227 & 0.338 & 0.292 & 0.386 & 0.272 & 0.370 & 0.311 & 0.397 \\

 
\midrule
\multirow{5}{*}{\rotatebox{90}{Traffic}}
 & 96  & 0.377 & 0.241 & 0.36  & 0.249 & 0.388 & 0.282 & 0.41  & 0.282 & 0.562 & 0.349 & 0.613 & 0.388 & 0.824 & 0.514 & 0.684 & 0.384 & 0.719 & 0.391 \\
 & 192 & 0.390 & 0.247 & 0.379 & 0.256 & 0.407 & 0.290 & 0.423 & 0.287 & 0.562 & 0.346 & 0.616 & 0.382 & 1.106 & 0.672 & 0.685 & 0.39  & 0.696 & 0.379 \\
 & 336 & 0.399 & 0.252 & 0.392 & 0.264 & 0.412 & 0.294 & 0.436 & 0.296 & 0.57  & 0.323 & 0.622 & 0.337 & 1.084 & 0.627 & 0.733 & 0.408 & 0.777 & 0.42  \\
 & 720 & 0.438 & 0.275 & 0.432 & 0.286 & 0.450 & 0.312 & 0.466 & 0.315 & 0.596 & 0.368 & 0.66  & 0.408 & 1.536 & 0.845 & 0.717 & 0.396 & 0.864 & 0.472 \\
 & Avg & 0.401 & \textbf{0.254} & \textbf{0.391} & 0.264 & 0.414 & 0.295 & 0.434 & 0.295 & 0.573 & 0.347 & 0.628 & 0.379 & 1.138 & 0.665 & 0.705 & 0.395 & 0.764 & 0.416 \\

 
\midrule
\multirow{5}{*}{\rotatebox{90}{Weather}}
 & 96  & 0.145 & 0.183 & 0.149 & 0.198 & 0.162 & 0.212 & 0.176 & 0.237 & 0.217 & 0.296 & 0.266 & 0.336 & 0.406 & 0.444 & 0.458 & 0.49  & 0.3   & 0.384 \\
 & 192 & 0.188 & 0.228 & 0.194 & 0.241 & 0.204 & 0.248 & 0.22  & 0.282 & 0.276 & 0.336 & 0.307 & 0.367 & 0.525 & 0.527 & 0.658 & 0.589 & 0.598 & 0.544 \\
 & 336 & 0.238 & 0.269 & 0.245 & 0.282 & 0.254 & 0.286 & 0.265 & 0.319 & 0.339 & 0.38  & 0.359 & 0.395 & 0.531 & 0.539 & 0.797 & 0.652 & 0.578 & 0.523 \\
 & 720 & 0.306 & 0.321 & 0.314 & 0.334 & 0.326 & 0.337 & 0.323 & 0.362 & 0.403 & 0.428 & 0.578 & 0.578 & 0.419 & 0.428 & 0.869 & 0.675 & 1.059 & 0.741 \\
 & Avg &\textbf{0.219} & \textbf{0.250} & 0.226 & 0.264 & 0.237 & 0.271 & 0.246 & 0.3   & 0.309 & 0.36  & 0.378 & 0.419 & 0.470 & 0.485 & 0.696 & 0.602 & 0.634 & 0.548 \\

 
\midrule
\multirow{5}{*}{\rotatebox{90}{Wind}}
 & 96  & 0.886 & 0.622 & 0.894 & 0.639 & 0.942 & 0.657 & 0.902 & 0.649 & 1.438 & 0.892 & 1.475 & 0.900 & 1.422 & 0.803 & 1.497 & 0.849 & 1.097 & 0.705 \\
 & 192 & 1.133 & 0.748 & 1.166 & 0.782 & 1.168 & 0.774 & 1.124 & 0.766 & 1.572 & 0.945 & 1.720 & 0.973 & 1.810 & 0.950 & 1.574 & 0.911 & 1.279 & 0.783 \\
 & 336 & 1.275 & 0.841 & 1.374 & 0.875 & 1.387 & 0.872 & 1.329 & 0.862 & 1.815 & 1.031 & 1.667 & 0.968 & 1.714 & 0.926 & 1.551 & 0.918 & 1.471 & 0.897 \\
 & 720 & 1.418 & 0.910 & 1.545 & 0.955 & 1.587 & 0.955 & 1.495 & 0.935 & 1.788 & 1.021 & 1.738 & 1.000 & 1.877 & 0.990 & 1.602 & 0.952 & 1.502 & 0.944 \\
 & Avg &\textbf{ 1.178} & \textbf{0.780} & 1.245 & 0.813 & 1.271 & 0.815 & 1.213 & 0.803 & 1.653 & 0.972 & 1.65  & 0.960 & 1.706 & 0.917 & 1.556 & 0.908 & 1.337 & 0.832 \\

\midrule
\multirow{5}{*}{\rotatebox{90}{Nordpool}}
 & 96  & 0.543 & 0.540 & 0.560 & 0.558 & 0.563 & 0.556 & 0.613 & 0.593 & 0.552 & 0.579 & 0.815 & 0.702 & 1.029 & 0.788 & 0.858 & 0.691 & 0.645 & 0.618 \\
 & 192 & 0.608 & 0.579 & 0.632 & 0.594 & 0.613 & 0.590 & 0.674 & 0.636 & 0.646 & 0.634 & 0.795 & 0.697 & 1.030 & 0.804 & 0.918 & 0.715 & 0.728 & 0.659 \\
 & 336 & 0.593 & 0.578 & 0.596 & 0.594 & 0.595 & 0.587 & 0.653 & 0.628 & 0.599 & 0.593 & 0.829 & 0.713 & 1.198 & 0.860 & 0.953 & 0.744 & 0.782 & 0.675 \\
 & 720 & 0.585 & 0.580 & 0.586 & 0.590 & 0.580 & 0.587 & 0.642 & 0.627 & 0.634 & 0.624 & 0.736 & 0.672 & 1.246 & 0.865 & 0.997 & 0.759 & 0.836 & 0.694 \\
 & Avg &\textbf{ 0.582} & \textbf{0.569} & 0.594 & 0.584 & 0.588 & 0.58  & 0.646 & 0.621 & 0.608 & 0.608 & 0.794 & 0.696 & 1.126 & 0.829 & 0.932 & 0.727 & 0.748 & 0.662 \\

 
\midrule
\multirow{5}{*}{\rotatebox{90}{Caiso}} 
 & 96  & 0.204 & 0.286 & 0.237 & 0.307 & 0.210 & 0.297 & 0.221 & 0.302 & 0.265 & 0.365 & 0.327 & 0.406 & 0.320 & 0.394 & 0.261 & 0.355 & 0.242 & 0.343 \\
 & 192 & 0.279 & 0.341 & 0.323 & 0.364 & 0.276 & 0.349 & 0.279 & 0.350 & 0.325 & 0.413 & 0.462 & 0.499 & 0.415 & 0.457 & 0.295 & 0.378 & 0.285 & 0.372 \\
 & 336 & 0.331 & 0.376 & 0.370 & 0.402 & 0.330 & 0.389 & 0.328 & 0.388 & 0.345 & 0.421 & 0.584 & 0.552 & 0.473 & 0.492 & 0.368 & 0.458 & 0.343 & 0.455 \\
 & 720 & 0.430 & 0.428 & 0.456 & 0.458 & 0.466 & 0.456 & 0.450 & 0.459 & 0.416 & 0.471 & 0.505 & 0.517 & 0.536 & 0.533 & 0.506 & 0.503 & 0.498 & 0.489 \\
 & Avg &\textbf{ 0.311} & \textbf{0.357} & 0.347 & 0.383 & 0.321 & 0.373 & 0.320 & 0.375 & 0.338 & 0.418 & 0.470 & 0.494 & 0.436 & 0.469 & 0.358 & 0.424 & 0.342 & 0.415 \\
 

\midrule

% \midrule
% \multicolumn{2}{c|}{Average} & & & & & & & & & & & & & & & \\
\bottomrule
\end{tabular}
\label{tab:full_bench_multi}
}
% \end{adjustwidth}
%\vskip 0.1in
\vskip -0.1in
\end{sc}
\end{table*}
%}

==> tables_vq/full_bench_multi_concise.tex <==
%\resizebox{!}{\.5\paperheight}{
% \vskip -0.2in
\begin{table*}[h]
\centering
\begin{sc}

%\begin{adjustwidth}{-1.5in}{-1in}
\caption{Multivariate long-term series forecasting results. All the results are with same input length $=512$ and averaged from 4 different prediction lengths $\in \{96,192,336,720\}$ . A lower MAE indicates better performance. %All experiments are repeated 3 times. %Full results of four ETT datasets are in Appendix \ref{subsec_appendix_long_forecasting} .
}\vspace{-2mm}
\scalebox{0.80}{
\begin{tabular}{cc|cccccccccccccccccc}



\toprule
&{Methods} &\multicolumn{2}{c|}{SVQ} &\multicolumn{2}{c|}{PatchTST} &\multicolumn{2}{c|}{OFA}  &\multicolumn{2}{c|}{Dlinear}  &\multicolumn{2}{c|}{FEDformer} &\multicolumn{2}{c|}{Autoformer} &\multicolumn{2}{c|}{Informer} &\multicolumn{2}{c|}{LogTrans} &\multicolumn{2}{c}{Reformer}\\
\midrule
&{Metric} & MSE  & MAE & MSE & MAE & MSE  & MAE & MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE & MSE  & MAE & MSE & MAE\\

\midrule
&{ETTm2}
 &\textbf{ 0.248} & \textbf{0.303} & 0.256 & 0.317 & 0.267 & 0.326 & 0.267 & 0.332 & 0.305 & 0.349 & 0.324 & 0.368 & 0.968 & 0.833 & 1.535 & 0.900 & 1.41  & 0.810 \\

\midrule
&{Electricity}
 &\textbf{ 0.157} & \textbf{0.246} & 0.159 & 0.253 & 0.167 & 0.263 & 0.166 & 0.264 & 0.205 & 0.315 & 0.227 & 0.338 & 0.292 & 0.386 & 0.272 & 0.370 & 0.311 & 0.397 \\

 
\midrule
&{Traffic}
 & 0.401 & \textbf{0.254} & \textbf{0.391} & 0.264 & 0.414 & 0.295 & 0.434 & 0.295 & 0.573 & 0.347 & 0.628 & 0.379 & 1.138 & 0.665 & 0.705 & 0.395 & 0.764 & 0.416 \\

 
\midrule
&{Weather}
 &\textbf{0.219} & \textbf{0.250} & 0.226 & 0.264 & 0.237 & 0.271 & 0.246 & 0.3   & 0.309 & 0.36  & 0.378 & 0.419 & 0.470 & 0.485 & 0.696 & 0.602 & 0.634 & 0.548 \\

 
\midrule
&{Wind}
 &\textbf{ 1.178} & \textbf{0.780} & 1.245 & 0.813 & 1.271 & 0.815 & 1.213 & 0.803 & 1.653 & 0.972 & 1.65  & 0.960 & 1.706 & 0.917 & 1.556 & 0.908 & 1.337 & 0.832 \\

\midrule
&{Nordpool}
 &\textbf{ 0.582} & \textbf{0.569} & 0.594 & 0.584 & 0.588 & 0.58  & 0.646 & 0.621 & 0.608 & 0.608 & 0.794 & 0.696 & 1.126 & 0.829 & 0.932 & 0.727 & 0.748 & 0.662 \\

 
\midrule
&{Caiso}
 &\textbf{ 0.311} & \textbf{0.357} & 0.347 & 0.383 & 0.321 & 0.373 & 0.320 & 0.375 & 0.338 & 0.418 & 0.470 & 0.494 & 0.436 & 0.469 & 0.358 & 0.424 & 0.342 & 0.415 \\
 

\midrule

% \midrule
% \multicolumn{2}{c|}{Average} & & & & & & & & & & & & & & & \\
\bottomrule
\end{tabular}
\label{tab:full_bench_multi_concise}
}
% \end{adjustwidth}
%\vskip 0.1in
\vskip -0.1in
\end{sc}
\end{table*}
%}

==> tables_vq/full_bench_uni.tex <==
%\resizebox{!}{\.5\paperheight}{
% \vskip -0.2in
\begin{table*}[t]
\centering
\begin{sc}

% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Univariate long-term series forecasting results on ten datasets with same input length $=512$ and prediction length $\in \{96,192,336,720\}$. A lower MAE indicates better performance. All experiments are repeated 3 times.}\vspace{-1mm}
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccccccccccccc}



\toprule
\multicolumn{2}{c|}{Methods} &\multicolumn{2}{c|}{SVQ} &\multicolumn{2}{c|}{PatchTST} &\multicolumn{2}{c|}{OFA}  &\multicolumn{2}{c|}{Dlinear}  &\multicolumn{2}{c|}{FEDformer} &\multicolumn{2}{c|}{Autoformer} &\multicolumn{2}{c|}{Informer} &\multicolumn{2}{c|}{LogTrans} &\multicolumn{2}{c}{Reformer}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE & MSE  & MAE & MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE & MSE  & MAE & MSE & MAE\\

 

\midrule
\multirow{5}{*}{\rotatebox{90}{ETTm2}} 

&96  & 0.063           & 0.183           & 0.065  & 0.187  & 0.066  & 0.191  & 0.063  & 0.183          & 0.063  & 0.189  & 0.065  & 0.189 & 0.088  & 0.225 & 0.075  & 0.208 & 0.076  & 0.214 \\
&192 & 0.090           & 0.225           & 0.093  & 0.230  & 0.098  & 0.262  & 0.092  & 0.227          & 0.102  & 0.245  & 0.118  & 0.256 & 0.132  & 0.283 & 0.129  & 0.275 & 0.132  & 0.29  \\
&336 & 0.118           & 0.262           & 0.122  & 0.267  & 0.134  & 0.305  & 0.119  & 0.261          & 0.13   & 0.279  & 0.154  & 0.305 & 0.18   & 0.336 & 0.154  & 0.302 & 0.16   & 0.312 \\
&720 & 0.172           & 0.320           & 0.173  & 0.324  & 0.176  & 0.328  & 0.175  & 0.320          & 0.178  & 0.325  & 0.182  & 0.335 & 0.3    & 0.435 & 0.16   & 0.321 & 0.168  & 0.335 \\
&Avg & \textbf{0.111}  & \textbf{0.248}  & 0.113  & 0.252  & 0.119  & 0.272  & 0.112  & \textbf{0.248} & 0.118  & 0.2595 & 0.130  & 0.271 & 0.175  & 0.320 & 0.130  & 0.277 & 0.134  & 0.288 \\


\midrule
\multirow{5}{*}{\rotatebox{90}{Electricity}}
&96  & 0.194           & 0.304           & 0.209  & 0.321  & 0.212  & 0.321  & 0.202  & 0.314          & 0.253  & 0.37   & 0.341  & 0.438 & 0.484  & 0.538 & 0.288  & 0.393 & 0.274  & 0.379 \\
&192 & 0.226           & 0.325           & 0.246  & 0.344  & 0.266  & 0.358  & 0.233  & 0.336          & 0.282  & 0.386  & 0.345  & 0.428 & 0.557  & 0.558 & 0.432  & 0.483 & 0.304  & 0.402 \\
&336 & 0.263           & 0.358           & 0.280  & 0.379  & 0.306  & 0.385  & 0.270  & 0.364          & 0.346  & 0.431  & 0.406  & 0.47  & 0.636  & 0.613 & 0.43   & 0.483 & 0.37   & 0.448 \\
&720 & 0.298           & 0.404           & 0.332  & 0.424  & 0.383  & 0.455  & 0.303  & 0.406          & 0.422  & 0.484  & 0.565  & 0.581 & 0.819  & 0.682 & 0.491  & 0.531 & 0.46   & 0.511 \\
&Avg & \textbf{0.245}  & \textbf{0.348}  & 0.267  & 0.367  & 0.292  & 0.380  & 0.252  & 0.355          & 0.326  & 0.418  & 0.414  & 0.479 & 0.624  & 0.598 & 0.410  & 0.473 & 0.352  & 0.435 \\

\midrule
\multirow{5}{*}{\rotatebox{90}{Traffic}} 
&96  & 0.115           & 0.183           & 0.134  & 0.223  & 0.145  & 0.252  & 0.122  & 0.194          & 0.17   & 0.263  & 0.246  & 0.346 & 0.257  & 0.353 & 0.226  & 0.317 & 0.313  & 0.383 \\
&192 & 0.112           & 0.182           & 0.130  & 0.221  & 0.148  & 0.255  & 0.125  & 0.199          & 0.173  & 0.265  & 0.266  & 0.37  & 0.299  & 0.376 & 0.314  & 0.408 & 0.386  & 0.453 \\
&336 & 0.113           & 0.190           & 0.133  & 0.227  & 0.156  & 0.261  & 0.124  & 0.202          & 0.178  & 0.266  & 0.263  & 0.371 & 0.312  & 0.387 & 0.387  & 0.453 & 0.423  & 0.468 \\
&720 & 0.126           & 0.204           & 0.146  & 0.241  & 0.173  & 0.276  & 0.139  & 0.222          & 0.187  & 0.286  & 0.269  & 0.372 & 0.366  & 0.436 & 0.491  & 0.437 & 0.378  & 0.433 \\
&Avg & \textbf{0.117}  & \textbf{0.190}  & 0.136  & 0.228  & 0.156  & 0.261  & 0.128  & 0.204          & 0.177  & 0.27   & 0.261  & 0.365 & 0.309  & 0.388 & 0.355  & 0.404 & 0.375  & 0.434 \\

\midrule
\multirow{5}{*}{\rotatebox{90}{Weather}} 
&96  & 0.0009          & 0.0210          & 0.0013 & 0.0265 & 0.0013 & 0.028  & 0.0050 & 0.056          & 0.0035 & 0.046  & 0.011  & 0.081 & 0.0038 & 0.044 & 0.0046 & 0.052 & 0.012  & 0.087 \\
&192 & 0.0011          & 0.0239          & 0.0014 & 0.0281 & 0.0014 & 0.0295 & 0.0061 & 0.065          & 0.0054 & 0.059  & 0.0075 & 0.067 & 0.0023 & 0.04  & 0.0056 & 0.06  & 0.0098 & 0.079 \\
&336 & 0.0013          & 0.0258          & 0.0015 & 0.0289 & 0.0017 & 0.031  & 0.0064 & 0.067          & 0.0041 & 0.05   & 0.0063 & 0.062 & 0.0041 & 0.049 & 0.006  & 0.054 & 0.005  & 0.059 \\
&720 & 0.0018          & 0.0305          & 0.0021 & 0.0341 & 0.0022 & 0.036  & 0.0068 & 0.070          & 0.015  & 0.091  & 0.0085 & 0.07  & 0.0031 & 0.042 & 0.0071 & 0.063 & 0.0041 & 0.049 \\
&Avg & \textbf{0.0013} & \textbf{0.0253} & 0.0016 & 0.0294 & 0.0017 & 0.0311 & 0.0061 & 0.0645         & 0.007  & 0.0615 & 0.0083 & 0.07  & 0.0033 & 0.044 & 0.0058 & 0.057 & 0.0077 & 0.069 \\

\midrule
\multirow{5}{*}{\rotatebox{90}{Wind}} 
&96  & 2.370           & 1.211           & 2.563  & 1.261  & 2.683  & 1.296  & 2.539  & 1.239          & 3.278  & 1.490  & 3.177  & 1.485 & 3.468  & 1.395 & 3.936  & 1.468 & 3.110  & 1.332 \\
&192 & 2.742           & 1.338           & 3.001  & 1.391  & 3.310  & 1.492  & 3.102  & 1.395          & 3.763  & 1.620  & 3.645  & 1.599 & 3.973  & 1.502 & 4.748  & 1.639 & 3.912  & 1.496 \\
&336 & 2.850           & 1.385           & 3.317  & 1.489  & 3.764  & 1.630  & 3.468  & 1.496          & 4.053  & 1.702  & 4.192  & 1.737 & 4.221  & 1.568 & 5.281  & 1.743 & 4.024  & 1.536 \\
&720 & 3.213           & 1.471           & 3.454  & 1.515  & 4.067  & 1.701  & 3.718  & 1.568          & 4.139  & 1.741  & 4.270  & 1.771 & 4.176  & 1.558 & 4.652  & 1.639 & 4.359  & 1.593 \\
&Avg & \textbf{2.794}  & \textbf{1.351}  & 3.084  & 1.414  & 3.456  & 1.530  & 3.207  & 1.425          & 3.808  & 1.638  & 3.821  & 1.648 & 3.960  & 1.506 & 4.654  & 1.622 & 3.851  & 1.489 \\

\midrule
\multirow{5}{*}{\rotatebox{90}{Nordpool}}
&96  & 0.871           & 0.702           & 0.856  & 0.714  & 0.868  & 0.716  & 0.853  & 0.715          & 0.849  & 0.736  & 0.932  & 0.767 & 0.921  & 0.758 & 0.895  & 0.720 & 0.904  & 0.722 \\
&192 & 0.776           & 0.667           & 0.930  & 0.748  & 0.938  & 0.757  & 0.926  & 0.758          & 0.914  & 0.777  & 1.061  & 0.831 & 0.848  & 0.731 & 0.868  & 0.727 & 0.858  & 0.713 \\
&336 & 0.777           & 0.681           & 0.900  & 0.749  & 0.906  & 0.753  & 0.896  & 0.752          & 0.863  & 0.747  & 0.966  & 0.785 & 0.812  & 0.709 & 0.855  & 0.725 & 0.877  & 0.754 \\
&720 & 0.768           & 0.687           & 0.872  & 0.747  & 0.871  & 0.746  & 0.873  & 0.748          & 0.878  & 0.755  & 1.035  & 0.817 & 0.816  & 0.713 & 0.909  & 0.745 & 0.851  & 0.767 \\
&Avg & \textbf{0.798}  & \textbf{0.684}  & 0.890  & 0.740  & 0.896  & 0.743  & 0.887  & 0.743          & 0.876  & 0.754  & 0.999  & 0.8   & 0.849  & 0.728 & 0.882  & 0.729 & 0.873  & 0.739 \\

\midrule
\multirow{5}{*}{\rotatebox{90}{Caiso}}
&96  & 0.140           & 0.255           & 0.162  & 0.279  & 0.169  & 0.285  & 0.151  & 0.262          & 0.191  & 0.327  & 0.227  & 0.353 & 0.217  & 0.337 & 0.206  & 0.311 & 0.207  & 0.340 \\
&192 & 0.211           & 0.308           & 0.212  & 0.322  & 0.233  & 0.328  & 0.215  & 0.312          & 0.247  & 0.367  & 0.262  & 0.370 & 0.293  & 0.394 & 0.254  & 0.360 & 0.221  & 0.344 \\
&336 & 0.257           & 0.342           & 0.263  & 0.355  & 0.281  & 0.361  & 0.259  & 0.346          & 0.266  & 0.360  & 0.299  & 0.399 & 0.302  & 0.405 & 0.310  & 0.422 & 0.298  & 0.396 \\
&720 & 0.325           & 0.391           & 0.325  & 0.403  & 0.373  & 0.424  & 0.346  & 0.404          & 0.372  & 0.451  & 0.504  & 0.535 & 0.382  & 0.464 & 0.380  & 0.479 & 0.356  & 0.441 \\
&Avg & \textbf{0.233}  & \textbf{0.324}  & 0.241  & 0.340  & 0.264  & 0.3495 & 0.243  & 0.331          & 0.269  & 0.376  & 0.323  & 0.414 & 0.299  & 0.4   & 0.288  & 0.393 & 0.271  & 0.380\\

\midrule
% \multicolumn{2}{c|}{Average} & & & & & & & & & & & & & & & \\
\bottomrule
\end{tabular}
\label{tab:full_bench_uni}
}
% \end{adjustwidth}
%\vskip -0.2in
%\vskip -0.1in
\end{sc}
\end{table*}
%}

==> tables_vq/full_bench_uni_concise.tex <==
%\resizebox{!}{\.5\paperheight}{
% \vskip -0.2in
\begin{table*}[h]
\centering
\begin{sc}

% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Univariate long-term forecasting task. All the results are with same input length $=512$ averaged from 4 different prediction lengths $\in \{96,192,336,720\}$. A lower MAE indicates better performance.}\vspace{-2mm}% All experiments are repeated 3 times. Appendix \ref{subsec_appendix_long_forecasting}  shows the full results.}\vspace{-3mm}

%Univariate long-term series forecasting results with same input length $=512$ and prediction length $\in \{96,192,336,720\}$. A lower MAE indicates better performance. All experiments are repeated 3 times. Full results are in appendix .}\vspace{-1mm}
\scalebox{0.75}{
\begin{tabular}{cc|ccccccccccccccccccc}



\toprule
&{Methods} &\multicolumn{2}{c|}{SVQ} &\multicolumn{2}{c|}{PatchTST} &\multicolumn{2}{c|}{OFA}  &\multicolumn{2}{c|}{Dlinear}  &\multicolumn{2}{c|}{FEDformer} &\multicolumn{2}{c|}{Autoformer} &\multicolumn{2}{c|}{Informer} &\multicolumn{2}{c|}{LogTrans} &\multicolumn{2}{c}{Reformer}\\
\midrule
&{Metric} & MSE  & MAE & MSE & MAE & MSE  & MAE & MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE & MSE  & MAE & MSE & MAE\\
\midrule
&{ETTm2}

& \textbf{0.111}  & \textbf{0.248}  & 0.113  & 0.252  & 0.119  & 0.272  & 0.112  & \textbf{0.248} & 0.118  & 0.2595 & 0.130  & 0.271 & 0.175  & 0.320 & 0.130  & 0.277 & 0.134  & 0.288 \\


\midrule
&{Electricity}
& \textbf{0.245}  & \textbf{0.348}  & 0.267  & 0.367  & 0.292  & 0.380  & 0.252  & 0.355          & 0.326  & 0.418  & 0.414  & 0.479 & 0.624  & 0.598 & 0.410  & 0.473 & 0.352  & 0.435 \\

\midrule
&{Traffic}
 & \textbf{0.117}  & \textbf{0.190}  & 0.136  & 0.228  & 0.156  & 0.261  & 0.128  & 0.204          & 0.177  & 0.27   & 0.261  & 0.365 & 0.309  & 0.388 & 0.355  & 0.404 & 0.375  & 0.434 \\

\midrule
&{Weather}
 & \textbf{0.0013} & \textbf{0.0253} & 0.0016 & 0.0294 & 0.0017 & 0.0311 & 0.0061 & 0.0645         & 0.007  & 0.0615 & 0.0083 & 0.07  & 0.0033 & 0.044 & 0.0058 & 0.057 & 0.0077 & 0.069 \\

\midrule
&{Wind}

 & \textbf{2.794}  & \textbf{1.351}  & 3.084  & 1.414  & 3.456  & 1.530  & 3.207  & 1.425          & 3.808  & 1.638  & 3.821  & 1.648 & 3.960  & 1.506 & 4.654  & 1.622 & 3.851  & 1.489 \\

\midrule
&{Nordpool}
 & \textbf{0.798}  & \textbf{0.684}  & 0.890  & 0.740  & 0.896  & 0.743  & 0.887  & 0.743          & 0.876  & 0.754  & 0.999  & 0.8   & 0.849  & 0.728 & 0.882  & 0.729 & 0.873  & 0.739 \\

\midrule
&{Caiso}
 & \textbf{0.233}  & \textbf{0.324}  & 0.241  & 0.340  & 0.264  & 0.3495 & 0.243  & 0.331          & 0.269  & 0.376  & 0.323  & 0.414 & 0.299  & 0.4   & 0.288  & 0.393 & 0.271  & 0.380\\

\midrule
% \multicolumn{2}{c|}{Average} & & & & & & & & & & & & & & & \\
\bottomrule
\end{tabular}
\label{tab:full_bench_uni_concise}
}
% \end{adjustwidth}
%\vskip -0.1in
\vskip -0.1in
\end{sc}
\end{table*}
%}

==> tables_vq/parameters.tex <==
%\resizebox{!}{\.5\paperheight}{
% \vskip -0.2in
\begin{table}[t]
\begin{center}
% \begin{small}
\begin{sc}

%\color{blue}
\caption{Model parameter comparison for PatchTST and PatchTST with FFN-free structure, both the input length $=512$, univariate prediction length $O\in \{96, 192, 336, 720\}$. The amount of parameters is expressed in millions (M).}
\vspace{-1mm}
\scalebox{0.85}{
\begin{tabular}{c|ccccccc}
\toprule
%I’m 
{$Param(M)$} &{96} &{192} &{336} &{720} \\
\midrule

PatchTST  &0.604	&0.801	&1.096	&1.883	\\
$FFN_{free}$  &0.406	&0.603	&0.898	&1.685 \\
Reduction  & $\downarrow32.78\%$ & $\downarrow 24.72\%$ & $\downarrow 18.07\%$  & $\downarrow 10.52\%$ \\

\midrule
%average21.52%
\bottomrule
\end{tabular}
}
\label{tab:FFN_parameters}
% \end{adjustwidth}
%\end{footnotesize}
\end{sc}
% \end{small}
\end{center}
\vskip -0.3in
\end{table}
%}







==> tables_vq/short_forecasting_average.tex <==
%\resizebox{!}{\.5\paperheight}{
% \vskip -0.2in
\begin{table*}[t]
\centering
\begin{sc}

% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Short-term forecasting task on M4. The prediction lengths are $\in \{6, 48\}$ and results are weighted
averaged from several datasets under different sample intervals. A lower score indicates better performance.% All experiments are repeated 3 times.%Full results are in Appendix \ref{subsec_appendix_short_forecasting}
}\vspace{-1mm}
\scalebox{0.80}{
\begin{tabular}{cc|cccccccccccccccccc}

\toprule


%\multicolumn{2}{c|}
&{Methods} &{SVQ} &{OFA} &{PatchTST} &{N-HiTS} &{N-BEATS} &{ETSformer} &{LighTS} &{Dlinear} &{FEDformer} &{Autoformer} &{Informer} &{Reformer} \\
\midrule
%\multirow{3}{*}{\rotatebox{90}{Average}} 

& SMAPE & 11.938 &{11.991} &12.059&11.927 &\textbf{11.851} &14.718 &13.525 &13.639 &12.840 &12.909 &14.086 &18.200 \\
& MASE & \textbf{1.593} & {1.600} &1.623 &1.613 &1.599 &2.408 &2.111 &2.095 &1.701 &1.771 &2.718 &4.223   \\
& OWA & 0.857 & {0.861} &0.869 &0.861 &\textbf{0.855} &1.172 &1.051 &1.051 &0.918&0.939 &1.230 &1.775 \\
\midrule

% \midrule
% \multicolumn{2}{c|}{Average} & & & & & & & & & & & & & & & \\
\bottomrule
\end{tabular}
\label{tab:short_forecasting_average}
}
% \end{adjustwidth}
%\vskip 0.1in
%\vskip -0.1in
\end{sc}
\end{table*}
%}
